Solving fluid flow problems in space-time with multiscale stabilization: formulation and examples

We present a space-time continuous-Galerkin finite element method for solving incompressible Navier-Stokes equations. To ensure stability of the discrete variational problem, we apply ideas from the variational multi-scale method. The finite element problem is posed on the ``full" space-time domain, considering time as another dimension. We provide a rigorous analysis of the stability and convergence of the stabilized formulation. And finally, we apply this method on two benchmark problems in computational fluid dynamics, namely, lid-driven cavity flow and flow past a circular cylinder. We validate the current method with existing results from literature and show that very large space-time blocks can be solved using our approach.

==> auxiliary/extras.tex <==
\section{Solution of the nonlinear system of equations}
\subsection{Solving nonlinear equations}\label{sec:implementation-nonlinear-solve}
The FEM problem formulated in \eqref{eq:fem-problem-vms} is a coupled nonlinear equation. To solve it numerically, we use the Newton-Raphson method \cite{leveque2007finite}. Suppose, the nonlinear system of equations resulting from  \eqref{eq:fem-problem-vms} is written as:
\begin{align}\label{eq:nla-nonlinear-system}
\mvec{b^g}(\mvec{x^g})=\mvec{f^g}
\end{align}
where $ \mvec{b^g} $ and $ \mvec{f^g} $ are the numerical versions of $ B^h $ and $ F^h $; and $ \mvec{x^g} $ is the vector containing all the unknown discrete degrees of freedoms, i.e.,
\begin{align}
\mvec{x^g} = \left( u_{x1},u_{y1}, u_{z1}, p_1, u_{x2},u_{y2}, u_{z2}, p_2,...,u_{xN},u_{yN}, u_{zN}, p_N  \right)
\end{align}
where $ N $ is the total number of nodes in the discretization $ \mesh $.
Assume that the unknown vector at the $ r^{th} $ iteration is denoted as $ \mvec{x^g}_r $. Then following the Newton-Raphson methodology, the $ (r+1)^{th} $-step is linearized in the neighborhood of $ \mvec{x^g}_r $ as:
\begin{align}\label{eq:nla-linearized-system}
\mvec{J}(\mvec{x^g}_r)\cdot\delta\mvec{x^g}_r = \mvec{z^g}
\end{align}
where $ \mvec{z^g} = \left(\mvec{f^g} - \mvec{b^g}(\mvec{x^g}_r)\right) $ is a known vector and  $ \mvec{J} $ is the Jacobian matrix, whose $ (i,j) $ element is the first derivative of the $ i $-th element of $ \mvec{b^g} $ with respect to the $ j $-th element of $ \mvec{x^g} $, i.e., $ J_{ij} = \partialder{b^g_i}{x^g_j} $.  \eqref{eq:nla-linearized-system} is now solved for $ \delta \mvec{x^g_r} $ and then $ \mvec{x^g}_{r+1} $ is obtained from:
\begin{align}\label{eq:nla-newton-update}
\mvec{x^g}_{r+1} = \mvec{x^g}_{r} + \delta \mvec{x^g}_{r},\quad r = 0,1,2,...
\end{align}
$ \mvec{x^g}_0 $ is the initial guess provided at the start of the Newton-Raphson iterations. The iteration is stopped when the norm of the increment vector $ \xvec^{\mvec{g}}_r $ is less than some previously set tolerance value $ \gamma > 0 $, i.e., when $ \norm{\delta \xvec^{\mvec{g}}_r}\leq\gamma $, where usually $ \gamma $ is a small real number.

The key step in the linear algebra problem is now  \eqref{eq:nla-linearized-system} which requires the solution of a large linear algebraic system. We use \petsc{} \cite{balay2001petsc} for solving this linear system. Once the global Jacobian matrix $ \mvec{J} $ and the global right hand side $ \mvec{z^g} $ are assembled, \petsc{} functions are called to solve  \eqref{eq:nla-linearized-system} for $ \delta\mvec{x^g}_r $. Once again, since the dimensionality of the problem is high, so is the size of $ \mvec{J} $. Thus, direct/non-iterative solvers such as LU-decomposition (with complexity $ O(n^3) $, $ n= $ matrix size) become very inefficient. Iterative methods, on the other hand, take about $\sim O(mn) $ time \cite{trefethen1997numerical} (where $ m $ is the number of iterations, $ m \ll n $) for sparse matrices, and are therefore preferred.

\subsection{Method of Continuation}\label{sec:implementation-moc}
A space-time formulation, as described in this paper, is by definition non-evolutionary. It is seen in  \eqref{eq:fem-problem-vms} which is formulated over a Hilbert space whose underlying domain is spatio-temporal; and consequently the algebraic problem in  \eqref{eq:nla-nonlinear-system} or \eqref{eq:nla-linearized-system} contain unknowns that span the full spatio-temporal domain $ \Omega $. When solving such equations using the Newton-Raphson scheme \eqref{eq:nla-linearized-system}, an initial guess for $ \xvec^{\mvec{g}}_r $ is required. One common characteristic of the Newton-Raphson method is that the convergence of system \eqref{eq:nla-linearized-system} depends on the quality of the initial guess $ \xvec^\mvec{g}_r $. Suppose the exact solution of the system \eqref{eq:nla-nonlinear-system} is $ \xvec^\mvec{g}_* $. Then, if $ \| \xvec^\mvec{g}_0-\xvec^\mvec{g}_* \|  $ is large, then the scheme \eqref{eq:nla-linearized-system} and \eqref{eq:nla-newton-update} might fail to converge to $ \xvec^\mvec{g}_* $. In these cases, we cannot simply rely solely on the increment $ \delta \xvec^{\mvec{g}}_r $ provided by the Newton-Raphson scheme \eqref{eq:nla-linearized-system}.

Thus, to overcome this issue, we use a variant of the method of continuation, known as the pseudo-transient continuation (PTC)  \cite{coffey2003pseudotransient, kelley1998convergence}. We do this by embedding the fully coupled space-time system of equations \eqref{eq:nla-nonlinear-system} in an auxiliary evolution space $ \tau $ as follows:
\begin{align}\label{eq:nla-nonlinear-system-ptc}
\partialder{\mvec{x^g}}{\tau} + \mvec{b^g}(\mvec{x^g})=\mvec{f^g}.
\end{align}
If we compare  \eqref{eq:nla-nonlinear-system-ptc} with  \eqref{eq:nla-nonlinear-system}, we can infer the role of the variable $ \tau $. In the ideal case, we want  \eqref{eq:nla-nonlinear-system-ptc} and \eqref{eq:nla-nonlinear-system} to yield the same solution for $ \mvec{x^g} $, thereby making $ \partialder{\mvec{x^g}}{\tau} = 0 $. This gives us an opportunity to design an iteration scheme similar to a time-marching algorithm that ``evolves'' the space-time solution $ \mvec{x^g} $  with respect to $ \tau $. Assume a discretization of the auxiliary variable $ \tau $ given by $ \tau^h = (\tau^0, \tau^1,...) $, where the elements in $ \tau^h $ are not necessarily equidistant. With this, we can approximate  \eqref{eq:nla-nonlinear-system-ptc} as
\begin{align}\label{eq:nla-nonlinear-system-ptc-beuler}
\frac{\mvec{x}^{\mvec{g}^{k+1}} - \mvec{x}^{\mvec{g}^{k}} }{\Delta \tau^{k+1}} + \mvec{b^g}(\mvec{x}^{\mvec{g}^{k+1}}) &=\mvec{f^g} \\
\label{eq:nla-nonlinear-system-ptc-beuler-iterations}
\implies \quad\quad\frac{\mvec{x}^{\mvec{g}^{k+1}}}{\Delta \tau^{k+1}} + \mvec{b^g}(\mvec{x}^{\mvec{g}^{k+1}}) &=\frac{\mvec{x}^{\mvec{g}^{k}} }{\Delta \tau^{k+1}} + \mvec{f^g},\quad k = 0,1,2,...,
\end{align}
where $ \Delta \tau^{k+1} = \tau^{k+1}-\tau^k $. With a sufficiently small choice of $ \Delta \tau^{k+1} $,  \eqref{eq:nla-nonlinear-system-ptc-beuler-iterations} is a contraction for $ \mvec{x^g} $, i.e., there exists a $ K^{\infty}\in\mathbb{N} $ such that $\|\mvec{x}^{\mvec{g}^k}- \mvec{x}^{\mvec{g}}_* \| \leq \epsilon$ for all $ k \geq K^{\infty} $. At $ k=0 $, we do not have a solution, rather, we just have an initial guess denoted by $ \mvec{x}^{\mvec{g}^{0}} $. But as we solve  \eqref{eq:nla-nonlinear-system-ptc-beuler-iterations} successively, each $ \mvec{x}^{\mvec{g}^k} $ gets closer and closer to the true solution $ \mvec{x}^{\mvec{g}}_* $.

\eqref{eq:nla-nonlinear-system-ptc-beuler-iterations} is still nonlinear in $ \mvec{x^g} $. Thus applying Newton-Raphson linearization to  \eqref{eq:nla-nonlinear-system-ptc-beuler-iterations}, we have:
\begin{align}\label{eq:nla-linearized-system-ptc-beuler}
\left[ \frac{\mvec{M}}{\Delta \tau^{k+1}} + \mvec{J}(\mvec{x}^{\mvec{g}^{k+1}}_r) \right]\cdot\delta \mvec{x}^{\mvec{g}^{k+1}}_r &= \mvec{z}^{\mvec{g}^{k+1}},\\
\label{eq:nla-newton-update-ptc-beuler}
\mvec{x}^{\mvec{g}^{k+1}}_{r+1} &= \mvec{x}^{\mvec{g}^{k+1}}_{r} + \delta \mvec{x}^{\mvec{g}^{k+1}}_{r},\quad r = 0,1,2,...
\end{align}
where $ \mvec{z}^{\mvec{g}^{k+1}}  = \left(\mvec{x}^{\mvec{g}^k}/\Delta \tau^{k+1} + \mvec{f^g} - \mvec{b^g}(\mvec{x}^{\mvec{g}^k}_r)\right)$. 

Once again, iteration \eqref{eq:nla-newton-update-ptc-beuler} is stopped when $ \norm{\delta\xvec^{\mvec{g}^{k+1}}_r} < \gamma_1$, and the backward Euler iterations \eqref{eq:nla-nonlinear-system-ptc-beuler-iterations} are stopped when $ \norm{\xvec^{\mvec{g}^{k+1}} - \xvec^{\mvec{g}^{k}}} < \gamma_2$, where $ \gamma_1>0 $ and $ \gamma_2>0 $ are preset tolerances of a small magnitude.

%The mean value condition is equivalent to specifying that the linear system for pressure has a non-trivial null space of constant vectors. Since the null space is known for the pressure rows, this information can be given to \petsc{}. While solving the linear system using Krylov methods such as GMRES, \petsc{} only constructs the basis of the column space of $ \mvec{A_g} $ that are orthogonal to the constant pressure vector, thereby finding a unique solution.

%Since the mean-value of the pressure in $ Q $ can be translated without affecting the Navier-Stokes equations \eqref{eq:ns-original}, thus an equivalent way of applying the constraint on pressure is to pick a node in the finite element discretization and apply a Dirichlet condition only on that node. Such application of Dirichlet condition on a node (which is of measure zero), helps ensure the uniqueness of an algebraic solution without affecting the FEM formulation. The actual boundary conditions to be applied for pressure will still vary from one problem to another. We discuss them in the context of each examples provided in Sec. \secref{sec:num-examples-results}.

%The present methodology was implemented through our in-house scalable parallel finite-element analysis software written in C++. It is optimized for distributed memory computing. This program in turn uses PETSc for the parallel matrix and vector data structures as well as the linear algebra routines. The spacetime formulation results in a system of equation that is not symmetric. Thus Krylov methods such as conjugate gradients and biconjugate gradient methods do not provide good parallel performance. GMRES works very well, especially with preconditioners such as block Jacobi, generalized ASM as well as SOR type and algebraic multigrid type preconditioners. Multigrid preconditioners provide marginal advantage in solve time but has a higher memory requirement. We found out that the SOR preconditioner and the block Jacobi preconditioners provided by PETSc works the reasonably well for this problem. In this work, we performed the convergence studies we have used both these preconditioners. In the larger runs, we used SOR since we found that it gives better scalability.

%\section{Additional results}
%%\subsection{Auxiliary proofs}
%\begin{lemma} \label{thm:final-time-laplacian}
%	\begin{align}
%	\innerFTh{\taum \visco \laplacian \uvech}{\uvech} \geq \taumMax \visco \innerFTh{\laplacian \uvech}{\uvech}.
%	\end{align}
%\end{lemma}
%\begin{proof}
%	Say $ z_1 = \innerFTh{\taum \visco \laplacian \uvech}{\uvech} $ and $ z_2 = \taumMax \visco \innerFTh{\laplacian \uvech}{\uvech} $. Then we have
%	\begin{align}
%	z_1 - z_2 &= \innerFTh{-[\taumMax - \taum^e] \laplacian \uvech}{\uvech} \\
%	&= \elmsumFT \visco \left[ \left\{ (\taumMax - \taum^e) \normElm{\grad\uvech}^2 - (\taumMax - \taum^e) \inner{\ddiv{\normalvec} \uvech}{\uvech}_e \right\} \right] \\
%	&\geq \elmsumFT \visco (\taumMax - \taum^e) \left[ \normElm{\grad\uvech}^2 - \left\{ \frac{\zeta}{2} \norm{\ddiv{\normalvec}\uvech}_{\partial e}^2 + \oneOver{2\zeta}\norm{\uvech}_{\partial e}^2 \right\} \right] \\
%	&\geq \elmsumFT \visco (\taumMax - \taum^e) \left[ \oneOver{C_{\partial e}^2} \norm{\grad \uvech}_{\partial e}^2 -\half \left\{ \zeta + \frac{\cinv}{\zeta} \right\} \norm{\grad\uvech}_{\partial e}^2 \right] \\
%	&= 	\elmsumFT \visco (\taumMax - \taum^e) \left[ \oneOver{C_{\partial e}^2} - \half \left( \zeta + \frac{\cinv}{\zeta} \right) \right] \norm{\grad\uvech}_{\partial e}^2
%	\end{align}
%The last expression is positive if
%\begin{align}
%	\oneOver{C_{\partial e}^2} - \left( \zeta + \frac{\cinv}{\zeta} \right) \geq 0 \implies \zeta^2 C_{\partial e}^2 -2\zeta + \cinv C_{\partial e}^2 \leq 0 \implies \zeta (\zeta C_{\partial e}^2 - 2) \leq -\cinv C_{\partial e}^2.
%\end{align}
%Since $ \cinv,\ C_{\partial e} $, and $ \zeta $ are positive, we can choose $ \zeta $ satisfying
%\begin{align}
%	\zeta C_{\partial e} - 2 \leq 0 \implies \zeta \leq \frac{2}{C_{\partial e}}.
%\end{align}
%\end{proof}

==> auxiliary/gory_details.tex <==
\section{The Nonlinear Term}
\subsection{The Trilinear Form}
\begin{itemize}
    \item The trilinear form:
    \begin{itemize}
    \item[*] {\color{black} $\avec$ = convection field}, {\color{blue} $\uvec = $ the solution field}, {\color{red} $\vvec = $ the test function}
    \item[*] %$\inner{(\uvec\cdot\grad){\color{blue}\vvec}}{\color{red}\wvec}$
    \end{itemize}
    \begin{align}
    \mvec{n} ({\avec}; {\color{blue}\uvec}, {\color{red}\vvec}) = \mvec{n} ({\avec}, {\color{blue}\uvec}, {\color{red}\vvec}) = 
        \begin{cases}
            \inner{(\avec\cdot\grad){\color{blue}\uvec}}{{\color{red}\vvec}} \\
            \inner{\grad\cdot({\color{blue}\uvec}\avec^T)}{{\color{red}\vvec}} \ [\text{assuming } (\divergence\avec = 0)]
        \end{cases}
    \end{align}
\end{itemize}
\subsection{Identities}
\begin{itemize}
    \item Gradient tensor:
    \begin{align}
        (\grad\vvec)_{ij} = 
        \begin{bmatrix}
    	   \grad v_1 \\ \grad v_2 \\ \grad v_3
    	\end{bmatrix}
     =
    \begin{bmatrix}
    	  v_{1,1} & v_{1,2} & v_{1,3} \\
        v_{2,1} & v_{2,2} & v_{2,3} \\
        v_{3,1} & v_{3,2} & v_{3,3}
    \end{bmatrix}
        = \partial_j v_i = \partialder{v_i}{x_j}, \ i,j = 1, 2,3
    \end{align}
    \item Divergence of a tensor $\mathbb{A}$
    \begin{align}
        \divergence\mathbb{A} = 
        \begin{bmatrix}
    	   \divergence(\text{row1})\\ \divergence(\text{row2})\\ \divergence(\text{row3})
    	\end{bmatrix} = \partial_j \mathbb{A}_{ij}
    \end{align}
    \item $\divergence(\uvec\avec^T) = (\divergence \avec)\uvec + (\ddiv{\avec})\uvec$
    \begin{itemize}
    	\item[*] \textit{Proof:} 
    	\begin{align}
    		\divergence(\uvec\avec^T) &=
    		\begin{bmatrix}
    			\divergence(u_1 \avec^T)\\ \divergence(u_2 \avec^T)\\ \divergence(u_3\avec^T)
    		\end{bmatrix}
    		=
    		\begin{bmatrix}
    			u_1(\divergence\avec)\\ u_2(\divergence\avec)\\ u_3(\divergence\avec)
    		\end{bmatrix}
    		+
    		\begin{bmatrix}
    			(\ddiv{\avec})u_1 \\ (\ddiv{\avec})u_2 \\ (\ddiv{\avec})u_3
    		\end{bmatrix}
    		= (\divergence\avec)\uvec + (\ddiv{\avec})\uvec
    	\end{align}
    \end{itemize}
    \item $\grad\cdot(\uvec\avec^T) = (\uvec\cdot\grad)\avec$ [when $\divergence\avec = 0$]
    \begin{itemize}
    	\item[*] \textit{Proof}:
    	\begin{align}
    		\grad\cdot(\uvec\avec^T) = \partial_j (u_i a_j) = \partialder{u_i}{x_j}a_j + u_i\partialder{a_j}{x_j} = a_j \partialder{u_i}{x_j} + 0 = (\ddiv{\avec})\uvec
    	\end{align}
    \end{itemize}
    \item Let $u, v, w \in H^1(\Omega)$, then
    \begin{align}
    	\inner{(\avecdiv)\uvec}{\vvec} &= \inner{\divergence(\uvec\avec^T)}{\vvec} - \inner{(\divergence\avec)\uvec}{\vvec} \\
    	\inner{(\avecdiv)\uvec}{\vvec} &= \inner{\avec}{\grad(\uvec\cdot\vvec)} - \inner{(\avecdiv)\vvec}{\uvec} \\
    	\inner{(\avecdiv)\uvec}{\vvec} &= \inner{(\grad\uvec)^T \vvec}{\avec} \\
    	\inner{(\avecdiv)\uvec}{\vvec} &= \int_{\partial\Omega}(\avec\cdot\normalvec)(\uvec\cdot\vvec)ds - \inner{\divergence\avec}{\uvec\cdot\vvec} - \inner{(\avecdiv)\vvec}{\uvec}
    \end{align}
    \item 
    \begin{align}
    	\inner{\divergence(\uvec\avec^T)}{\vvec} &= \inner{\partial_j (u_i a_j)}{v_i} \\
    	&= -\inner{u_i a_j}{\partial_j v_i} + \inner{u_i a_j} {n_j v_i}_{\partial U} \\
    	&= I + BC
    \end{align}
    \item
    \begin{align}
    	I
    	&= -\inner{u_i a_j}{\partial_j v_i} \\
    	&= -\inner{u_i}{a_j\partial_j v_i} \\
    	&= -\inner{\uvec}{\mmat{G}\avec}, \ [\text{where } \mmat{G} = (\grad\vvec)] \\
    	&=\begin{cases}
    		-\int_{\Omega} \uvec^T\mmat{G}\avec = -\inner{\uvec^T\mmat{G}}{\avec} \\
    		-\int_{\Omega} \avec^T\mmat{G}^T\uvec = -\inner{\avec^T\mmat{G}^T}{\uvec}   
    	\end{cases} \\
    \end{align}
    \item
    \begin{align}
    	\nvec(\avec,\uvec,\vvec)
    	&= \inner{\grad\cdot(\uvec\avec^T)}{\vvec} \\
    	&= -\inner{\uvec\avec^T}{\grad\vvec} + \inner{\normalvec\cdot(\uvec\avec^T)}{\vvec} \\
    	&= -\inner{(\avecdiv)\vvec}{\uvec} + \inner{\normalvec\cdot(\uvec\avec^T)}{\vvec} \\
    	&= -\inner{\uvec^T(\grad\vvec)}{\avec} + \inner{\normalvec\cdot(\uvec\avec^T)}{\vvec}
    \end{align}
\end{itemize}

\subsection{Advection Operators}
\begin{itemize}
	\item Consider the advection operator
	\begin{align}
		\opLAdv[a] \equiv (\avecdiv) + \half (\divergence \avec)
	\end{align}
	\item Then
	\begin{align}
		\inner{\opLAdv[a] \uvec}{\vvec} 
		&= \inner{\left[(\avecdiv)\uvec + \half (\divergence \avec)\uvec\right]}{\vvec} \\
		&= \inner{\left[(\avecdiv)\uvec + (\divergence \avec)\uvec\right]}{\vvec} - \half \inner{(\divergence \avec)\uvec}{\vvec} \\
		&= \inner{\divergence (\uvec \avec^T)}{\vvec} - \half \inner{(\divergence \avec)\uvec}{\vvec} \\
		&= -\inner{(\avecdiv)\vvec}{\uvec} + \inner{\normalvec\cdot(\uvec\avec^T)}{\vvec}_{\partial \Omega}  - \half \inner{(\divergence \avec)\uvec}{\vvec}\\
		&= -\inner{(\avecdiv)\vvec}{\uvec} - \half \inner{(\divergence \avec)\vvec}{\uvec} + (Boundary-terms) \\
		&= \inner{-\left[ (\avecdiv)\vvec + \half (\divergence \avec)\vvec \right]}{\uvec} + (B.T.) \\
		&= \inner{\uvec}{-\left[ (\avecdiv)\vvec + \half (\divergence \avec)\vvec \right]} + (B.T.) \\
		&= \inner{\uvec}{\opLAdvStar[a] \vvec} + (B.T.)
	\end{align}
	\item Thus
	\begin{align}
		\opLAdvStar[a] \equiv -\opLAdv[a]
	\end{align}
\end{itemize}

\clearpage
\section{Linearized Navier-Stokes}
\subsection{Operator view}
We define the following functions variables:
\begin{subequations}
	\begin{align}
	x &:= (u,p) \quad \text{(trial functions)} \\
	y &:= (v,q) \quad \text{(test functions)} \\
	z &:= (w,r) \quad \text{(special trial functions)}
	\end{align}
\end{subequations}
The function $ z $ will be mostly used for $ z = x_1 - x_2 $.

We define the following operators and their adjoint operators:
\begin{subequations}
	\begin{align}
		\opLAdv[a]u &:= (\adiv) u + \halfnice (\divergence a) u \\
		\opLTAdv[a]u &:= (\ut + \opLAdv[a]u) \\
		&\ = \ut + (\adiv) u + \halfnice (\divergence a) u
	\end{align}
\end{subequations}
And the adjoint operators
\begin{subequations}
	\begin{align}
	\opLAdvStar[a]v &= -\opLAdv[a]v \\
	\opLTAdvStar[a]v &= -\opLTAdv[a]v
	\end{align}
\end{subequations}
\begin{subequations}
	\begin{align}
	\opLOne[a] u &:= u_{,t} + (\adiv) u + \halfnice (\divergence a) u - \visco \laplacian u \\
	\opLOneStar[a] v &= -v_{,t} - (\adiv) v - \halfnice (\divergence a) v - \visco \laplacian v	
	\end{align}
\end{subequations}
\begin{subequations}
	\begin{align}
		\opLTwo u &:= - \divergence u \\ % \quad (\implies -\opLTwo u := \divergence u) \\
		\opLTwoStar q &:= \grad q
	\end{align}
\end{subequations}

We also define
\begin{subequations}
	\begin{align}
	\opLm[a] x = \opLOne[a](u,p) &:= \opLOne[a] u + \opLTwoStar p \\
	\opLc x = \opLc(u,p) &:= -\opLTwo u \\
	\opLn[a] y = \opLn[a](v,q) &:= \opLOneStar[a] v - \opLTwoStar q
	\end{align}
\end{subequations}
Then the Navier-Stokes equations become:
\begin{subequations}
	\begin{align}
	\opLm[a](u,p) &= f \qquad \implies &\opLOne[a] u + \opLTwoStar p &= f \\
	\opLc(u,p) &=0 \qquad \implies  &-\opLTwo u &= 0 
	\end{align}
\end{subequations}
Assume $ \delta a_{12} = a_1-a_2 $. Then note that,
\begin{subequations}
	\begin{align}
		\opLAdv[a_1]u - \opLAdv[a_2]u &= (\delta a_{12} \cdot\grad) u + \halfnice (\divergence \delta a_{12}) u \\
		&= \opLAdv[\delta a_{12}] u,\\
		\opLAdvStar[a_1]v - \opLAdvStar[a_2] v
		&= -\opLAdv[\delta a_{12}]v \\
		&= \opLAdv[\delta a_{21}]v \\
		\opLOne[a_1] - \opLOne[a_2] &= \opLAdv[\delta a_{12}] \\
		\opLOneStar[a_1] - \opLOneStar[a_2] &= \opLAdv[\delta a_{21}]
	\end{align}
\end{subequations}
Then we have
\begin{subequations}
	\begin{align}
		[\opLm[a_1] - \opLm[a_2]] = [\opLOne[a_1] - \opLOne[a_2]] = [\opLAdv[a_1] - \opLAdv[a_2]] = \opLAdv[\delta a_{12}] \\
		[\opLn[a_1] - \opLn[a_2]] = [\opLOneStar[a_1] - \opLOneStar[a_2]] = [\opLAdvStar[a_1] - \opLAdvStar[a_2]] = \opLAdv[\delta a_{21}]
	\end{align}
\end{subequations}

The unstabilized bilinear form is
\begin{align}
\bformUnstab(a; y, \xc) &= \inner{y}{\opLm[a] \xc} \\
&= \inner{v}{[\opLOne[a]\uc + \opLTwoStar \pc]} + \inner{q}{[-\opLTwo \uc]} \\
&= \inner{v}{\partial_t \uc} - \inner{\left[(\adiv)+\halfnice(\divergence a)\right]v}{\uc}+\visco\inner{\grad v}{\grad \uc}-\inner{\grad\cdot v}{\pc} + \inner{q}{\grad\cdot\uc} \\
&= -\inner{\partial_t v}{\uc} - \inner{\left[(\adiv)+\halfnice(\divergence a)\right]v}{\uc}+\visco\inner{\grad v}{\grad \uc}-\inner{\grad\cdot v}{\pc} + \inner{q}{\grad\cdot\uc} + \inner{v}{\uc}_{\bft}
\end{align}

Then we have
\begin{align}
\begin{split}
b(a; y, \xc) &= l(y),
\end{split}
\end{align}
where
\begin{subequations}
	\begin{align}
	b(a;y,\xc) &= \bformUnstab(a;y,\xc) + \sum_{K \in \mesh} \left[\inner{\opLn[a] y}{\uf}_{K} + \inner{\opLTwo v}{\pf}_K\right] + \sum_{e \in \bftmesh} \inner{v}{n_t \uf}_e \\
	l(y) &= \inner{v}{f}.
	\end{align}
\end{subequations}

If the fine scales are modeled using the coarse-scale residuals as
\begin{subequations}
	\begin{align}
	\uf &= -\taum^K [\opLOne[a]\uc + \opLTwoStar \pc - f] \ \text{in}\ K, \\
	\pf &= -\tauc^K [-\opLTwo \uc] \ \text{in}\ K,
	\end{align}
\end{subequations}
then we have
\begin{align}
\begin{split}
\bformh(a; y, \xc) &= \lformh(a;y),
\end{split}
\end{align}
where
\begin{subequations}
	\begin{align}
	\bformh(a;y,\xc) &= \bformUnstab(a;y,\xc) - \big[\sum_{K \in \mesh} \inner{\opLn[a] y}{\taum^K \opLm[a]\xc}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K \opLm[a]\xc}_e \big] + \sum_{K \in \mesh} \inner{\opLTwo v}{\tauc^K \opLTwo \uc}_K\\
	\lformh(a;y) &= l(y) - \big[\sum_{K \in \mesh} \inner{\opLn[a] y}{\taum^K f}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K f}_e \big]
	\end{align}
\end{subequations}

\subsection{Continuity / Uniqueness}
For $ x_1 = (u_1,p_1) $ and $ x_2 = (u_2, p_2) $, we have
\begin{subequations}
	\begin{align}
	\bformh(a_1;y,\xc_1) &= \bformUnstab(a_1;y,\xc_1) - \big[\sum_{K \in \mesh} \inner{\opLn[a_1] y}{\taum^K \opLm[a_1]\xc_1}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K \opLm[a]\xc_1}_e \big] + \sum_{K \in \mesh} \inner{\opLTwo v}{\tauc^K \opLTwo \uc_1}_K\\
	\lformh(a_1;y) &= l(y) - \big[\sum_{K \in \mesh} \inner{\opLn[a_1] y}{\taum^K f}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K f}_e \big]
	\end{align}
\end{subequations}

\begin{subequations}
	\begin{align}
	\bformh(a_2;y,\xc_2) &= \bformUnstab(a_2;y,\xc_2) - \big[\sum_{K \in \mesh} \inner{\opLn[a_2] y}{\taum^K \opLm[a_2]\xc_2}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K \opLm[a]\xc_2}_e \big] + \sum_{K \in \mesh} \inner{\opLTwo v}{\tauc^K \opLTwo \uc_2}_K\\
	\lformh(a_2;y) &= l(y) - \big[\sum_{K \in \mesh} \inner{\opLn[a_2] y}{\taum^K f}_{K} + \sum_{e \in \bftmesh} \inner{v}{n_t \taum^K f}_e \big]
	\end{align}
\end{subequations}

Then
\begin{subequations}
	\begin{align}
	\bformh(a_1;y,\xc_1) - \bformh(a_2;y,\xc_2)
	&= \lformh(a_1;y) - \lformh(a_2;y) \\
	&= \sum_{K}\inner{\opLn[a_2]y - \opLn[a_1]y}{\taum^K f}_K \\
	&= \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f} \\
	\implies \bformh(a_1;y,\xc_1) &= \bformh(a_2;y,\xc_2) + \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f}
	\end{align}
\end{subequations}

Now,
\begin{subequations}
	\begin{align}
	\bform(a_1; y, x_1-x_2)
	&= \bform(a_1; y,x_1) - \bform(a_1; y, x_2) \\
	&= \left[\bformh(a_2;y,\xc_2) + \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f}\right] - \bform(a_1; y, x_2) \\
	&= \left[\bformh(a_2;y,\xc_2) - \bform(a_1; y, x_2) \right] + \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f} \\
	&= \left[ \bformUnstab(a_2;y,\xc_2) - \bformUnstab(a_1;y,\xc_2) - \sum_{K}\inner{\left[\opLn[a_2] - \opLn[a_1]\right]}{\taum^K \opLm[a_2]\xc_2}_K \right] + \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f} \\
	&= \left[ \bformUnstab(a_2;y,\xc_2) - \bformUnstab(a_1;y,\xc_2) \right] - \sum_{K}\inner{\opLAdv[\delta a_{12}]}{\taum^K \opLm[a_2]\xc_2}_K + \sum_{K} \inner{\opLAdv[\delta a_{12}]}{\taum^K f} \\
	&= \inner{\opLAdv[\delta a_{12}]}{\uc_2} - \sum_{K}\inner{\opLAdv[\delta a_{12}]}{ \taum^K \left[f - \opLm[a_2]\xc_2\right]}_K \\
	&= \inner{\opLAdv[\delta a_{12}]}{\uc_2} + \sum_{K}\inner{\opLAdv[\delta a_{12}]}{\uc_2 '}_K
	\end{align}
\end{subequations}

\clearpage
\section{Linearized Navier-Stokes}
\subsection{Operator view}
We define the following functions variables: $ \psi $
\begin{subequations}
	\begin{align}
	\phi &:= (\uvec,p) \quad \text{(trial functions)} \\
	\psi &:= (\vvec,q) \quad \text{(test functions)} \\
	\omega &:= (\wvec,r) \quad \text{(special trial functions)}
	\end{align}
\end{subequations}
The function $ \omega $ will be mostly used for $ \omega = \phi_1 - \phi_2 $.

We define the following operators and their adjoint operators:
\begin{subequations}
	\begin{align}
	\opLAdv[\avec]\uvec &:= (\adiv) \uvec + \halfnice (\divergence \avec) \uvec \\
	\opLTAdv[\avec]\uvec &:= (\ut + \opLAdv[\avec]\uvec) \\
	&\ = \ut + (\adiv) \uvec + \halfnice (\divergence \avec) \uvec
	\end{align}
\end{subequations}
And the adjoint operators
\begin{subequations}
	\begin{align}
	\opLAdvStar[a]\vvec &= -\opLAdv[a]\vvec \\
	\opLTAdvStar[a]\vvec &= -\opLTAdv[a]\vvec.
	\end{align}
\end{subequations}
Note that,
\begin{align}
\opLTAdv[\avec^1]\uvec - \opLTAdv[\avec^2]\uvec &= (\ut + \opLAdv[\avec^1]\uvec) - (\ut + \opLAdv[\avec^2]\uvec) \\
&= \opLAdv[\avec^1]\uvec - \opLAdv[\avec^2]\uvec \\
&= (\ddiv{\avec^1}) \uvec + \halfnice (\divergence \avec^1) \uvec - (\ddiv{\avec^2}) \uvec - \halfnice (\divergence \avec^2) \uvec \\
&= (\ddiv{\delta \avec^{12}}) \uvec + \halfnice (\divergence \delta \avec^{12}) \uvec \\
&= \opLAdv[\delta \avec^{12}]
\end{align}

The unstabilized bilinear form is
\begin{align}
\bformUnstab(\avec;\phi,\psi) 
&= - \inner{\uvec}{\opLTAdv[\avec]\vvec}+\visco\inner{\grad \uvec}{\grad \vvec}-\inner{p}{\grad\cdot \vvec} + \inner{\grad\cdot\uvec}{q} + \inner{\uvec}{\vvec}_{\bft}.
\end{align}
Note that
\begin{align}
	\bformUnstab(\avec;\phi,\phi) = \halfnice \normFT{\uvec}^2 + \visco\norm{\grad \uvec}^2.
\end{align}

Now, assuming $ \phi = \upairc + \upairf $, we have
\begin{subequations}
	\begin{align}
	\bformUnstab(\avec;\phi,\psi) &= \bformUnstab(\avec;\upairc,\psi) - \innerh{\uf}{\opLTAdv[\avec]\vvec} - \innerh{\pf}{\divergence \vvec} - \innerh{\uf}{\grad q} + \innerFTh{\uf}{\vvec} \\
	&= \bformUnstab(\avec;\upairc,\psi) - \innerh{\uf}{[\opLTAdv[\avec]\vvec+\grad q]} - \innerh{\pf}{\divergence \vvec} + \innerFTh{\uf}{\vvec} 
	\end{align}
\end{subequations}
If the fine scales are modeled using the coarse-scale residuals as
\begin{subequations}
	\begin{align}
	\uf &= -\taum^K (\opLTAdv[\avec]\uc -\visco\laplacian\uc + \grad\pc - \fvec) \ \text{in}\ K, \\
	\pf &= -\tauc^K (\divergence\uc) \ \text{in}\ K,
	\end{align}
\end{subequations}
then we have
\begin{align}
\begin{split}
\bformh(\avec; \upairc, \vpair) &= \lformh(\avec;\psi) \quad \forall \vpair \in \spaceV \times Q,
\end{split}
\end{align}
where
\begin{align}
\begin{split}
    \bformh(\avec; \upairh,\vpairh) &= \bformUnstab(\avec; \upairh,\vpairh) + \innerh{\taum [\opLTAdv[\avec]\uvech-\visco\laplacian\uvech + \grad \ph ]}{[\opLTAdv[\avec]\vvech-\visco\laplacian\vvech +\grad \qh]} + \innerh{\tauc \divergence \uvech}{\divergence \vvech} \\
    &\quad -\innerFTh{\taum [\opLTAdv[\avec]\uvech-\visco\laplacian\uvech + \grad \ph ]}{\vvech}
\end{split}
 \\
\lformh(\avec; \vpairh) &= \inner{\fvec}{\vvech} + \innerh{\taum \fvec}{[\opLTAdv[\avec]\vvech-\visco\laplacian\vvech +\grad \qh]} - \innerFTh{\taum \fvec}{\vvech}
\end{align}

We define the discrete norm
\begin{align}
\vertiii{\uvech}^2 = \half\normFT{\uvech}^2 + \norm{\grad\uvech}^2 + \normh{\taum^{\halfnice}X(\uvech,\ph)}^2 + \normh{\tauc^{\halfnice}\divergence\uvech}^2
\end{align}

\subsection{Stability}
\begin{multline*}
\bformh(\avec; \upairh, \upairh) = \halfnice \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\normh{\taum^{\halfnice}\visco \laplacian \uvech}^2 \\
+ \normh{\tauc^{\halfnice}\divergence\uvech}^2 -\innerFTh{\taum [\opLTAdv[\avec]\uvech + \grad \ph ]}{\uvech} + \innerFTh{\taum\visco\laplacian\uvech}{\uvech}
\end{multline*}
Using Cauchy's inequality with $ \epsilon $ for any $ x $ and $ y $,
\begin{align}
-2ab \geq -\oneOver{\epsilon}a^2 - \epsilon b^2,\ \epsilon > 0,
\end{align}
%the fourth term can be estimated as
%\begin{align*}
%-\innerh{\taum \visco\laplacian\uvech}{[\opLTAdv[\avec]\uvech + \grad \ph ]} &\geq -\oneOver{\epsilon}\normh{\taum^{\halfnice}\visco\laplacian\uvech}^2 - \epsilon\normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 \\
%&\geq -\frac{\visco^2 \cinv^2}{\epsilon} \normh{\taum^{\halfnice} h^{-1}\grad\uvech}^2 - \epsilon\normh{\taum^{\halfnice} [\opLTAdv[\avec]\uvech + \grad \ph ]}^2.
%\end{align*}
the sixth term can be estimated as
\begin{flalign}
&-\innerFTh{\taum [\opLTAdv[\avec]\uvech -\visco\laplacian\uvech + \grad \ph ]}{\uvech} \\
&\quad = -\innerFTh{\taum [\opLTAdv[\avec]\uvech + \grad \ph ]}{\uvech} + \innerFTh{\taum\visco\laplacian\uvech}{\uvech} \\
&\quad \geq -\frac{\epsilon}{2}\normFTh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\uvech}^2,
\end{flalign}
and the seventh term as
\begin{align}
\innerFTh{\taum\visco\laplacian\uvech}{\uvech} \geq - \taumMax\visco \innerFTh{\grad \uvech}{\grad \uvech} + \taumMax\inner{\uvech}{\ddiv{\normalvec}\uvech}_{\partial \spatialD} = -\taumMax\visco \normFTh{\grad \uvech}^2.
\end{align}
Combining,
\begin{align*}
    \bformh(\avec; \upairh, \upairh) &\geq \half \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\normh{\taum^{\halfnice}\visco \laplacian \uvech}^2 + \normh{\tauc^{\halfnice}\divergence\uvech}^2 \\
    &\hspace{8em} -\frac{\epsilon}{2}\normFTh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\uvech}^2 -\taumMax\visco \normFTh{\grad \uvech}^2 \\
    &\geq \half \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\frac{\visco^2 \cinv^2}{h^2}\normh{\taum^{\halfnice}\visco \grad \uvech}^2 + \normh{\tauc^{\halfnice}\divergence\uvech}^2 \\
    &\hspace{8em} -\frac{\epsilon\traceConstant}{2}\normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\uvech}^2 -\frac{\taumMax\visco \cinv^2}{h^2} \normFTh{\uvech}^2 \\
    &= \Xsum_{\elemVol\in\mesh}\left[ \left( 1 - \frac{\taum^e \visco \cinv^2}{h^2}\right) \visco \norm{\grad \uvech}_{\elemVol}^2 + \left(1-\frac{\epsilon\traceConstant}{2}\right) \norm{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}_{\elemVol}^2 + \norm{\tauc^{\halfnice}\divergence\uvech}_{\elemVol}^2 \right] \\
    &\quad +\Xsum_{\elemFT\in\bftmesh} \left[ \left( \half -\oneOver{2\epsilon} -\frac{\taumMax\visco\cinv^2}{h^2} \right) \norm{\uvech}_{\elemFT}^2 \right].
\end{align*}
Each of the quantities in the parentheses must be positive, i.e.,
\begin{align}
    1 - \frac{\taum^e \visco \cinv^2}{h^2} > 0 &\implies \taum^e < \frac{h^2}{\visco \cinv^2}, \\
    1-\frac{\epsilon\traceConstant}{2} >0 &\implies \epsilon < \frac{2}{\traceConstant}, \\
    \text{and}\ \half -\oneOver{2\epsilon} -\frac{\taumMax\visco\cinv^2}{h^2} >0 &\implies \taumMax < \left(1-\oneOver{\epsilon}\right)\frac{h^2}{2\visco\cinv^2}.
\end{align}
So, we must have respectively $\epsilon > 1$, and $\epsilon < \nicefrac{2}{\traceConstant}$, i.e., $ 1 < \epsilon < \nicefrac{2}{\traceConstant} $.

The right hand side,
\begin{align}
\lformh(\avec; \upairh) &= \inner{\fvec}{\uvech} + \innerh{\taum \fvec}{[\opLTAdv[\avec]\uvech-\visco\laplacian\uvech +\grad \ph]} - \innerFTh{\taum \fvec}{\uvech} \\
&\leq \norm{\fvec}\norm{\uvech} + \normh{\taum^{\halfnice}\fvec} \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech -\visco\laplacian\uvech +\grad \ph]} + \normh{\taum^{\halfnice} \fvec} \normh{\taum^{\halfnice}\uvech} \\
&\leq \norm{\oneOver{\visco} \fvec}\norm{\visco \grad \uvech} + \normh{\taum^{\halfnice}\fvec} \left(\normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech +\grad \ph]} + \visco \normh{\taum^{\halfnice} \laplacian\uvech} \right) + \normFTh{\taum^{\halfnice} \fvec} \normFTh{\taum^{\halfnice}\uvech} \\
&\leq \left[\norm{\visco^{-1}\fvec}^2 + 2\normh{\taum^{\halfnice}\fvec}^2 + \normFTh{\taum^{\halfnice}\fvec}^2\right]^{\halfnice} \\
&\qquad \times \left[\visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech +\grad \ph]}^2 + \visco \normh{\taum^{\halfnice} \laplacian\uvech}^2 + \normFTh{\taum^{\halfnice}\uvech}^2 \right]^{\halfnice}
\end{align}

\subsection{Continuity of operator}
\begin{align}
\bformh(\avec_i; {\upairh}_i, \vpairh) &= \lformh({\upairh}_i,\vpairh) \ \ \forall \vpairh \in \spaceVh \times \spaceQh, \quad i=1,2
\end{align}

\begin{align}
\bformh(\avec^1; \uvech^1, \vvech) - \bformh(\avec^2; \uvech^2, \vvech) &= \lformh(\avec^1, \vpairh) - \lformh(\avec^2, \vpairh) \\
&= \innerh{\taum \fvec}{(\opLTAdv[\avec^1]\vvech - \opLTAdv[\avec^2]\vvech)} \\
\implies \bformh(\avec^1; \uvech^1, \vvech) &= \bformh(\avec^2; \uvech^2, \vvech) + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech}
\end{align}

Now,
\begin{align}
\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &= \bformh(\avec^1; \uvech^1, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) \\
&= \bformh(\avec^2; \uvech^2, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech} \\
&= -\inner{\uvech^2}{(\opLTAdv[\avec^2]-\opLTAdv[\avec^1])\vvech} \\
&\quad + \innerh{\taum [\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 + \grad \ph^2 ]}{[\opLTAdv[\avec^2]\vvech^2-\visco\laplacian\vvech^2 +\grad \qh^2]} \\
&\quad- \innerh{\taum [\opLTAdv[\avec^1]\uvech^2-\visco\laplacian\uvech^2 + \grad \ph^2 ]}{[\opLTAdv[\avec^1]\vvech^2-\visco\laplacian\vvech^2 +\grad \qh^2]} \\
&\quad -\innerFTh{\taum (\opLTAdv[\avec^2]\uvech - \opLTAdv[\avec^1] \uvech)}{\vvech} \\
&\quad + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech} \\
&= -\inner{\uvech^2}{\opLTAdv[\delta \avec^{21}]\vvech} \\
&\quad + \innerh{\taum \opLTAdv[\delta \avec^{21}]\uvech^2}{[\opLTAdv[\avec^1]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
&\quad + \innerh{\taum ([\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \qh^2]}{\opLTAdv[\delta \avec^{21}] \vvech} \\
&\quad -\innerFTh{\taum \opLTAdv[\delta \avec^{21}]\uvech^2}{\vvech} \\
&\quad - \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{21}]\vvech}
\end{align}

\begin{align}
\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &= \bformh(\avec^1; \uvech^1, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) \\
&= -\inner{\uvech^2}{\opLAdv[\delta \avec^{21}]\vvech} \\
&\quad + \innerh{\taum \opLAdv[\delta \avec^{21}]\uvech^2}{[\opLTAdv[\avec^1]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
&\quad + \innerh{\taum ([\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \qh^2]}{\opLAdv[\delta \avec^{21}] \vvech} \\
&\quad -\innerFTh{\taum \opLAdv[\delta \avec^{21}]\uvech^2}{\vvech} \\
&\quad - \innerh{\taum \fvec}{\opLAdv[\delta \avec^{21}]\vvech} \\
&=: S_1 + S_2 + S_3 + S_4 + S_5
\end{align}

\begin{align}
|S_5| \leq \norm{\taum f}_{L^2}\norm{\delta \avec^{21}}_{L^{\infty}}\norm{\grad \vvech}_{L^2}
\end{align}
by the discrete inverse inequality and Poincare's inequality, we have
\begin{align}
\norm{\davec}_{L^{\infty}} &\leq Ch^{-\xi} \norm{\davec}_{L^2} \\
&\leq Ch^{-\xi} \norm{\grad \davec}_{L^2}
\end{align}
where $ \xi = -1,-\halfnice $ for $ n=2,3 $ respectively. Therefore
\begin{align}
	\seminorm{S_5} \leq \cinv h^{-\xi} \norm{\taum f}_{L^2}\norm{\grad \delta \avec^{21}}_{L^2}\norm{\grad \vvech}_{L^2}
\end{align}
\begin{align}
\seminorm{S_1} \leq \beta R\norm{\grad \davec}_{L^2}\norm{\grad \vvech}_{L^2}
\end{align}
\begin{align}
\seminorm{S_2} &\leq \cinv h^{-\xi}\taumMax \norm{\grad \uvech^2}_{L^2} \norm{\grad \davec}_{L^2} \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} + \visco \normh{\grad \vvech}  \right) \\
&\leq \cinv h^{-\xi}\taumMax R \norm{\grad \davec}_{L^2} \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} + \visco \normh{\grad \vvech}  \right)
\end{align}
\begin{align}
\seminorm{S_3} &\leq \cinv h^{-\xi}\taumMax \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^2]\uvech^2 + \grad \qh^2]} + \visco \normh{\grad \uvech^2} \right) \norm{\grad \davec}_{L^2} \norm{\grad \vvech}_{L^2} \\
&\leq \cinv h^{-\xi}\taumMax R \norm{\grad \davec}_{L^2} \norm{\grad \vvech}_{L^2}
\end{align}
\begin{align}
\seminorm{S_4} &\leq \cinv h^{-\xi_b} \taumMax R \normFT{\grad \davec} \normFT{\grad \vvech} \\
&\leq \cinv^2 h^{-\xi_b-1} \taumMax R \norm{\grad \davec} \normFT{\vvech}
\end{align}
where we have used $ \normFT{\grad\davec} \leq C\norm{\grad\davec} $ and $ \normFT{\grad \vvech} \leq \frac{\cinv}{h}\normFT{\uvech}$.

Combining
\begin{align}
\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &\leq \Xsum_{i=1}^4 \seminorm{S_i} \\
&\leq \norm{\grad \davec} \Bigg[ C_1(R,h,\taumMax) \normFT{\vvech} + C_2(R,h,\taumMax) \norm{\grad\vvech} \\
&\qquad\qquad\qquad + C_3(R,h,\taumMax) \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} \Bigg] \\
&\leq \norm{\grad \davec} \left[C_1^2 + C_2^2 + C_3^2 \right]^{\halfnice} \left[\normFT{\vvech}^2 + \norm{\grad\vvech}^2 + \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]}^2 \right]^{\halfnice} \\
&=: \tilde{C} Z(\vpairh) \norm{\grad (\avec^1-\avec^2)}
\end{align}
where $ \tilde{C} = \left[C_1^2 + C_2^2 + C_3^2 \right]^{\halfnice} $ and $ Z(\vpairh) = Z((\vvech,\qh)) = \left[\normFT{\vvech}^2 + \norm{\grad\vvech}^2 + \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]}^2 \right]^{\halfnice} $.
Now, if we choose $ \vpairh = \upairh^1 - \upairh^2 $, then
\begin{align}
\bformh(\avec^1; \upairh^1-\upairh^2, \upairh^1-\upairh^2) &\leq \tilde{C}Z(\upairh^1-\upairh^2) \norm{\grad(\avec^1-\avec^2)}
\end{align}
We also have
\begin{align}
\bformh(\avec^1; \upairh^1-\upairh^2, \upairh^1-\upairh^2) \geq C_s Z(\upairh^1-\upairh^2)^2
\end{align}
Thus
\begin{align}
C_s Z(\upairh^1-\upairh^2)^2 &\leq \tilde{C}Z(\upairh^1-\upairh^2) \norm{\grad(\avec^1-\avec^2)} \\
Z(\upairh^1-\upairh^2) &\leq \left(\frac{\tilde{C}}{C_s}\right) \norm{\grad(\avec^1-\avec^2)}
\end{align}

\subsection{Uniqueness}
$ \eta = \upairh^1-\upairh^2 $
\begin{align}
\bformh(\uvec^1; \eta, \eta) &= \bformh(\uvec^1; \uvech^1, \wvech) - \bformh(\uvec^1; \uvech^2, \wvech) \\
&= -\inner{\uvech^2}{\opLAdv[\wvech]\wvech} \\
&\quad + \innerh{\taum \opLAdv[\wvech]\uvech^2}{[\opLTAdv[\uvec^1]\wvech-\visco\laplacian\wvech +\grad \rh]} \\
&\quad + \innerh{\taum ([\opLTAdv[\uvec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \rh^2]}{\opLAdv[\wvech] \wvech} \\
&\quad -\innerFTh{\taum \opLAdv[\wvech]\uvech^2}{\wvech} \\
&\quad - \innerh{\taum \fvec}{\opLAdv[\wvech]\wvech} \\
&=: T_1 + T_2 + T_3 + T_4 + T_5
\end{align}
\begin{align}
\seminorm{T_1} &\leq \beta R \norm{\grad \wvech}^2 \\
\seminorm{T_2} &\leq \cinv h^{-\xi} \taumMax R \left(\norm{\grad \wvech} \normh{\taum^{\halfnice}[\opLTAdv[\uvech^1]\wvech + \grad \rh]} + \visco\norm{\grad \wvech}^2\right) \\
&\leq \cinv h^{-\xi} \taumMax R \left[\left(\visco + \half\right) \norm{\grad \wvech}^2 + \half \normh{\taum^{\halfnice}[\opLTAdv[\uvech^1]\wvech + \grad \rh]}^2 \right] \\
\seminorm{T_3} &\leq \cinv h^{-\xi} \taumMax R \norm{\grad \wvech}^2 \\
\seminorm{T_4} &\leq \cinv h^{-\xi_b} \taumMax R \normFT{\grad \wvech}^2 \\ 
&\leq \cinv^2 h^{-\xi_b-1} \taumMax R \normFT{\wvech}^2 \\
\seminorm{T_5} &\leq \cinv h^{-\xi} \taumMax \norm{\fvec} \norm{\grad\wvech}^2
\end{align}
therefore,
\begin{align}
\lambda_1 \normFT{\wvech}^2
+\lambda_2 \normh{\taum^{\halfnice}\left[\opLTAdv[\uvech^1] \wvech + \grad \rh \right]}^2 + \lambda_3 \norm{\grad \wvech}^2 \leq 0
\end{align}
where
\begin{align}
\lambda_1 &= C_s - \cinv^2 h^{-\xi_b-1} \taumMax R \\
\lambda_2 &= C_s - \half \cinv^2 h^{-2\xi}  {\taumMax}^2 R^2 \\
\lambda_3 &= C_s - \left[\beta R + \cinv h^{-\xi}\taumMax \left\{R \left( \nicefrac{3}{2} + \visco \right) + \norm{\fvec} \right\} + \half \cinv^2 h^{-2\xi} {\taumMax}^2 R^2 \right]
\end{align}

\subsection{Convergence}
\begin{align*}
\bformh(\uvec; \hat{\eta}, \hat{\eta}) &= \bformh(\uvec; \upairh - \interp{\upair}, \hat{\eta}) \\
&= \bformh(\uvec; \upairh, \hat{\eta}) - \bformh(\uvec; \interp{\upair}, \hat{\eta}) \\
&= \bformh(\uvec; \upair, \hat{\eta}) - \bformh(\uvec; \interp{\upair}, \hat{\eta}) \\
&= -\inner{\uvec-\interp{\uvec}}{\opLTAdv[\uvec] \wvech} + \visco \inner{\grad (\uvec-\interp{\uvec})}{\grad \wvech} - \inner{p-\interp{p}}{\divergence\wvec} + \inner{\divergence (\eie{\uvec})}{\rh} \\
&\quad + \innerFT{\eie{\uvec}}{\wvech} + \innerh{\taum [\opLTAdv[\uvec] (\eie{\uvec}) -\visco \laplacian (\eie{\uvec}) + \grad (\eie{\uvec})] }{[\opLTAdv[\uvec]-\visco\laplacian\wvech + \grad\rh]} \\
&\quad \innerh{\tauc \divergence(\eie{\uvec})}{\divergence \wvech} - \innerFTh{\taum [\opLTAdv[\uvec](\eie{\uvec})-\visco\laplacian(\eie{\uvec})+\grad (\eie{p})]}{\wvech}
\end{align*}
\clearpage
\subsection{Stabilized method}
\begin{subequations}\label{eq:ns-linearized}
	\begin{align}
	\timeder{\uvec}+\divergence(\uvec\avec^T)-\visco\laplacian \uvec+\grad p - 
	\mvec{f} &= 0, \text{ }\tilde{\xvec}\in\Omega, \label{eq:ns-original-momentum}
	\\
	\grad\cdot\uvec &= 0, \text{ }\tilde{\xvec}\in\Omega, \label{eq:ns-original-continuity}
	\\
	\uvec &= \mvec{g}, \text{ }\tilde{\xvec}\in\Gamma_{S1}\subseteq\Gamma_{S}, \label{eq:ns-original-dirichlet}
	\\
	\mathscr{B}_{NR} \uvec &= h, \text{ }\tilde{\xvec}\in\Gamma_{S2}\subseteq\Gamma_{S}, \label{eq:ns-original-neumann}
	\\
	\uvec &= \uvec_0, \text{ }\xvec\in\Gamma_{0}, \label{eq:ns-original-ic}
	\end{align}
\end{subequations}

Find $ (\uvech,\ph)\in \mvec{V}^h\times Q^h $ for every $ (\vvec,q) \in \mvec{V}^h\times Q^h $, such that
\begin{align}\label{eq:fem-problem-vms}
B^h((\vvec, q), (\uvech, \ph)) - F^h((\vvec,\qh)) = \mvec{0},
\end{align}
where $ B^h $ and $ F^h $ are defined as
\begin{align}\label{eq:fem-problem-vms-bh-linear}
\begin{split}
B^h\Big((\vvec,q), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\vvec}{\timeder{\uvech}} 
	- \innerBig{(\ddiv{\avec})\vvec}{\uvech}+\visco\inner{\grad \vvec}{\grad 
		\uvech}-\inner{\grad\cdot\vvec}{\ph} + \inner{q}{\grad\cdot\uvech}}_{\text{original terms}} \\
&\quad-\underbrace{\inner{\timeder{\vvec}}{\uvec'}
	+\inner{\vvec}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}} \\
&\quad-\underbrace{\innerBig{(\ddiv{\avec})\vvec}{\uvec'}}_{\text{convective stab terms}}\\
&\quad+\underbrace{\tauc\inner{\grad\cdot\vvec}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad-\underbrace{\inner{\grad q}{\uvec'}}_{\text{PSPG}},
\end{split}\\
\label{eq:fem-problem-vms-fh}
F^h((\vvec,q)) = \inner{\vvec}{\mvec{f}}.
\end{align}
The bilinear form can be written as:
\begin{align}\label{eq:fem-problem-vms-bh-linear-2}
\begin{split}
B^h\Big(\avec;(\vvec,q), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\vvec}{\timeder{\uvech}} 
	- \innerBig{(\ddiv{\avec})\vvec}{\uvech}+\visco\inner{\grad \vvec}{\grad 
		\uvech}-\inner{\grad\cdot\vvec}{\ph} + \inner{q}{\grad\cdot\uvech}}_{\text{original terms}} \\
&\quad-\underbrace{\inner{\timeder{\vvec}}{\uvec'}
	+\inner{\vvec}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}} \\
&\quad-\underbrace{\innerBig{(\ddiv{\avec})\vvec}{\uvec'}}_{\text{convective stab terms}}\\
&\quad-\underbrace{\visco\innerBig{\laplacian\vvec}{\uvec'}}_{\text{viscous term}}\\
&\quad+\underbrace{\tauc\inner{\grad\cdot\vvec}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad-\underbrace{\inner{\grad q}{\uvec'}}_{\text{PSPG}},
\end{split} \\
\begin{split}
&=\underbrace{\inner{\vvec}{\timeder{\uvech}} 
	- \innerBig{(\ddiv{\avec})\vvec}{\uvech}+\visco\inner{\grad \vvec}{\grad 
		\uvech}-\inner{\grad\cdot\vvec}{\ph} + \inner{q}{\grad\cdot\uvech}}_{\text{original terms}} \\
&\quad+\underbrace{\inner{\vvec}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}} \\
&\quad+\underbrace{\innerBig{\left[-\timeder{\vvec}-(\ddiv{\avec})\vvec - \visco\laplacian\vvec- \grad q \right]}{\uvec'}}_{\text{stab terms}}\\
&\quad+\underbrace{\tauc\inner{\grad\cdot\vvec}{\grad\cdot\uvech}}_{\text{Grad-div term}}
\end{split}
\end{align}
\begin{align}
B^h\Big(\avec; (\vvec,q), (\uvech,\ph)\Big) \\ 
\begin{split}
&=\underbrace{\mathscr{A}\Big(\avec; (\vvec,q), (\uvech,\ph)\Big)}_{\text{original}} +\underbrace{\tauc\inner{\grad\cdot\vvec}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad+\underbrace{\innerBig{\mathcal{L}^*\vvec}{\uvec'}}_{\text{stab terms}} +\underbrace{\inner{\vvec}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}}, \\
\end{split}
\end{align}
where
\begin{align}
\mathcal{L}^*\vvec = \left[-\timeder{\vvec}-(\ddiv{\avec})\vvec - \visco\laplacian\vvec- \grad q \right]
\end{align}

\subsection{Coercivity}
\begin{align}\label{eq:fem-problem-vms-bh-linear-coercivity}
\begin{split}
B^h\Big(\avec;(\uvech,\ph), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\uvech}{\timeder{\uvech}} 
	- \innerBig{(\ddiv{\avec})\uvech}{\uvech}+\visco\inner{\grad \uvech}{\grad 
		\uvech}\cancel{-\inner{\grad\cdot\uvech}{\ph}} + \cancel{\inner{\ph}{\grad\cdot\uvech}}}_{\text{original terms}} \\
&\quad+\underbrace{\tauc\inner{\grad\cdot\uvech}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad+\underbrace{\innerBig{\mathcal{L}^*\uvech}{\uvec'}}_{\text{stab terms}} +\underbrace{\inner{\uvech}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}},
\end{split}
\end{align}

\begin{align}\label{eq:coercivity-1}
\begin{split}
B^h\Big(\avec;(\uvech,\ph), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\uvech}{\timeder{\uvech}} 
	- \innerBig{(\ddiv{\avec})\uvech}{\uvech}+\visco\inner{\grad \uvech}{\grad 
		\uvech}}_{\text{original terms}} +\underbrace{\tauc\inner{\grad\cdot\uvech}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad+\underbrace{\innerBig{\mathcal{L}^*\uvech}{\uvec'}}_{\text{stab terms}} +\underbrace{\inner{\uvech}{n_t \uvec'}_{\bft}}_{\text{temporal-stab terms}},
\end{split}
\end{align}

\begin{align}
\inner{\uvech}{\timeder{\uvech}} &= \int_{0}^{T}\int_{\spatialD} \uvech\timeder{\uvech}d\Omega = \half \int_{\spatialD} \int_{0}^{T} \timeder{} (\uvech)^2 dtd\spatialD = \half\left[\int_{\spatialD}(\uvech(\xvec,T))^2dD - \int_{\spatialD}(\uvech(\xvec,0))^2dD\right] \\
&= \half \left( \normL[2]{\uvech}{\spatialD}(T) - \normL[2]{\uvech}{\spatialD}(0) \right)
\end{align}

Now, using 
\begin{align}
\divergence(\uvec\avec^T) = (\divergence \avec)\uvec + (\ddiv{\avec})\uvec,
\end{align}
we have
\begin{align}
\inner{\divergence(\uvech\avec^T)}{\vvec} &= \inner{(\divergence \avec)\uvech + (\ddiv{\avec})\uvech}{\vvec} \\
&= \inner{(\divergence \avec)\uvech}{\vvec} +  \inner{(\ddiv{\avec})\uvech}{\vvec}.
\end{align}
On the other hand, using integration by parts,
\begin{align}
\inner{\divergence(\uvech\avec^T)}{\vvec} = -\inner{\uvech\avec^T}{\grad \vvec}n = -\inner{\uvech}{\avecdiv \vvec} = -\inner{\uvech}{(\avecdiv) \vvec}
\end{align}
So, we have,
\begin{align}
\inner{(\divergence \avec)\uvech}{\vvec} +  \inner{(\ddiv{\avec})\uvech}{\vvec} &= -\inner{\uvech}{(\avecdiv) \vvec} \\
\implies \inner{(\ddiv{\avec})\uvech}{\vvec} + \inner{\uvech}{(\avecdiv) \vvec} &= -\inner{(\divergence \avec)\uvech}{\vvec}
\end{align}
Substituting $ \vvec = \uvech $,
\begin{align}
2 \inner{(\divergence \avec)\uvech}{\uvech} &= -\inner{(\divergence \avec)\uvech}{\uvech} \\
\implies -\inner{(\divergence \avec)\uvech}{\uvech} &= \half\intOmega (\divergence \avec)(\uvech)^2 d\Omega \\
&\geq \half \alpha \normL{\uvech}{\Omega}^2
\end{align}

Stabilization  term
\begin{align}
\innerBig{\mathcal{L}^*\uvech}{\uvec'} &= \inner{-\left[ \timeder{\uvech} + (\ddiv{\avec}) \uvech + \visco \laplacian \uvech + \grad \ph \right]}{-\taum \resUvech} \\
&= \Xsum_{K\in\mesh} \inner{\left[\timeder{\uvech} + (\ddiv{\avec}) \uvech + \visco \laplacian \uvech + \grad \ph \right]}{\taum^K\left[\timeder{\uvech} + (\ddiv{\avec}) \uvech - \visco \laplacian \uvech + \grad \ph \right]}_K \\
&= \sum_{K\in\mesh}\int_K \taum^K \left(\left[\timeder{\uvech} + (\ddiv{\avec}) \uvech + \grad \ph \right]^2 - \visco^2(\laplacian \uvech)^2 \right)dK \\
&= \sum_{K\in\mesh}\taum^K \normL{\timeder{\uvech} + (\ddiv{\avec}) \uvech + \grad \ph}{K}^2 - \sum_{K\in\mesh}\taum^K\visco^2\normL[2]{\laplacian \uvech}{K}^2 \\
&\geq \sum_{K\in\mesh}\taum^K\normL{\timeder{\uvech} + (\ddiv{\avec}) \uvech + \grad \ph}{K}^2 - \sum_{K\in\mesh}\taum^K C_{I}h^{-2} \visco^2\normL[2]{\grad \uvech}{K}^2
\end{align}

For the boundary stabilization term, 
\begin{align}
\begin{split}
\inner{\uvech}{n_t \uvec'} &= \inner{\uvech}{\uvec'}_{\bft} - \cancel{\inner{\uvech}{\uvec'}_{\bit}} = -\taum \inner{\uvech}{\resUvech} \\
&= -\sum_{K\in\mesh_T}\taum^K \inner{\uvech}{\left[\timeder{\uvech} + (\ddiv{\avec}) \uvech - \visco \laplacian \uvech + \grad \ph \right]}_K \\
&= -\sum_{K\in\mesh_T}\taum^K \inner{\uvech}{\timeder{\uvech}}_{K}\Bigg|_{T} -\sum_{K\in\mesh_T}\taum^K \inner{\uvech}{(\ddiv{\avec}) \uvech}_{K}\Bigg|_{T} \\ &\quad +\sum_{K\in\mesh_T}\taum^K\inner{\uvech}{\visco \laplacian \uvech}_{K}\Bigg|_{T} -\sum_{K\in\mesh_T}\taum^K\inner{\uvech}{\grad \ph}_{K}\Bigg|_{T} \\
&\geq -C\sum_{K\in\mesh_T}\taum^K \normL{\uvech}{K}\normL{\timeder{\uvech}}{K} - C\sum_{K\in\mesh_T}\taum^K |\avec|_{\infty} \normL{\uvech}{K}\normL{\grad \uvech}{K} \\ 
&\quad - \sum_{K\in\mesh_T}\taum^K C_I h^{-2} \normL{\uvech}{K}^2- \sum_{K\in\mesh_T}\taum^K C\normL{\uvech}{K}\normL{\grad \ph}{K} \\
&\geq -\sum_{K\in\mesh_T}CC_I h^{-1}\taum^K \normL{\uvech}{K}^2 - \sum_{K\in\mesh_T}CC_Ih^{-1}\taum^K |\avec|_{\infty} \normL{\uvech}{K}^2 - \sum_{K\in\mesh_T}C_I \taum^K\visco h^{-2} \normL{\uvech}{K}^2 \\
&\quad - \sum_{K\in\mesh_T}C\taum^K \left(\frac{\normL{\uvech}{K^2}}{2} + \frac{\normL{\grad \ph}{K}}{2}\right) \\
& = \sum_{K\in\mesh_T} C(h)\taum^K \normL{\uvech}{K}^2 + \sum_{K\in\mesh_T} C(h)\taum^K \normL{\grad \ph}{K}^2
\end{split}
\end{align}
where we have used
\begin{align}
\sum_{K\in\mesh_T}\taum^K\inner{\uvech}{\visco \laplacian \uvech}_{K} &= -\sum_{K\in\mesh_T}\taum^K \inner{\grad \uvech}{\grad \uvech}_K\Bigg |_T + \sum_{K\in\mesh_T}\taum^K\visco \inner{\uvech}{\normalvec\cdot\grad \uvech}_K \Bigg |_T \\
&= -\sum_{K\in\mesh_T}\taum^K\normL{\grad\uvech}{K}^2 \geq \sum_{K\in\mesh_T}\taum^K C_I h^{-2} \normL{\uvech}{K}^2
\end{align}

Collating all terms, we have,
\begin{align}\label{eq:coercivity-2}
\begin{split}
B^h\Big(\avec;(\uvech,\ph), (\uvech,\ph)\Big) \\ 
&\geq\half \normL[2]{\uvech}{\spatialD}^2(T) + \half \alpha \normL{\uvech}{\Omega}^2 + \visco \normL[2]{\grad\uvech}{\Omega}^2 \\
&\quad +\sum_{K\in\mesh}\taum^K\normL{\timeder{\uvech} + (\ddiv{\avec}) \uvech + \grad \ph}{K}^2 - \sum_{K\in\mesh}\taum^K C_{I}h^{-2} \visco^2\normL[2]{\grad \uvech}{K}^2 \\
&\quad +\sum_{K\in\mesh_T} C(h)\taum^K \normL{\uvech}{K}^2 + \sum_{K\in\mesh_T} C(h)\taum^K \normL{\grad \ph}{K}^2
\end{split}
\end{align}

\section{Nonlinear form}
The modified FEM problem is then to find $ (\uvech,\ph)\in \mvec{V}^h\times Q^h $ for every $ (\wvech,\qh) \in \mvec{V}^h\times Q^h $, such that
\begin{align}\label{eq:fem-problem-vms}
B^h((\wvech, \qh), (\uvech, \ph)) - F^h((\wvech,\qh)) = \mvec{0},
\end{align}
where $ B^h $ and $ F^h $ are defined as
% \begin{align}\label{eq:fem-problem-vms-bh}
% \begin{split}
% B^h\Big((\wvech,\qh), (\uvech,\ph)\Big) \\ 
% &=\underbrace{\inner{\wvech}{\timeder{\uvech}} 
% 	+ \innerBig{\wvech}{(\uvech\cdot\grad)\uvech}+\visco\inner{\grad \wvech}{\grad 
% 		\uvech}-\inner{\grad\cdot\wvech}{p} + \inner{\qh}{\grad\cdot\uvech}}_{\text{original terms}} \\
% &\quad+\underbrace{\taum\inner{\timeder{\wvech}}{\resUvech}
% 	-\taum\inner{\wvech}{\resUvech}_{\bft}}_{\text{temporal-stabilization terms}} \\
% &\quad+\underbrace{\taum\Big(\grad\wvech,\resUvech\otimes\uvech\Big)-\taum\Big(\wvech, (\resUvech\cdot\grad) \uvech\Big)-\taum^2\Big(\grad\wvech,\resUvech\otimes\resUvech\Big)}_{\text{convective stabilization terms}}\\
% &\quad+\underbrace{\tauc\inner{\grad\cdot\wvech}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
% &\quad+\underbrace{\taum \inner{\grad\qh}{\resUvech}}_{\text{PSPG}},
% \end{split}\\
% \label{eq:fem-problem-vms-fh}
% F^h((\wvech,\qh)) = \inner{\wvech}{\mvec{f}}.
% \end{align}
\begin{align}\label{eq:fem-problem-vms-bh-2}
\begin{split}
B^h\Big((\wvech,\qh), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\wvech}{\timeder{\uvech}} 
	- \innerBig{\uvech\cdot\grad\wvech}{\uvech}+\visco\inner{\grad \wvech}{\grad 
		\uvech}-\inner{\grad\cdot\wvech}{p} + \inner{\qh}{\grad\cdot\uvech}}_{\text{original terms}} \\
&\quad-\underbrace{\inner{\timeder{\wvech}}{\uvec'}
	+\inner{\wvech}{n_t \uvec'}_{\bft}}_{\text{temporal-stabilization terms}} \\
&\quad-\underbrace{\Big(\uvech\cdot\grad\wvech,\uvec'\Big)-\Big(\uvec'\cdot\grad\wvech, \uvech\Big)-\Big(\uvec'\cdot\grad\wvech,\uvec'\Big)}_{\text{convective stabilization terms}}\\
&\quad+\underbrace{\tauc\inner{\grad\cdot\wvech}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad-\underbrace{\inner{\grad\qh}{\uvec'}}_{\text{PSPG}},
\end{split}\\
\label{eq:fem-problem-vms-fh}
F^h((\wvech,\qh)) = \inner{\wvech}{\mvec{f}}.
\end{align}
\begin{align}\label{eq:fem-problem-vms-bh-3}
\begin{split}
B^h\Big((\wvech,\qh), (\uvech,\ph)\Big) \\ 
&=\underbrace{\inner{\wvech}{\timeder{\uvech}} 
	- \innerBig{\uvech\cdot\grad\wvech}{\uvech}+\visco\inner{\grad \wvech}{\grad 
		\uvech}-\inner{\grad\cdot\wvech}{p} + \inner{\qh}{\grad\cdot\uvech}}_{\text{original terms}} \\
&\quad+\taum\underbrace{\inner{\timeder{\wvech}}{\resUvech}
	-\taum\inner{\wvech}{n_t \resUvech}_{\bft}}_{\text{temporal-stabilization terms}} \\
&\quad+\taum\underbrace{\Big(\uvech\cdot\grad\wvech,\resUvech\Big)+\taum\Big(\resUvech\cdot\grad\wvech, \uvech\Big)-\taum^2\Big(\resUvech\cdot\grad\wvech,\resUvech\Big)}_{\text{convective stabilization terms}}\\
&\quad+\underbrace{\tauc\inner{\grad\cdot\wvech}{\grad\cdot\uvech}}_{\text{Grad-div term}} \\
&\quad+\taum\underbrace{\inner{\grad\qh}{\resUvech}}_{\text{PSPG}},
\end{split}\\
\label{eq:fem-problem-vms-fh}
F^h((\wvech,\qh)) = \inner{\wvech}{\mvec{f}}.
\end{align}

==> data_files/FPC_study/St_table.tex <==
%\begin{table}[]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|c|}
%    \hline
%        Reynolds  &  100  &   200  &   300  &   400  &   500 \\
%        \hline
%        \hline
%        St        &  0.17172 & 0.19192 & 0.20202 & 0.21212 & 0.21212 \\
%        \hline
%        Cd mean   &  -1.3696 & -1.2395 & -1.213  & -1.2068 & -1.2092 \\
%        \hline
%    \end{tabular}
%    \caption{Strouhal number and drag force as function of Re}
%    \label{tab:fpc_st_table}
%\end{table}

\begin{table}[]
	\centering
	%\color{blue}{
	\csvreader[
	tabular=ccc,
	table head=\hline {$Re$} & {$C_d$} & {$St$} \\ 
	\hline
	\hline,
	late after last line=\\ \hline % horizontal line at the end of the table
	]{
		data_files/FPC_study/strouhal_data.txt
	}{}{\csvlinetotablerow}
	%}
	\caption{Mean drag force $ C_d $ and the Strouhal number ($ St $) 
	calculated for various Reynolds number}
	\label{tab:drag-strouhal-list}
\end{table}

==> sections/0_abstract.tex <==
%We solve fluid flow problems through a space-time finite element method. The weak form of the Navier-Stokes equations is stabilized using the variational multi-scale formulation. The finite element problem is posed on the ``full" space-time domain, considering time as another dimension. We provide a rigorous analysis of the stability and convergence of the stabilized formulation. We apply this method on two benchmark problems in computational fluid dynamics, namely, lid-driven cavity flow and flow past a circular cylinder. We validate the current method with existing results from literature and show that very large space-time blocks can be solved using our approach. %One challenge of this method is to come up with a good initial guess in space-time, which is non-trivial. We suggest various approaches including continuation methods and surrogates to circumvent this issue.
We present a space-time continuous-Galerkin finite element method for solving incompressible Navier-Stokes equations. To ensure stability of the discrete variational problem, we apply ideas from the variational multi-scale method. The finite element problem is posed on the ``full" space-time domain, considering time as another dimension. We provide a rigorous analysis of the stability and convergence of the stabilized formulation. And finally, we apply this method on two benchmark problems in computational fluid dynamics, namely, lid-driven cavity flow and flow past a circular cylinder. We validate the current method with existing results from literature and show that very large space-time blocks can be solved using our approach.

==> sections/1001_LDC_setup.tex <==
%\subsection{Problem setup for Lid driven cavity}


\begin{figure}[!tb]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{data_files/LDC_study/ldc_mesh_setup_c2-ver2.png}
    \caption{Space-time mesh with clustering in space dimensions}
    \label{fig:ldc_mesh_c2}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{data_files/LDC_study/ldc_mesh_setup_c3-ver2.png}
    \caption{Space-time mesh with clustering in space and time dimensions}
    \label{fig:ldc_mesh_c3}
    \end{minipage}
\end{figure}


==> sections/1002_LDC_benchmark_comparison_re1000.tex <==
\subsection{Lid driven cavity with Re=1000}

Table with PETSc options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 case name & ksp & prec & snes tol & ksp tol & add. opt. \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=180 & ibcgs & asm & atol 1e-8 rtol 1e-8 & default & -snes\_ksp\_ew \\ 
 \hline
 128x128x128,c,TFEM,t=180 & bcgsl & default & atol 1e-8 rtol 1e-8 & default & none \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
Table with configure.txt options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 case name & Lx,Ly,Lz & Nelemx,Nelemy,Nelemz & num of blocks \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=180 & 1,1,1 & 32,32,32 & 180 \\ 
 \hline
 128x128x128,c,TFEM,t=180 & 1,1,1 & 128,128,128 & 180 \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
where:
\begin{itemize}
\item[c] - means clustered grid in $x$ and $y$ direction
\item[TFEM] - means FEM in time formulation for Navier-Stokes equation with VMS stabilization
\item[t] - is a simulation time
\end{itemize}





%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		%title={Velocity in X direction along vertical line (Re=1000)},
%		%scale only axis,
%		%width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$y$},
%		ylabel={$u_x$},
%		legend pos=north west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers] 
%		table {data_files/LDC_study/Re-1000-32x32-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=180}}
%		
%		\addplot+ [no markers,]
%		table {data_files/LDC_study/Re-1000-128x128-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-1000-32x32-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=180}}
%		
%		\addplot+ [no markers,,dashed,thick] 
%		table {data_files/LDC_study/Re-1000-128x128-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=180}}
%		
%		\addplot [only marks,color = black,mark=x,] 
%		table [x index = 0, y index = 3] 
%		{data_files/LDC_study/ghia_vel_x.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-1000-ux}
%		%\subcaption{$Re=1000$, $u_x$}
%	\end{minipage}
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		%title={Velocity in Y direction along horizontal line (Re=1000)},
%		%scale only axis,
%		%width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$x$},
%		ylabel={$u_y$},
%		legend pos=south west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-1000-32x32-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=180}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-1000-128x128-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-1000-32x32-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-1000-128x128-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=180}}
%		
%		\addplot [only marks,color = black,mark=x,] 
%		table [x index = 0, y index = 3] 
%		{data_files/LDC_study/ghia_vel_y.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa 
%		%t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-1000-uy}
%		%\subcaption{$Re=1000$, $u_y$}
%	\end{minipage}	
%	\label{fig:ldc-re-1000}
%	\caption{LDC, Re1000}
%\end{figure}



==> sections/1003_LDC_benchmark_comparison_re3200.tex <==

\subsection{Lid driven cavity with Re=3200}

Table with PETSc options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 case name & ksp & prec & snes tol & ksp tol & add. opt. \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=180 & ibcgs & asm & atol 1e-8 rtol 1e-8 & default & -snes\_ksp\_ew \\ 
 \hline
 128x128x128,c,TFEM,t=180 & bcgsl & default & atol 1e-8 rtol 1e-8 & default & none \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
Table with configure.txt options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 case name & Lx,Ly,Lz & Nelemx,Nelemy,Nelemz & num of blocks \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=180 & 1,1,1 & 32,32,32 & 180 \\ 
 \hline
 128x128x128,c,TFEM,t=180 & 1,1,1 & 128,128,128 & 180 \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
where:
\begin{itemize}
\item[c] - means clustered grid in $x$ and $y$ direction
\item[TFEM] - means FEM in time formulation for Navier-Stokes equation with VMS stabilization
\item[t] - is a simulation time
\end{itemize}


%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in X direction along vertical line (Re=3200)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$y$},
%		ylabel={$vel\_x$},
%		legend pos=north west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-3200-32x32-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=180}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-3200-128x128-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-3200-32x32-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-3200-128x128-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=180}}
%		
%		\addplot [only marks,color = black,mark=x,] 
%		table [x index = 0, y index = 4] 
%		{data_files/LDC_study/ghia_vel_x.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-3200-ux}
%		%\subcaption{$Re=3200$, $u_x$}
%	\end{minipage}
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in Y direction along horizontal line (Re=3200)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$x$},
%		ylabel={$vel\_y$},
%		legend pos=south west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-3200-32x32-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=180}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-3200-128x128-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-3200-32x32-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=180}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-3200-128x128-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=180}}
%		
%		\addplot [only marks,color = black,mark=x,] 
%		table [x index = 0, y index = 4] 
%		{data_files/LDC_study/ghia_vel_y.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa 
%		%t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-3200-uy}
%		%\subcaption{$Re=3200$, $u_y$}
%	\end{minipage}	
%	\label{fig:ldc-re-3200}
%	\caption{LDC, Re=3200}
%\end{figure}

==> sections/1004_LDC_benchmark_comparison_re5000.tex <==
\subsection{Lid driven cavity with Re=5000}

Table with PETSc options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 case name & ksp & prec & snes tol & ksp tol & add. opt. \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=360 & ibcgs & asm & atol 1e-8 rtol 1e-8 & default & none \\ 
 \hline
 128x128x128,c,TFEM,t=360 & ibcgs & asm & atol 1e-8 rtol 1e-8 & default & -snes\_ksp\_ew \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
Table with configure.txt options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 case name & Lx,Ly,Lz & Nelemx,Nelemy,Nelemz & num of blocks \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=360 & 1,1,1 & 32,32,32 & 360 \\ 
 \hline
 128x128x128,c,TFEM,t=360 & 1,1,1 & 128,128,128 & 360 \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
where:
\begin{itemize}
\item[c] - means clustered grid in $x$ and $y$ direction
\item[TFEM] - means FEM in time formulation for Navier-Stokes equation with VMS stabilization
\item[t] - is a simulation time
\end{itemize}





%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in X direction along vertical line (Re=5000)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$y$},
%		ylabel={$vel\_x$},
%		legend pos=north west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-5000-32x32-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=360}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-5000-128x128-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=360}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-5000-32x32-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=360}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-5000-128x128-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=360}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 5] 
%		{data_files/LDC_study/ghia_vel_x.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-5000-ux}
%		%\subcaption{$Re=5000$, $u_x$}
%	\end{minipage}
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in Y direction along horizontal line (Re=5000)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$x$},
%		ylabel={$vel\_y$},
%		legend pos=south west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-5000-32x32-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=360}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-5000-128x128-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=360}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-5000-32x32-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=360}}
%		
%		\addplot+[no markers,dashed,thick]
%		table {data_files/LDC_study/Re-5000-128x128-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=360}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 5] 
%		{data_files/LDC_study/ghia_vel_y.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa 
%		%t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-5000-uy}
%		%\subcaption{$Re=5000$, $u_y$}
%	\end{minipage}	
%	\label{fig:ldc-re-5000}
%	\caption{LDC, Re=5000}
%\end{figure}


==> sections/1005_LDC_benchmark_comparison_re7500.tex <==
\subsection{Lid driven cavity with Re=7500}

Table with PETSc options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 case name & ksp & prec & snes tol & ksp tol & add. opt. \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=720 & bcgsl & default & atol 1e-8 rtol 1e-8 & default & none \\ 
 \hline
 128x128x128,c,TFEM,t=720 & ibcgs & asm & atol 1e-8 rtol 1e-8 & default & -snes\_ksp\_ew \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
Table with configure.txt options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 case name & Lx,Ly,Lz & Nelemx,Nelemy,Nelemz & num of blocks \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=720 & 1,1,1 & 32,32,32 & 720 \\ 
 \hline
 128x128x128,c,TFEM,t=720 & 1,1,1 & 128,128,128 & 720 \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
where:
\begin{itemize}
\item[c] - means clustered grid in $x$ and $y$ direction
\item[TFEM] - means FEM in time formulation for Navier-Stokes equation with VMS stabilization
\item[t] - is a simulation time
\end{itemize}



%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in X direction along vertical line (Re=7500)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$y$},
%		ylabel={$vel\_x$},
%		legend pos=north west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-7500-32x32-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=720}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-7500-128x128-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=720}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-7500-32x32-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=720}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-7500-128x128-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=720}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 6] 
%		{data_files/LDC_study/ghia_vel_x.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-7500-ux}
%		%\subcaption{$Re=7500$, $u_x$}
%	\end{minipage}
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in Y direction along horizontal line (Re=7500)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$x$},
%		ylabel={$vel\_y$},
%		legend pos=south west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-7500-32x32-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=720}}
%		
%		\addplot+ [no markers]
%		table {data_files/LDC_study/Re-7500-128x128-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=720}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-7500-32x32-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=720}}
%		
%		\addplot+ [no markers,dashed,thick]
%		table {data_files/LDC_study/Re-7500-128x128-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,TFEM,t=720}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 6] 
%		{data_files/LDC_study/ghia_vel_y.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa 
%		%t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-7500-uy}
%		%\subcaption{$Re=7500$, $u_y$}
%	\end{minipage}	
%	\label{fig:ldc-re-7500}
%	\caption{LDC, Re=7500}
%\end{figure}

==> sections/1006_LDC_benchmark_comparison_re10000.tex <==
\subsection{Lid driven cavity with Re=10000}

Table with PETSc options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c|c|c| } 
 \hline
 case name & ksp & prec & snes tol & ksp tol & add. opt. \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=1000 & bcgsl & default & atol 1e-8 rtol 1e-8 & default & none \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
Table with configure.txt options
\begin{center}
\begin{small}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 case name & Lx,Ly,Lz & Nelemx,Nelemy,Nelemz & num of blocks \\ 
 \hline
 \hline
 32x32x32,c,TFEM,t=1000 & 1,1,1 & 32,32,32 & 1000 \\ 
 \hline
\end{tabular}
\end{small}
\end{center}
where:
\begin{itemize}
\item[c] - means clustered grid in $x$ and $y$ direction
\item[TFEM] - means FEM in time formulation for Navier-Stokes equation with VMS stabilization
\item[t] - is a simulation time
\end{itemize}



%\begin{figure}[!htb]
%	\centering
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in X direction along vertical line (Re=10000)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$y$},
%		ylabel={$vel\_x$},
%		legend pos=north west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-32x32-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=1000}}
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-128x128-ts_cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=1000}}
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-32x32-cos-vel_x.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=1000}}
%		
%		%\addplot+ [
%		%    no markers,
%		%    ] 
%		%    table {data_files/LDC_study/Re-10000-128x128-cos-vel_x.curve};
%		%\addlegendentry{{128x128x128,c,TFEM,t=1000}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 7] 
%		{data_files/LDC_study/ghia_vel_x.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-10000-ux}
%		%\subcaption{$Re=10000$, $u_x$}
%	\end{minipage}
%	\begin{minipage}{.49\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%%		title={Velocity in Y direction along horizontal line (Re=10000)},
%%		scale only axis,
%%		width=0.75\textwidth,
%		width=0.99\linewidth,
%		xlabel={$x$},
%		ylabel={$vel\_y$},
%		legend pos=south west,
%		legend cell align=left,
%		major grid style=dotted,
%		grid=major,
%		]
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-32x32-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,seq,t=1000}}
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-128x128-ts_cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 128^2\times 128 $,c,seq,t=1000}}
%		
%		\addplot+ [
%		no markers,
%		] 
%		table {data_files/LDC_study/Re-10000-32x32-cos-vel_y.curve};
%		\addlegendentry{\tiny{$ 32^2\times 32 $,c,TFEM,t=1000}}
%		
%		%\addplot+ [
%		%    no markers,
%		%    ] 
%		%    table {data_files/LDC_study/Re-10000-128x128-cos-vel_y.curve};
%		%\addlegendentry{{128x128x128,c,TFEM,t=1000}}
%		
%		\addplot [
%		only marks,
%		color = black,
%		mark=x,
%		] 
%		table [x index = 0, y index = 7] 
%		{data_files/LDC_study/ghia_vel_y.curve};
%		\addlegendentry{\tiny Reference(Ghia)}
%		
%		\end{axis}
%		\end{tikzpicture}
%		% \subcaption{Pure diffusion with analytical solution $u = 
%		%e^{-2\pi^2\kappa 
%		%t}\sin{(\pi x)}\sin{(\pi y}$)}
%		\label{fig:ldc-re-10000-uy}
%		%\subcaption{$Re=10000$, $u_y$}
%	\end{minipage}	
%	\label{fig:ldc-re-10000}
%	\caption{LDC, Re=10000}
%\end{figure}

==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
%Intro-intro
%Spacetime parallelism
%Early spacetime multigrid methods
%Other attempts at space-time methods different usage of this terminology
%Continuous Galerkin space-time attempts
%Theoretical works
%Our work

Transient physical processes are typically described by time-dependent partial differential equations (PDEs). Mathematical analysis shows that, given smooth and compatible initial condition and boundary conditions, many of these equations have solutions of certain regularity in both space and time dimensions. When solving these equations numerically, the most common practice is to use the method of lines which has two variants: (i) where the PDE is discretized in space to obtain a large system of ordinary differential equations (ODEs), which are then integrated in time; and (ii) where the equations are discretized is time first, to obtain a continuous PDE in spatial variables, which are then solved using techniques for solving stationary PDEs.

The nature of the method of lines makes it a sequential process. To illustrate this, suppose $ \temporalInterval = [0,T] $ denotes a time interval of interest. In the method of lines, say we discretize this interval into $ n_t $ finite time steps, each of length $ \Delta t = \frac{T}{(n_t - 1)} $. So the PDE of interest, now semidiscrete, has to be solved at time points: $ \Delta t,\ 2\Delta t,\ 3\Delta t,...,\ (n_t-1)\Delta t = T $. In such algorithms, the solution at a particular step depends on the solutions at previous time steps. Thus, the solution process essentially becomes evolutionary: marching from one time step to the next, thereby mimicking the physical process itself. 

But, it is not necessary for a numerical method to really mimic the physical process in its evolutionary characteristics. Prior work \citep{nievergelt1964parallel,Hackbusch:1985:PMM:4673.4714,chartier1993parallel,horton1995space,gander1996overlapping,gander1999optimal,LionsEtAl2001} has shown that solving for a solution at a later time does not have to wait for the solutions of intermediate points to finish. Rather, all these computations can progress in parallel. A brief review of some of these methods can be found in \cite{gander201550}. A common theme that runs through these methods is the idea of parallelization of computation, possibly coupled with decomposing the spatiotemporal domain (i.e., the tensor product of the spatial domain and the time window) into multiple smaller subdomains.

Multiple types of decompositions have been proposed in the context of space-time parallelism. Early works such as \cite{nievergelt1964parallel,saha1996parallel} or more recent works such as \cite{LionsEtAl2001} decompose the PDE primarily in time. Such methods fall under the methods relying on temporal domain decomposition. Similarly, works based on waveform relaxation methods \cite{gander1996overlapping,gander1999optimal} achieve decomposition primarily in spatial domain. Domain decomposition in both space and time was considered by \cite{Hackbusch:1985:PMM:4673.4714, horton1995space, lubich1987multi}, where mulitigrid approach was adopted to solve the spatiotemporal system of equations. But it was noticed that the multigrid coarsening does not work the same way in time as it would in the spatial dimension; in particular, coarsening in time may not always lead to right convergence. 

In the context of finite element method (FEM), a method of lines discretization usually employs a finite difference scheme (e.g., Euler scheme), and many space-time parallel implementations rely on them \cite{LionsEtAl2001, dyja2018parallel}. But works such as \cite{hughes1988space, hulbert1990space} have applied discontinuous Galerkin (dG) discretization in the time dimension in tandem with continuous Galerkin (cG) approximation in space. These methods are also commonly known as ``space-time finite element methods'', but these are still sequential in nature, i.e., one usually solves one ``slab'' of time-window before solving another in order. Some more examples of this kind of discretization can be found in \cite{pontaza2004space, tezduyar2006space, tezduyar2008arterial, scovazzi2007stabilized, song2015nitsche, gander2016analysis}.

Recently, efforts have been made to apply continuous Galerkin method for time discretization \cite{munts2006space, behr2008simplex,steinbach2015space, langer2016space, fuhrer2021space}. And works such as \cite{ishii2019solving} explore the scalability and advantages of solving these formulations on large computing clusters. Most of these works are limited to linear parabolic equations such as the heat equation, but they do highlight some of the issues of approximating the dependence of the solution on time through continuous basis functions, in particular, the need for a stabilized method. Theoretical analysis \cite{andreev2012stability} of this problem also refers to a need for such a method. 

In this work, our goal is to develop a fast and scalable \textit{continuous Galerkin} method for a space-time coupled discretization of the Navier-Stokes equations. As will be discussed in Sec. \ref{sec:formulations}, the stabilization requirements for the space-time discretization of the Navier-Stokes equations reduce to the following: (i) stabilization of the dominant convection terms and (ii) stabilization of the saddle point nature of the incompressible Navier-Stokes equations. The first kind of stability can be provided by multiple ways, including the streamline upwind Petrov Galerkin (SUPG) method \cite{brooks1982streamline}, the Galerkin Least Square (GLS) method \cite{hughes1989new,douglas1989absolutely}, or the variational multiscale (VMS) method \cite{hughes1995multiscale}. The second type of stability can be provided by the pressure stabilized Petrov Galerkin (PSPG) method \cite{hughes1986new}. But it has been shown that the application of the multiscale ideas can naturally lead to a stabilization scheme that encompass both SUPG and PSPG type of stabilizations \cite{bazilevs2007variational}. The application of VMS also leads to a grad-divergence stabilization.

In this paper, we argue that VMS also helps stabilize the space-time variational equations in a continuous Galerkin setting. The variational problem then can be solved in a domain-decomposed manner to obtain a fully coupled space-time problem that also translates into a stable linear algebra problem. Our contributions in this paper are as follows:
\begin{enumerate}
	\item A continuous Galerkin method for solving the Navier-Stokes equations in coupled space-time.
	\item An application of VMS to stabilize the linear algebra problem against both spatial and temporal convective effects and with equal-order velocity-pressure pair spaces.
	\item A rigorous analysis of the space-time variational problem.
	\item Validation of the method against benchmark problems.
\end{enumerate}

The rest of the paper is organized as follows:  \secref{sec:formulations} presents the mathematical background and derives the variational formulation, \secref{sec:analysis} provides an analysis of the variational problem, \secref{sec:implementation} provides the implementations details, \secref{sec:num-examples-results} presents the numerical experiments and validation results; and  \secref{sec:conclusions} provides some discussions and conclusions.

%Most of these methods rely on some finite difference discretization in time. They are discrete times and nothing between them exists
%
%Space-time finite element methods in the sense of Hughes, Tezduyar, Kenji Takizawa.. and also those based on Neumuller, and even Parareal etc.
%
%But those are still marching solutions. what about non-marching solutions?
%
%Even in non-marching solutions, many are DG. Is it possible to do it in CG?
%
%What about stability? talk about vms
%
%In the context of solving time-dependent PDEs, the so called ``space-time methods" refer to the formalisms where the entire time horizon of the problem is solved simultaneously. Thus, it is inherently different from the conventional ``time-marching methods" where the PDE is solved sequentially at discrete time points.But space-time methods have one more interesting feature, i.e., parallelism in time. In a sequential method, some kind of domain decomposition can be achieved in the spatial operators. But in space-time method, time, along with space, can be domain decomposed. This gives us an interesting motivation to develop methods in coupled space-time and explore the extent to which the computations can be parallelized.
%
%This parallelization has been demonstrated with finite difference methods. Refer to some of the early space-time multigrid literature. In these methods, the PDE is first discretized using any suitable and well-known sequential time-discretization methods (such as backward Euler, Crank-Nicolson scheme etc). But this discretized equation is not solved using a marching algorithm. Instead, the discrete equation is written down for each time point in the entire time horizon; and finally all those equations are collected to form a large coupled system of equations. Ref, e.g., \cite{dyja2018parallel}.
%
%But a straightforward adaptation of this technique using FEM is fraught with some issues. The crux of this problem is the time-derivative term itself, which is a directional operator, just like any other gradient. On the other hand, it is well known that the classical Galerkin method (with piecewise polynomial basis functions) is not suitable for problems where a directional operator such as a gradient is dominant. In the last forty years, many prominent methods have been developed to tackle this issue, such as SUPG, GLS, SGS and VMS, all of which can be accommodated in a CG framework. This interpretation of the time-derivative as an ``advection" in the time direction (with positive velocity) then allows us to bring the ideas of spatial stabilizations and apply to the time direction.
%
%In this work, we present a space-time coupled CG formulation for solving flow problems using the Navier-Stokes equations. We present the mathematical formulations, numerical results and conclusions. In this paper, we focus on the challenges of formulating a nonlinear flow problem using a couple space-time CG method. The performance of this method in a large parallel environment needs to be studied further, which will be undertaken in future.
%\begin{itemize}
%    \item Solution of time dependent partial differential equations can be done 
%    with space-time finite elements
%    \item Popular approach is to discretize space using finite elements 
%    (semi-discretization in space) and then discretize time using finite 
%    differences (time marching)
%    \item Space-time finite elements use finite element discretization in both space and time
%    \item Advantage of treating time the same way as space dimensions is possibility of mesh refining in both space and time
%    \item We solve Navier-Stokes equation using VMS stabilization together with space-time formulation of finite element
%    \item We present results for lid driven cavity up to Reynolds number 10000, flow past cylinder with Reynolds number in range 100-500
%    \item We also use pseudo time continuation to overcome problems with initial guess for nonlinear solver
%    \item Space-time approach has been exploited by many researchers: \cite{hughes1988space}, \cite{hulbert1990space} solved second order hyperbolic elastodynamic problems by discontinuous Galerkin 
%    \item \cite{pontaza2004space} solves incompressible Navier-Stokes equation
%    \item \cite{tezduyar2006space}, \cite{tezduyar2008arterial} solve fluid-structure interaction problem
%    \item \cite{takizawa2011multiscale}, \cite{takizawa2013space} solve multiscale fluid structure interaction problem
%    \item Similar approaches (like solving in blocks of time, “parareal”, multidimensional simplex FEs) were investigated by \cite{behr2008simplex}, \cite{carey2010blockwise}, \cite{mani2011efficient}, \cite{rendall2012conservative}, \cite{wang2015high}, \cite{dyja2018parallel}
%    \item space-time tensor product discretization for wave equations \cite{french1993space,french1996continuous}
%    \item space-time CG for NS - \cite{pontaza2003spectral,pontaza2004space}
%    \item enriched space-time method (EST) \cite{zilian2008enriched}
%\end{itemize}
%\begin{itemize}
%	\item Blah
%	\item Talk about space-time parallelizations (mention baskar's earlier paper.. and also our SC paper)
%	\item Space-time FE CG discretizations
%	\item talk about nonlinear problems, flow problems
%	\item the contributions of this paper
%\end{itemize}


==> sections/2003_FPC_Re_study.tex <==
%\subsubsection{Flow past cylinder results with different Reynolds number}
%
%\include{data_files/FPC_study/St_table}

==> sections/2_spacetime_vms_formulation.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
\section{Space-time variational formulation}
\label{sec:formulations}
\subsection{Preliminaries} \label{sec:prelim}
\begin{figure}[!t]
	\centering
	\def \mpagefrac{0.7}
	\begin{minipage}{\mpagefrac\textwidth}
		\centering
		\begin{tikzpicture}
		\def \myscale{\mpagefrac / 0.5} % needs \usepackage{calc}
		\draw (0, 0) node[inner sep=0] {\includegraphics[trim=3.3in 0.5in 3.3in 0.8in, clip,width=0.7\linewidth]{images/domain-notations.pdf}};
		\draw (0, 0) node {$ \stDom = \spDom \times \temporalInterval $};
		\draw (-2.5*\myscale, 3.0*\myscale) node {$t$};
		\draw (-2.7*\myscale,  2.1*\myscale) node {$t=T$};
		\draw (-2.7*\myscale, -1.5*\myscale) node {$t=0$};
		\draw (-2.2*\myscale, -2.7*\myscale) node {$x_1$};
		\draw ( 2.6*\myscale, -1.5*\myscale) node {$x_2$};
		\draw[stealth-, thick] (-0.2*\myscale, -1.6*\myscale) -- ++(0.5*\myscale,-1.3*\myscale) node[right, black, fill=white, anchor=north]{$\bit = \spDom\times \{0\}$};
		\draw[stealth-, thick] (-0.2*\myscale, 2.1*\myscale) -- ++(0.2*\myscale,1.0*\myscale) node[right, black, fill=white, anchor=south]{$\bft = \spDom\times \{T\}$};
		\draw[stealth-, thick] (1.45*\myscale, 0.1*\myscale) -- ++(0.7*\myscale,1.0*\myscale) node[right, black, fill=white, anchor=south west]{$\bsp = \partial \spDom \times (0,T)$};
%		\draw (3*\myscale, 3*\myscale) node {$ (3, 3) $};
%		\draw (-3*\myscale, -3*\myscale) node {$ (-3, -3) $};
		\end{tikzpicture}
	\end{minipage}
	\caption{Schematic depiction of the space-time domain $ \stDom = \spDom \times \temporalInterval $, where $ \spDom \subset \mathbb{R}^{\nsd} $, and $ \temporalInterval = [0,T] \subset \mathbb{R}^{+}. $} 
	\label{fig:schematic-space-time-domain}
\end{figure}
Consider a bounded, open spatial domain $\spDom \in \mathbb{R}^\nsd, \nsd\in\{2,3\}$ with Lipschitz continuous boundary $\partial \spDom$ and a bounded time interval $\temporalInterval = (0,T] \in \mathbb{R^+}$. We define the space-time domain as the Cartesian product of the two: $\stDom = \spDom \times \temporalInterval = \spDom\times(0,T]$ (see \figref{fig:schematic-space-time-domain}). Suppose $ \xvec\in\spDom $ and $ t\in\temporalInterval $ and define $ \xvecst = (\xvec, t)^T \in \stDom$. The overall boundary of this space-time domain is defined as $\Gamma = \partial \stDom$. This ``overall boundary" is the union of the ``spatial boundaries" and the ``time boundaries". The spatial domain boundary is denoted by $\bsp = \partial \spDom \times (0,T)$; whereas the time boundaries are denoted by $\bit = \bar{\spDom}\times\{0\}$ and $\bft = \bar{\spDom}\times\{T\}$ which are the initial and final time boundaries respectively. Therefore $\Gamma = \bsp \cup \bit \cup \bft$.

On this space-time domain $ \stDom $, the incompressible Navier-Stokes equations can then be written for the vector function $\uvec = \uvec(\xvecst): \stDom \rightarrow \mathbb{R}^\nsd$ and the scalar function $ p = p(\xvecst):\stDom\rightarrow \mathbb{R} $ as:
\begin{subequations}\label{eq:ns-original}
	\begin{align}
	\timeder{\uvec}+(\uvec\cdot\grad)\uvec + \half(\divergence\uvec)\uvec -\visco\laplacian \uvec+\grad p - 
	\fvec &= \zerovec, \text{ }\xvecst\in\stDom, \label{eq:ns-original-momentum}
	\\
	\grad\cdot\uvec &= 0, \text{ }\xvecst\in\stDom, \label{eq:ns-original-continuity}
	\\
	\uvec &= \zerovec, \text{ }\xvecst\in\bsp, \label{eq:ns-original-dirichlet}
%	\\
%	\mathscr{B}_{NR} \uvec &= h, \text{ }\xvecst\in\Gamma_{S2}\subseteq\bsp, \label{eq:ns-original-neumann}
	\\
	\uvec &= \uvec_0, \text{ }\xvecst\in\bit, \label{eq:ns-original-ic}
	\end{align}
\end{subequations}
where, $ \uvec = (\ucomp{1}, \ldots, \ucomp{\nsd})^T $ is the velocity vector, $ p $ is the pressure, and $ \nu $ is the kinematic viscosity, which is assumed constant. The Reynolds number is expressed as $Re = \nicefrac{1}{\visco}$ and the forcing function $\fvec : \stDom \rightarrow \mathbb{R}^\nsd$ is assumed to be smooth. Note that $\grad$ is the usual spatial gradient operator in the space $\mathbb{R}^{\nsd}$, i.e., $ \grad \equiv (\nicefrac{\partial}{\partial x}, \nicefrac{\partial}{\partial y}) $ for $ \nsd = 2 $ and $ \grad \equiv (\nicefrac{\partial}{\partial x}, \nicefrac{\partial}{\partial y}, \nicefrac{\partial}{\partial z}) $ for $ \nsd = 3 $ respectively. We further define the space-time gradient operator $\gradst$ as: $ \gradst \equiv (\grad, \nicefrac{\partial}{\partial t}) $.

%The velocity $ \uvec $ on the domain boundaries is determined via some essential (or Dirichlet) boundary condition on a subset of the spatial boundary $ \Gamma_{S1} $. In addition, a Neumann/Robin condition is applied on another subset of the spatial boundary $ \Gamma_{S2} $ (equation \ref{eq:ns-original-neumann}). Here, $ \mathscr{B}_{NR} $ is a  linear combination of differential operators of order 1 or 0. Note that, $ \Gamma_{S1}\cup\Gamma_{S2} \subseteq \bsp $ and $ \Gamma_{S1}\cap\Gamma_{S2} = \varnothing $.

Let us define two operators $ \opLAdv[\avec] $ and $ \opLTAdv[\avec] $ as follows:
\begin{subequations} \label{eq:def-la-ma}
	\begin{align}
	\opLAdv[\avec] \uvec &= \adiv \uvec + \halfnice (\divergence \avec) \uvec, \label{eq:opL} \\
	\text{and}\ \ \opLTAdv[\avec] \uvec &= \ut + \opLAdv[\avec] \uvec = \ut + \adiv \uvec + \halfnice (\divergence \avec) \uvec. \label{eq:opLT}
	\end{align}
\end{subequations} 
For a given $ \avec $, the operators $ \opLAdv[\avec]\uvec $ and $ \opLTAdv[\avec]\uvec $ are linear in $ \uvec $, whereas $ \opLAdv[\uvec]\uvec,\ \opLTAdv[\uvec]\uvec $ are nonlinear. With this notation, we can rewrite \eqref{eq:ns-original-momentum} as
\begin{align} \label{eq:ns-linearized-0}
\opLTAdv[\uvec]\uvec - \visco\laplacian\uvec + \grad p &= \fvec \ \text{in} \ \stDom.
\end{align}

\begin{remark}
	Note that in \eqref{eq:ns-original-momentum} and \ref{eq:def-la-ma}, we have included the additional terms $ \halfnice(\divergence\uvec)\uvec $ and $ \halfnice(\divergence\avec)\uvec $ respectively. This term was introduced in \cite{temam1968methode}, and has been included in the literature to ensure dissipativity of  various numerical schemes, especially when the function spaces are not divergence-free \cite{shen1996error, shen1997pseudo, codina2001stabilized}. In addition, the presence of this term makes the operators $ \opLAdv[\avec] $ and  $ \opLTAdv[\avec] $ skew-symmetric (see \autoref{item:adjoint-op} in \secref{sec:anlys-prelim}).
\end{remark}
\begin{remark}
	The case of non-zero boundary  conditions will be discussed in \secref{sec:nonzero-icbc}.
\end{remark}

\subsubsection{Space-time inner products and norms}
\label{sec:inner-prod-norms}
The $ L^2 $-inner product on the space-time domain $ \stDom $ is expressed as: 
\begin{itemize}
	\item Scalar-valued functions:
	\begin{align} \label{eq:inner-prod-scalar}
	\inner{a}{b} &:= \inner{a}{b}_{\stDom} = \intSTDom  a(\xvecst)b(\xvecst) \text{ }d\xvecst = \intTimeSpace a(\xvec, t)b(\xvec,t) \text{ } d\mvec{x} dt.
	\end{align}
	\item Vector-valued functions:
	\begin{align} \label{eq:inner-prod-vector}
	\inner{\mvec{a}}{\mvec{b}} &:= \inner{\mvec{a}}{\mvec{b}}_{\stDom} = \intSTDom  \mvec{a}(\xvecst)^T \mvec{b}(\xvecst) \text{ }d\xvecst = \intTimeSpace \mvec{a}(\xvec, t)\cdot\mvec{b}(\xvec,t) \text{ } d\mvec{x} dt,
	\end{align}
	\item Gradients of vector-valued functions:
	\begin{align} \label{eq:inner-prod-gradients}
	\inner{\grad \mvec{a}}{\grad \mvec{b}} &:=   \Xsum_{i=1}^{\nsd} \inner{\grad a_i}{\grad b_i},
	\end{align}
	where $ a_i $ and $ b_i $ are the scalar components of $ \avec $ and $ \bvec $ respectively. Each inner product $ \inner{\grad a_i}{\grad b_i} $ is calculated according to \eqref{eq:inner-prod-vector}.
\end{itemize}

We define a ``temporal slice'' as a slice of $ \stDom $ obtained by fixing the time at a particular $ t=t' $, and denote it by $ \spDom(t') $. An inner product on such a slice at $ t=t' $ will be denoted with a subscript, i.e.,
\begin{align}
\inner{\mvec{a}}{\mvec{b}}_{\spDom(t')} = \int_{\spDom(t')} \mvec{a}(\xvec,t=t')^T \mvec{b}(\xvec,t=t')\text{ } d \mvec{x}.
\end{align}
A special case of temporal slices is the ``final time'' slice, i.e., $ \spDom(T) $. Since $ \spDom(T) $ is the same as $ \bft $, we will denote this inner product by
\begin{align}
\innerFT{\avec}{\bvec} = \inner{\mvec{a}}{\mvec{b}}_{\spDom(T)} = \int_{\spDom(T)} \avec(\xvec,T)^T\bvec(\xvec,T) \ d\xvec.
\end{align}
Similarly, the space-time and the spatial $ L^2 $-norms are defined as:
\begin{align}
\norm{\avec} := \norm{\avec}_{\stDom} = \normL{\avec}{\stDom} &= \sqrt{\inner{\avec}{\avec}}, \\
\norm{\avec}_{\spDom(t')} := \normL{\avec}{\spDom(t')} &= \sqrt{\inner{\avec}{\avec}_{\spDom (t')}}, \ t' \in\temporalInterval, \\
\normFT{\avec} := \norm{\avec}_{L^2(\bft)} = \normL{\avec}{\spDom (T)} &= \sqrt{\inner{\avec}{\avec}_{\spDom (T)}}.
\end{align}
respectively, where $ \avec(\xvec,t) $ is any function that belongs to $ L^2(\stDom) $. In the sequel, unless otherwise specified, $ \inner{\cdot}{\cdot} $ and $ \norm{\cdot} $  will denote $ \inner{\cdot}{\cdot}_{\stDom} $ and $ \norm{\cdot}_{\stDom} $ respectively.

\begin{remark}[\textit{Integration by parts}]
	A typical integration-by-parts \textit{over spatial derivatives} can be written as follows.
	\begin{itemize}
		\item Scalar functions:
		\begin{align}
		\inner{\laplacian a}{b} = \intTimeSpace \laplacian a \ b \ d\spDom \ dt &= \intTime \left[ -\intSpace \grad a \cdot \grad b\ d\spDom + \int_{S=\partial \spDom}  (\normalvec\cdot\grad a)b \ dS \right]dt \\
		&= -\inner{\grad a}{\grad b} + \inner{\normalvec\cdot \grad a}{b}_{\bsp}.
		\end{align}
		\item Vector functions:
		\begin{align*}
		\inner{\laplacian \avec}{\bvec} = \Xsum_{i=1}^{\nsd} \inner{\laplacian a_i}{b_i} &= \Xsum_{i=1}^{\nsd} \left[-\inner{\grad a_i}{\grad b_i} + \inner{\normalvec\cdot \grad a_i}{b_i}_{\bsp} \right] \\
		&= -\inner{\grad \avec}{\grad \bvec} + \inner{(\normalvec\cdot \grad)\avec}{\bvec}_{\bsp}.
		\end{align*}
	\end{itemize}	
	Similarly, integration by parts \textit{over temporal derivatives} can be written as:
	\begin{itemize}
		\item Scalar functions:
		\begin{align*}
		\inner{\partial_t a}{b} = \intSpaceTime \partial_t a\ b\ dt d\spDom &= \intSpace \left[-\intTime a\ \partial_t b\ dt + ab \big|_{0}^{T} \right]d\spDom \\
		&= -\inner{a}{\partial_t b} + \intSpace a(\xvec,T)b(\xvec,T)d\spDom - \intSpace a(\xvec,0)b(\xvec,0) d\spDom \\
		&= -\inner{a}{\partial_t b} + \innerFT{a}{b} - \inner{a}{b}_{\bit}
		\end{align*}
		\item Vector functions:
		\begin{align*}
		\inner{\partial_t \avec}{\bvec} = \Xsum_{i=1}^{\nsd} \inner{\partial_t a_i}{b_i} &= -\inner{a_i}{\partial_t b_i} + \innerFT{a_i}{b_i} - \inner{a_i}{b_i}_{\bit} \\
		&= -\inner{\avec}{\partial_t \bvec} + \innerFT{\avec}{\bvec} - \inner{\avec}{\bvec}_{\bit}.
		\end{align*}
	\end{itemize}
\end{remark}

\begin{remark}[\textit{Discrete inner products and norms}]
	Given a mesh $ \mesh $, we define the following notations for discrete inner products and norms on the mesh $ \mesh $:
	\begin{subequations} \label{eq:discrete-norms}
		\begin{align}
		\innerh{\avec}{\bvec} &= \Xsum_{K \in \mesh} \inner{\avec}{\bvec}_{K}, \quad
		\normh{\avec} = \left[\Xsum_{K \in \mesh} \inner{\avec}{\avec}_{K}\right]^{\halfnice}, \\
		\innerFTh{\avec}{\bvec} &= \Xsum_{K \in \bft} \inner{\avec}{\bvec}_{K} \quad \normFTh{\avec} = \left[\Xsum_{K \in \bft} \inner{\avec}{\bvec}_{K} \right]^{\halfnice}.
		\end{align}
	\end{subequations}
\end{remark}

\subsection{Stabilized finite element formulations} \label{sec:stabilized-formulations}

%Let us also define a trilinear product $ (\cdot,\cdot,\cdot) $ as
%\begin{align}
%	(\mvec{u},\mvec{v},\mvec{w}) := \Big( \mvec{w},(\mvec{u}\cdot\grad)\mvec{v} \Big)
%\end{align}

%\subsection{Linearized equations}
%Since \eqref{eq:ns-original} is nonlinear in $ \uvec $, we first linearize it by assuming that the convection field is known and is given by $ \avec $.
%Let us define two operators $ \opLAdv[\avec] $ and $ \opLTAdv[\avec] $ as follows:
%\begin{subequations}
%	\begin{align}
%		\opLAdv[\avec] \uvec &= \adiv \uvec + \halfnice (\divergence \avec) \uvec, \label{eq:opL} \\
%		\text{and}\ \ \opLTAdv[\avec] \uvec &= \ut + \opLAdv[\avec] \uvec = \ut + \adiv \uvec + \halfnice (\divergence \avec) \uvec. \label{eq:opLT}
%	\end{align}
%\end{subequations}
%For a given $ \avec $, the operators $ \opLAdv[\avec] $ and $ \opLTAdv[\avec] $ are linear in $ \uvec $. With this notation, we can rewrite \eqref{eq:ns-original-momentum} for a given convection field $ \avec $ as
%%\begin{align}
%%	\opLTAdv[\uvec] \uvec - \visco\laplacian \uvec + \grad p - \fvec = \zerovec.
%%\end{align}
%%
%%Using the operator notations defined in \eqref{eq:opLT}, we can write \eqref{eq:ns-original-momentum} for a given convection field $ \avec $ as
%\begin{align} \label{eq:ns-linearized-0}
%	\opLTAdv[\avec]\uvec - \visco\laplacian\uvec + \grad p &= \fvec \ \text{in} \ \stDom.
%\end{align}
%Now, suppose
%\begin{align}
%	\mvec{W} &= \setbuilder{\uvec:\ \ut \in C(\stDom),\ \laplacian \uvec \in C(\stDom),\ \uvec|_{\bsp} = \uvec_D,\ \uvec|_{\bit} = \uvec_0}, \\
%	\mvec{W}_0 &= \left\{\uvec:\ \ut \in C(\stDom),\ \laplacian\uvec \in C(\stDom),\  \uvec = \zerovec \text{ on }\bsp\cup\bit\right\}, \\
%	\mvec{W}_{\text{div}} &= \setbuilder{\uvec:\ \grad\uvec \in C(\stDom),\ \divergence\uvec = 0}.
%\end{align}
%Let $ \mvec{h} \in \mvec{W} \cap \mvec{W}_{\text{div}} $ be a given function and $ \uvec\in \mvec{W}_0 $ be unknown. For a given convection $ \avec $, if the exact solution of \eqref{eq:ns-linearized-0} is $ (\uvec_*, p_*) $, then $ \uvec_* $ can be written as
%\begin{align}\label{eq:exact-sol-decomposition}
%	\uvec_*(\xvecst) = \uvec(\xvecst) + \gvec (\xvecst).
%\end{align}
%Substituting \eqref{eq:exact-sol-decomposition} in \eqref{eq:ns-linearized-0}, and redefining $ \fvec $ as $ \fvec := \fvec -(\opLTAdv[\avec]\mvec{h} - \visco\laplacian\mvec{h}) $, we have the following set of linearized equations with homogeneous boundary conditions:
%\begin{subequations}\label{eq:ns-linearized-zerobc}
%	\begin{align} 
%		\opLTAdv[\avec]\uvec - \visco\laplacian\uvec + \grad p &= \fvec \ \text{in} \ \stDom, \label{eq:ns-lin-momentum}\\
%		\divergence\uvec &= 0\ \text{in}\ \stDom, \label{eq:ns-lin-continuity} \\
%		\uvec &= \zerovec\ \text{on} \ \bsp\cup\bit. \label{eq:ns-lin-zerobc}
%	\end{align}
%\end{subequations}

\subsubsection{Galerkin formulation and its lack of stability} \label{sec:lack-of-stability}
A classical Galerkin FEM formulation of \eqref{eq:ns-transformed} suffers from two major issues:
%There are two major issues associated with the FEM formulation in Eq. \eqref{eq:var-problem-unstabilized}:
\begin{itemize}
	\item The first issue is associated with the choice of the continuous function spaces themselves, i.e., each of the velocities belong to the same function space as the pressure. This is an obvious case of a non \textit{inf-sup} stable pair of function spaces. So, a stable numerical solution cannot be guaranteed \cite{babuvska1973finite, brezzi1974existence, john2016finite}.
	\item At the discrete level, a continuous Galerkin method is most commonly implemented using low order local Lagrangian basis functions (globally $ C^0 $) which generally have no directional properties. Differential operators such as the Laplacian can be approximated very well with such basis functions, so that the final linear algebra system is stable. But it is well known that the use of such functions to approximate differential operators possessing directional properties (e.g., first derivatives like $ \partialder{}{x} $) can lead to numerical instabilities if these derivatives become dominant in the equation \cite{brooks1982streamline, hughes1989new, codina1998comparison}. In the case of the Navier-Stokes equations, this might happen when the convection term $ (\uvec\cdot\grad)\uvec $ becomes much larger than the diffusion term $ -\nu\laplacian \uvec $ (or in other words, when $ \nu \ll 1 $). In addition to the spatial advection term $ (\uvec\cdot\grad)\uvec $, the time derivative term $ \timeder{\uvec} $ also possesses a directional property.
\end{itemize}

%In fact, in the continuous momentum equations \eqref{eq:ns-original-momentum}, the time derivative term $ \timeder{\mvec{u}} = \left(1\cdot\timeder{}\right)\uvec $ can be thought of as an ``advection'' in the time dimension with a (constant) velocity of 1. Conceptually, it is natural then to combine both the spatial and temporal advection terms from Eq. \eqref{eq:ns-original-momentum} as follows:
%\begin{align}\label{eq:st-advection-illustration-1}
%	\timeder{\uvec} + (\uvec\cdot\grad)\uvec = 1\cdot\timeder{\uvec} + u_x\cdot\partialder{\uvec}{x} + u_y\cdot\partialder{\uvec}{y} + u_z\cdot\partialder{\uvec}{z} = \left[(u_x,u_y,u_z,1)\cdot\gradst\right]\uvec.
%\end{align}
%The operator within the square brackets of \eqref{eq:st-advection-illustration-1} can be interpreted as an advection in space-time. We can proceed with this notation and rewrite the momentum equations \eqref{eq:ns-original-momentum} as follows:
%\begin{align}
%	\label{eq:momentum-in-spacetime-1}
%	(\ellipticC\cdot\gradst)\uvec - \gradst\cdot( \ellipticD \gradst\uvec) + \ellipticI\gradst p &= \zerovec\\
%	\label{eq:momentum-in-spacetime-2}
%	\text{or,  }
%	\left[\ellipticC^T\gradst - \gradst^T\ellipticD\gradst\right]\uvec + \ellipticI\gradst p &= \zerovec
%\end{align}
%where $ \ellipticC $ $ \ellipticD $ and $ \ellipticI $ are defined as:
%\begin{align}\label{eq:def-elliptic-matrices-cdi}
%%	[u_x, u_y, u_z, 1]
%	\ellipticC = 
%	\begin{bmatrix}
%	u_x\\ u_y\\ u_z\\ 1
%	\end{bmatrix},
%	\quad
%	\ellipticD = 
%	\begin{bmatrix}
%	\visco & 0 & 0 & 0 \\
%	0 & \visco & 0 & 0\\
%	0 & 0 & \visco & 0 \\
%	0 & 0 & 0 & 0
%	\end{bmatrix},
%	\quad
%	\ellipticI = 
%	\begin{bmatrix}
%	1 & 0 & 0 & 0 \\
%	0 & 1 & 0 & 0\\
%	0 & 0 & 1 & 0 \\
%	0 & 0 & 0 & 0
%	\end{bmatrix}
%%	\begin{bmatrix}
%%	\frac{\partial}{\partial x}\\
%%	\frac{\partial}{\partial y}\\
%%	\frac{\partial}{\partial z}\\
%%	\frac{\partial}{\partial t}
%%	\end{bmatrix}
%%	\left( 
%%	\frac{\partial}{\partial x},
%%	\frac{\partial}{\partial y},
%%	\frac{\partial}{\partial z},
%%	\frac{\partial}{\partial t}
%%	\right)
%\end{align}
%when $ \nsd = 3 $. For $ \nsd = 2 $, they are obtained by removing the third row (as well as the third column for $ \ellipticD $ and $ \ellipticI $).
%
%The operator within the square brackets in Eq. \eqref{eq:momentum-in-spacetime-2} is now immediately identified as a generalized ``advection-diffusion'' operator. Note that the ``diffusion'' part of the operator, i.e., $ -\gradst^T\ellipticD\gradst $ is degenerate since there is no diffusion in the time dimension, as represented by the zero-diagonal in the fourth row of $ \ellipticD $. But the advection part, i.e., $ \ellipticC^T\gradst $ is effective in all spatial and temporal directions, and thus all the numerical issues associated with the advection term - when formulated with conventional FEM basis functions - are inherited by equation \eqref{eq:fem-problem-unstabilized}.

There are multiple ways to resolve these two issues. The issue of instabilities due to non inf-sup conformity can be resolved by using methods such as PSPG \cite{hughes1986new, douglas1989absolutely, tezduyar1992incompressible} that remove the saddle point nature of the resulting FEM problem. The second issue can be resolved by using some kind of ``upwinding''-type modification to the test function $ \mvec{w} $ (e.g., SUPG \cite{brooks1982streamline}) or by using a least squares or subgrid-scale modifications to the FEM problem (e.g., GLS \cite{hughes1989new}, VMS \cite{hughes1995multiscale}) etc.


\subsubsection{Multiscale decomposition, and function spaces}

The variational multiscale (VMS) method is a technique that naturally resolves both issues discussed above in a consistent manner \cite{bazilevs2007variational}. Following the VMS methodology of \cite{hughes1995multiscale, bazilevs2007variational}, we decompose the infinite dimensional velocity $ \uvec $ and pressure $ p $ as:
\begin{align}\label{eq:vms-coarse-fine-decomposition}
\uvec = \uc + \uf \quad \text{and} \quad p = \pc + \pf,
\end{align}
where the bar ( $ \bar{} $ ) denotes a \emph{coarse scale} that can be resolved by the numerical method (i.e., by the grid/mesh) and the prime $(') $ denotes the \emph{fine scales} or the \emph{sub-grid scales} that are not resolved by the numerical method.

The variational problem is then formulated $ \uc $ and $ \pc $ and the \textit{effect} of $ \uvec' $ and $ p' $ (i.e., the sub-grid scales) is expressed using the residuals of $ \uc $ and $ \pc $ (i.e., the coarse scales). In the residul based VMS approach, the fine scales are modeled using the coarse-scale residuals (for a given $ \avec $) as
 \begin{subequations}
 	\label{eq:fine-scale-approximations}
 	\begin{align}
 	\uf &= -\taum^K (\opLTAdv[\avec]\uvech -\visco\laplacian\uvech + \grad\ph - \fvec) \ \text{in any element}\ K\in \mesh, \\
 	\pf &= -\tauc^K (\divergence\uvech) \ \text{in any element}\  K \in \mesh.
 	\end{align}
 \end{subequations}

\subsubsection{Stabilized variational form}
Consider the function spaces
\begin{subequations}\label{eq:fem-subspaces-modified}
	\begin{align}
		\spaceV &= \left\{ \mvec{v} \in \mvec{H}^1(\stDom):\  \mvec{v} = \zerovec \text{ on }\bsp\cup\bit\right\}, \\
		\spaceVd &= \left\{ \mvec{v} \in \mvec{H}^1(\stDom):\  \mvec{v} = \zerovec \text{ on }\bsp,\ \vvec = \uvec_0 \ \text{on} \ \bit \right\}, \\
		\spaceQ &= {H}^1(\stDom), \\
		\spaceVh &= \left\{ \vvech \in {\mvec{V}}:\  \vvech|_{K} \in \mvec{P_m}(K), \text{ } K \in \mesh \right\}, \\
		\spaceVhd &= \left\{ \vvech \in {\spaceVd}:\  \vvech|_{K} \in \mvec{P_m}(K), \text{ } K \in \mesh \right\}, \\
		\spaceQh &= \left\{ \qh \in {Q} \enspace|\enspace \qh|_{K} \in P_m(K), \text{ } K \in \mesh \right\}.
	\end{align}
\end{subequations}

%\begin{align}\label{eq:fem-subspaces-modified}
%\spaceVh &= \left\{ \vvech \in {\mvec{V}}:\  \vvech|_{K} \in \mvec{P_m}(K), \text{ } K \in \mesh \right\}, \\
%\spaceQh &= \left\{ \qh \in {Q} \enspace|\enspace \qh|_{K} \in P_m(K), \text{ } K \in \mesh \right\}.
%\end{align}

For describing the variational problem, we  will use the following symbols for test and trial function pairs:
\begin{subequations}
	\begin{align}
	\phi &:= (\uvec,p) \quad \text{(trial functions)}, \\
	\psi &:= (\vvec,q) \quad \text{(test functions)}.
	%		\omega &:= (\wvec,r) \quad \text{(special trial functions)}
	\end{align}
\end{subequations}

For a given $ \avec \in \spaceVd$, multiplying \eqref{eq:ns-original} by a vector test function $ \vvec \in \spaceV $ and performing integration-by-parts wherever applicable, we have the following bilinear and linear forms $ \bformUnstab(\avec;\upair,\vpair) $ and $ \lform(\avec; \vpair) $: 
%Let us define the bilinear $ \bformUnstab(\avec;\upair,\vpair) $ and the linear form $ \lform(\avec; \vpair) $ for a given convection field $ \avec \in \spaceVd $ as follows:
\begin{subequations}\label{eq:var-problem-b-and-f}
	\begin{align}\label{eq:var-problem-b}
	\bformUnstab(\avec;\upair,\vpair) 
	&= - \inner{\uvec}{\opLTAdv[\avec]\vvec}+\visco\inner{\grad \uvec}{\grad \vvec}-\inner{p}{\grad\cdot \vvec} + \inner{\grad\cdot\uvec}{q} + \inner{\uvec}{\vvec}_{\bft}, \\
	\label{eq:var-problem-f}
	\lform(\vpair) &= \inner{\fvec}{\vvec}.
	\end{align}
\end{subequations}

Substituting $ (\uvec,p) = (\uvech,\ph) + (\uf,\pf) $ (or, $ \phi = \upairh + \upairf $ ) in \eqref{eq:var-problem-b}, we have
\begin{subequations}
	\label{eq:bform-vms-decomp}
	\begin{align}
		\bformUnstab(\avec;\upair,\vpair) &= \bformUnstab(\avec;\upairh,\vpairh) - \innerh{\uf}{\opLTAdv[\avec]\vvech} - \innerh{\pf}{\divergence \vvech} - \innerh{\uf}{\grad \qh} + \innerFTh{\uf}{\vvech} \\
		&= \bformUnstab(\avec;\upairh,\vpairh) - \innerh{\uf}{[\opLTAdv[\avec]\vvech+\grad \qh]} - \innerh{\pf}{\divergence \vvech} + \innerFTh{\uf}{\vvech} .
	\end{align}
\end{subequations}
Now, substituting these expressions for $ (\uf,\pf) $, and also the expression for $ \bformUnstab(\avec;\upair,\vpair) $ (from \eqref{eq:var-problem-b-and-f}) in \eqref{eq:bform-vms-decomp}, we can rearrange the equation as
\begin{align}
\bformh(\avec; \upairh, \vpairh) = \lformh(\avec; \vpairh),
\end{align}
where
\begin{subequations} \label{eq:fem-problem-vms-bh-lh}
\begin{align}
\label{eq:fem-problem-vms-bh}
\begin{split}
\bformh(\avec; \upairh,\vpairh) &= - \inner{\uvech}{\opLTAdv[\avec]\vvech}+\visco\inner{\grad \uvech}{\grad \vvech}-\inner{\ph}{\grad\cdot \vvech} + \inner{\grad\cdot\uvech}{\qh} + \inner{\uvech}{\vvech}_{\bft} \\ &\quad + \innerh{\taum [\opLTAdv[\avec]\uvech-\visco\laplacian\uvech + \grad \ph ]}{[\opLTAdv[\avec]\vvech+\visco\laplacian\vvech +\grad \qh]} \\
&\quad + \innerh{\tauc \divergence \uvech}{\divergence \vvech} -\innerFTh{\taum [\opLTAdv[\avec]\uvech-\visco\laplacian\uvech + \grad \ph ]}{\vvech},
\end{split}
\\
\label{eq:fem-problem-vms-lh}
\lformh(\avec; \vpairh) &= \inner{\fvec}{\vvech} + \innerh{\taum \fvec}{[\opLTAdv[\avec]\vvech-\visco\laplacian\vvech +\grad \qh]} - \innerFTh{\taum \fvec}{\vvech}.
\end{align}
\end{subequations}

Then the stabilized finite element method is to find $ \upairh = (\uvech,\ph) \in \spaceVhd\times\spaceQh $, such that
\begin{align}\label{eq:fem-problem-vms}
\begin{split}
\bformh(\uvech; \upairh, \vpairh) &= \lformh(\upairh;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh.
\end{split}
\end{align}

\begin{remark}
	Note that in \eqref{eq:fem-problem-vms}, a choice of basis functions $ \vpairh = (\vvech, 0) $ will recover the (weak) momentum equations, whereas a choice $ \vpairh = (\zerovec, \qh) $ will recover the (weak) continuity equation.
\end{remark}
\begin{remark}
	Note that for a given $ \avec \in \spaceVhd $, the inner product operators defined in \eqref{eq:fem-problem-vms-bh-lh} are linear, i.e., $ \bformh(\avec;\upairh,\vpairh) $ is linear in both $ \upairh $ and $ \vpairh $; and similarly $ \lform(\avec; \vpairh) $ is linear in $ \vpairh $. However, \eqref{eq:fem-problem-vms} is \textit{nonlinear} since the unknown $ \uvech $ appears in place of $ \avec $.
\end{remark}

\begin{remark}[\textbf{Differences with respect to method of lines discretizations}]
	In a \textit{method of lines} discretization, the time derivative $ \ut $ is discretized using finite differences. Suppose the time interval $ \temporalInterval $ is discretized into $ N $ points $ \{t_i\},\ i=1,\ldots,N $. Using the following notation:
	\begin{align*}
	p_i &= p(\cdot,t_i), \\
	\uvec_i &= \uvec(\cdot,t_i), \\
	\partial_t \uvec_i &= \partial_t \uvec(\cdot,t_i), \\
	\inner{\avec}{\bvec}_i &= \inner{\avec}{\bvec}_{\spDom(t_i)},
	\end{align*}	
	and assuming $ \uvec_D= \zerovec $ in \eqref{eq:ns-original-dirichlet}, the Galerkin formulation of \eqref{eq:ns-original} at $ t= t_{i} $ would be to find $ \uvec_i \in H^1_0(\spDom(t_i)) $ such that
	\begin{align} \label{eq:var-prob-sequential}
	\inner{\ut_{i}}{\vvec}_{i} + \inner{\opLAdv[\uvec_{i}] \uvec_i}{\vvec}_{i} + \visco \inner{\grad \uvec_i}{\grad \vvec}_{i} -\inner{p_i}{\grad\cdot \vvec}_{i} + \inner{\grad\cdot\uvec_i}{q}_{i} = \inner{\fvec_i}{\vvec}_{i}
	\end{align}
	for all $ \vvec \in H^1_0(\spDom(t_i)) $. Comparing \eqref{eq:fem-problem-vms} with \eqref{eq:var-prob-sequential}, we note the following:
	\begin{enumerate}[(i)]
		\item \textit{Multiscale decomposition:} When the VMS method is applied to \eqref{eq:var-prob-sequential}, the following decomposition is assumed:
		\begin{align} \label{eq:vms-decomp-sequential}
		\uvec(\xvec,t_i) &= \uc(\xvec,t_i) + \uf(\xvec,t_i) \\
		\implies \uvec_i &= \uc_i + \uf_i.
		\end{align}
		Therefore, the VMS approximation in a sequential discretization is essentially a \textit{spatial approximation}. However, in the present formulation, the multiscale decomposition becomes a \textit{spatiotemporal} ansatz since we assume
		\begin{align} \label{eq:vms-decomp-st}
		\uvec(\xvec,t) &= \uc(\xvec,t) + \uf(\xvec,t),
		\end{align}
		%\todo{Should we add a comment comparing with LES methodology?}
		
		\item All the inner products appearing in \eqref{eq:var-problem-b-and-f} are over the space-time $ \stDom $, whereas those appearing in \eqref{eq:var-prob-sequential} are over the spatial domain $ \spDom(t_i) $.
		
		\item \textit{The time derivative term:} When the multiscale decomposition \eqref{eq:vms-decomp-sequential} is applied to \eqref{eq:var-prob-sequential}, the time derivative term $ \inner{\ut_i}{\vvec} $ yields
		\begin{align*}
		\inner{\ut_i}{\vvec}_i = \inner{\partial_t \uc_i}{\vvec}_i + \inner{\partial_t \uf_i}{\vvec}_i.
		\end{align*}		
		In \cite{bazilevs2007variational}, it is assumed that
		\begin{subequations}
			\begin{align}
			\inner{\partial_t \uf_i}{\vvec}_i &= 0 \\
			\text{or}\quad \inner{\ut_i}{\vvec}_i &= \inner{\partial_t \uc_i}{\vvec}_i
			\end{align}
		\end{subequations}
		for all $ i $. However, in the current formulation, we \textit{do not} make such an assumption. Noting $ \uvec' (\cdot,t=0) = \zerovec $, we have
		\begin{align*}
		\inner{\ut'}{\vvec} = -\inner{\uvec'}{\vt} + \innerFT{\uvec'}{\vvec}.
		\end{align*}				
		
		\item \textit{The viscous term:} Similarly, the viscous term from \eqref{eq:var-prob-sequential} gives
		\begin{align}
		\inner{\grad \uvec_i}{\grad \vvec}_{i} = \inner{\grad \uc_i}{\grad \vvec}_{i} + \inner{\grad \uf_i}{\grad \vvec}_{i}.
		\end{align}
		In \cite{bazilevs2007variational}, the following projection is assumed on each time slab $ i $:
		\begin{subequations}
			\begin{align} \label{eq:vms-projection-1}
			\inner{\grad\uvec'_i}{\grad \vvec}_{i} &= 0 \\
			\label{eq:vms-projection-2}
			\text{or}\quad\inner{\grad \uvec_i}{\grad \vvec}_{i} &= \inner{\grad \uc_i}{\grad \vvec}_{i}.
			\end{align}
		\end{subequations} 
		In this paper, we \textit{extend this assumption} over the whole spatiotemporal domain $ \stDom $ as
		\begin{align} \label{eq:vms-projection-spacetime}
		\inner{\grad \uvec}{\grad \vvec} = \inner{\grad \uc}{\grad \vvec}.
		\end{align}
		This implies
		\begin{align*}
		0 = \inner{\grad\uvec'}{\grad \vvec} = \intTime \inner{\grad \uf}{\grad \vvec}_{\spDom(t)}\ dt,
		\end{align*}
		or $ \inner{\grad \uf}{\grad \vvec}_{\spDom(t)} = 0 $ almost everywhere in $\temporalInterval$. We have made use of assumption \eqref{eq:vms-projection-spacetime} in deriving the expression for $ B^h $ in \eqref{eq:fem-problem-vms-bh}.
	\end{enumerate}
\end{remark}
\begin{remark}
	The issue of numerical instability due to the time derivative does not become prominent in a conventional time-marching formulation, because the time derivative $ \ut $ is  approximated using either finite differences or time-discontinuous basis functions, but \textit{not} using continuous basis functions.	For example, using a BDF-$ r $ scheme, the time derivative at time $ t_{i} $ is approximated as:
	\begin{align}\label{eq:time-disc-bdf-r}
	\ut_i = \oneOver{\dt} \Xsum_{j=0}^{r} \beta_{j}\uvec_{i-j},
	\end{align}
	where $ \beta_j $ are constants. In the weak formulation, we obtain the following inner product:
	\begin{align}
	\inner{\ut_i}{\vvec}_{\spDom} = \oneOver{\dt} \inner{\left[\Xsum_{j=0}^{r} \beta_{j}\uvec_{i-j}\right]}{\vvec}_{i}.
	\end{align}
	The term $ \inner{\nicefrac{\uvec_{i}}{\dt}} {\vvec}_{\spDom} $ effectively acts a linear ``mass'' term, and adds to the stability of the linear algebra problem.
\end{remark}
\begin{remark}
	The stabilization parameters $ \taum $ and $ \tauc $ are defined element-wise and are intimately related to the transformation Jacobian between element and the master element \cite{hughes1986newBeyondSUPG, shakib1991new, bazilevs2007variational}. Suppose, a ``master'' finite element $ \hat{K} \subset \mathbb{R}^{(d+1)}$ can be transformed into any element $ K\in\mesh $ through an affine transformation. Then for $ \hat{x}_i \in \hat{K} $ and $ x_j \in K$, we define the tensors $ \mvec{T},\ \mvec{G} $ and $ \gvec $ as follows:
	\begin{subequations} \label{eq:transform-tensors}
		\begin{align}
		T_{ij} &= \frac{\partial \hat{x}_i}{\partial x_j}, \ \ i,j=1,2,\ldots,(d+1), \ \ (K\rightarrow\hat{K}), \\
		G_{ij} &= T_{ki}T_{kj},\ \ i,j=1,2,\ldots,(d+1),\\
		g_i &= \Xsum_{j = 1}^{d+1} T_{ij}.
	\end{align}
	\end{subequations}
	Given a convection field $ \avec $ in element $ K $, we can define the \textit{spatiotemporal convection} as
	\begin{align} \label{eq:augmented-advection}
		\widetilde{\avec} := (\avec, 1),
	\end{align}
	where the ``1'' denotes the coefficient of $ \ut $ in \eqref{eq:ns-original-momentum} (convection in time). Using the quantities in \eqref{eq:transform-tensors} and \eqref{eq:augmented-advection}, $ \taum $ and $ \tauc $ are calculated by
	\begin{subequations} \label{eq:taum-tauc}
		\begin{align}
		\taum &= \left[(\widetilde{\avec} \cdot\mvec{G}) \widetilde{\avec}+ C_I \visco^2 (\mvec{G}:\mvec{G}) \right]^{-\halfnice} \\
		\tauc &= \frac{1}{\taum (\gvec \cdot \gvec)},
	\end{align}
	\end{subequations}
	\begin{subequations} \label{eq:taum-tauc-codina}
		\begin{align}
			\taum &= \left[ \frac{c_1\cinv^2\visco}{h^2} + \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} \right]^{-1}, \\
			\tauc &= c_4 \cinv^2\visco + c_5 |\widetilde{\avec}|_{\infty} h,
		\end{align}
	\end{subequations}
	where the inner products $ \mvec{G}:\mvec{G} $ and $ \gvec\cdot \gvec $ are the defined  as
	\begin{align*}
	\mvec{G}:\mvec{G} &= G_{ij}G_{ij}, \\
	\gvec\cdot \gvec &= g_i g_i,
	\end{align*}
	and $ C_I $ is a constant value for which the inverse Poincare inequality holds for each element in the mesh \cite{johnson2012numerical}.
\end{remark}

%\subsection{VMS Assumptions}\label{sec:vms-assumptions}
%One major assumption made in \cite{bazilevs2007variational}, is that $\timeder{\uf{i}}=0$. We do not make that assumption here.
%
%But we still assume the following:
%\begin{itemize}
%    \item $\uf{i}=0$ on the boundaries.
%    \item $\inner{\grad w}{2\visco\grad^s\uf{i}}=0$
%\end{itemize}

%\subsection{VMS Weak form}\label{sec:weak-form-vms}
%The VMS formulation of equations \ref{eq:weak-form-nostab-momentum} and \ref{eq:weak-form-nostab-continuity} is as follows:
%%\begin{align}\label{eq:weak-form-momentum-vms}
%%\begin{split}
%%    \inner{w}{\timeder{\ui}} 
%%    &+ \inner{w}{\uvec\cdot\grad\ui}+\visco\inner{\grad w}{\left[\grad \ui + 
%%\frac{\partial}{\partial \xii}(\uvec)\right]}-\inner{\partialder{w}{\xii}}{p} 
%%- 
%%\inner{w}{\fii}\\
%%    &+\taum\inner{\timeder{w}}{\resUi} \mathbf{\color{teal}- 
%%\taum\Big(w,\resUi\Big)_{\bft}}\\
%%    &+\taum\Big(\grad w,\resUi\uvec\Big) 
%%    -\taum\Big(w, \resUvec\cdot\grad \ui\Big) 
%%    -\taum^2\Big(\grad w,\resUi\resUvec\Big)\\
%%    &\hspace{100mm}+\tauc\Big(\partialder{w}{\xii},\grad\cdot\uvec\Big)
%%    = 0
%%\end{split}\\
%%\label{eq:weak-form-continuity-vms}
%%&\hspace{81mm}\inner{q}{\grad\cdot\uvec} + \taum\Big(\grad q, \resUvec\Big)= 0
%%\end{align}
%\begin{align}\label{eq:weak-form-momentum-vms}
%	\inner{w}{R_i^m} &= 0, \text{  }i = 1,2,3 \\
%	\inner{q}{R^c} &= 0
%\end{align}
%where, the inner products on the left are defined as:
%
%%\begin{remark}
%%Equation \ref{eq:weak-form-momentum-vms} is for the $\ith$ momentum equation 
%%($i=1,2,3$) and equation \ref{eq:weak-form-continuity-vms} is for the 
%%continuity equation.
%%\end{remark}
%%\begin{remark}
%%Note that the second inner product on the second line of equation 
%%\ref{eq:weak-form-momentum-vms}, i.e., $\mathbf{\color{teal}- 
%%\taum\Big(w,\resUi\Big)_{\bft}}$ is with respect to the final time boundary, 
%%i.e., this is a surface integral term. All other inner products in this 
%%equation are with respect to the full space-time domain. In the following 
%%equations, $\mathbf{\color{teal} teal}$ terms will represent surface 
%%integration terms.
%%\end{remark}
%
%
%% The VMS formulation of the continuity equation \ref{eq:weak-form-nostab-continuity} is as follows:
%% \begin{align}
%%     \inner{q}{\grad\cdot\uvec} + \taum\Big(\grad q, \resUvec\Big)= 0
%% \end{align}
%
%
%% \begin{remark}
%% When implementing a Newton iteration for the above formulation, the left hand sides of equations \ref{eq:weak-form-momentum-vms} and \ref{eq:weak-form-continuity-vms} represent the function evaluation. That means, if using $\snes$ provided by $\petsc$, then the LHS can be directly coded for the residual (without any negative sign).
%% \end{remark}
%
%%In the following section, we derive the Jacobian matrix for the residuals 
%%represented by the LHS of \ref{eq:weak-form-momentum-vms} and 
%%\ref{eq:weak-form-continuity-vms}.
%
%%\subsection{Residual}\label{sec:residual-vms}
%%The residuals for Newton iteration can be represented as (these are basically 
%%the left hand sides of \ref{eq:weak-form-momentum-vms} and 
%%\ref{eq:weak-form-continuity-vms}):
%%\begin{align}
%%\label{def:vms-momentum-residual-0}
%%    \begin{split}
%%    R^m_i &= \inner{w}{\timeder{\ui}} 
%%    + \inner{w}{\uvec\cdot\grad\ui}+\visco\inner{\grad w}{\left[\grad \ui + 
%%\frac{\partial}{\partial \xii}(\uvec)\right]}-\inner{\partialder{w}{\xii}}{p} 
%%- 
%%\inner{w}{\fii}\textbf{\color{blue}(original)}\\
%%    &\hspace{10mm}+\taum\inner{\timeder{w}}{\resUi}
%%    \mathbf{\color{teal}-\taum\Big(w,\resUi\Big)_{\bft}} 
%%\textbf{\color{blue}(Time stab terms)}\\
%%    &\hspace{10mm}+\taum\Big(\grad w,\resUi\uvec\Big)  
%%\textbf{\color{blue}(Cross term 1)} \\
%%    &\hspace{10mm}-\taum\Big(w, \resUvec\cdot\grad \ui\Big) 
%%\textbf{\color{blue}(Cross term 2)}\\
%%    &\hspace{10mm}-\taum^2\Big(\grad w,\resUi\resUvec\Big) 
%%\textbf{\color{blue}(Reynolds stress term)}\\
%%    
%%&\hspace{10mm}+\tauc\Big(\partialder{w}{\xii},\grad\cdot\uvec\Big)\textbf{\color{blue}(Grad-div
%% stab)}
%%    \end{split}\\
%%    \label{def:vms-continuity-residual-0}
%%    \begin{split}
%%         R^c &= \inner{q}{\grad\cdot\uvec}\textbf{\color{blue}(original)}\\
%%         &\hspace{10mm}+ \taum\Big(\grad q, \resUvec\Big) 
%%\textbf{\color{blue}(PSPG equivalent stabilization)}
%%    \end{split}
%%\end{align}
%\begin{align}
%\label{def:vms-momentum-residual}
%\begin{split}
%\inner{w}{R^m_i} &= \underbrace{\inner{w}{\timeder{\ui}} 
%	+ \inner{w}{\uvec\cdot\grad\ui}+\visco\inner{\grad w}{\grad 
%	\ui}-\inner{\partialder{w}{\xii}}{p} - 
%	\inner{w}{\fii}\textbf{\color{blue}}}_{\text{original}}\\
%&\hspace{10mm}+\underbrace{\taum\inner{\timeder{w}}{\resUi}
%	-\taum\Big(w,\resUi\Big)_{\bft}}_{\text{temporal-stabilization}}
%	 \\
%&\hspace{10mm}+\underbrace{\taum\Big(\grad w,\resUi\uvec\Big)-\taum\Big(w, 
%\resUvec\cdot\grad \ui\Big) 
%	-\taum^2\Big(\grad w,\resUi\resUvec\Big)}_{(\text{VMS convective 
%	cross terms})} 
%\\
%&\hspace{10mm} + 
%\underbrace{\tauc\Big(\partialder{w}{\xii},\grad\cdot\uvec\Big)}_{\text{Grad-div
% term}}
%\end{split}\\
%\label{def:vms-continuity-residual}
%\begin{split}
%\inner{q}{R^c} &= \underbrace{\inner{q}{\grad\cdot\uvec}}_{\text{original}} + 
%\underbrace{\taum\Big(\grad q, \resUvec\Big)}_{\text{PSPG equivalent term}}
%\end{split}
%\end{align}
%The coarse scale residual $\resUi$ is defined in \ref{eq:coarse-scale-residuals}. The vector $\resUvec$ was defined in \ref{remark:coarse-scale-residual-vector}.
%
%
%\begin{align}
%	\mvec{B}((\wvec, q), (\uvec, p)) - \mvec{F}((\wvec,q)) = \zerovec,
%\end{align}
%
%where $ \mvec{B} $ and $ \mvec{F} $ are defined as:
%
%\begin{align}
%	\begin{split}
%		\mvec{B}\Big((\wvec, q), (\uvec, p)\Big) \\ 
%		&=\underbrace{\inner{\wvec}{\timeder{\uvec}} 
%			+ \innerBig{\wvec}{(\uvec\cdot\grad)\uvec}+\visco\inner{\grad \wvec}{\grad 
%				\uvec}-\inner{\grad\cdot\wvec}{p} + \inner{q}{\grad\cdot\uvec}}_{\text{original}} \\
%		&+\underbrace{\taum\inner{\timeder{\wvec}}{\resUvec}
%			-\taum\inner{\wvec}{\resUvec}_{\bft}}_{\text{temporal-stabilization}} \\
%		&+\underbrace{\taum\Big(\grad w,\resUi\uvec\Big)-\taum\Big(w, \resUvec\cdot\grad \ui\Big)-\taum^2\Big(\grad w,\resUi\resUvec\Big)}_{\text{VMS convective cross terms}}
%	\end{split}
%\end{align}


%\subsection{Jacobian (functional form)}\label{sec:jacobian-vms}
%Let us write the Jacobian for the momentum rows in its functional form, i.e., 
%not worrying about the matrix form right now. Applying the incremental 
%operator 
%$\delta$ to the residual $R^m_i$, we have
%
%\begin{align}\label{def:vms-momentum-jacobian}
%    \begin{split}
%    \delta R^m_i =& 
%    \inner{w}{\timeder{\delta\ui}} \\
%    &+\inner{w}{\delta\uvec\cdot\grad\ui}+ 
%\inner{w}{\uvec\cdot\grad(\delta\ui)}\\
%    &+\visco\inner{\grad w}{\left[\grad (\delta\ui) 
%    + \frac{\partial}{\partial \xii}(\delta\uvec)\right]}\\
%    &-\inner{\partialder{w}{\xii}}{\delta p} 
%    \hspace{60mm}\textbf{\color{blue}(original)}\\
%    &+\taum\inner{\timeder{w}}{\delta[\resUi]}
%    \mathbf{\color{teal}-\taum\Big(w,\delta[\resUi]\Big)_{\bft}} 
%\textbf{\color{blue}(Time stab terms)}\\
%    &+\taum\Big(\grad w,\delta[\resUi]\uvec\Big)+\taum\Big(\grad 
%w,\resUi\delta\uvec\Big)  \textbf{\color{blue}(Cross term 1)} \\
%    &-\taum\Big(w, \delta[\resUvec]\cdot\grad \ui\Big)-\taum\Big(w, 
%\resUvec\cdot\grad (\delta\ui)\Big) \textbf{\color{blue}(Cross term 2)}\\
%    &-\taum^2\Big(\grad w,\delta[\resUi]\resUvec\Big)-\taum^2\Big(\grad 
%w,\resUi\delta[\resUvec]\Big) \textbf{\color{blue}(Reynolds stress term)}\\
%    
%&+\tauc\Big(\partialder{w}{\xii},\grad\cdot(\delta\uvec)\Big)\textbf{\color{blue}(Grad-div
% stab)}
%    \end{split}
%\end{align}
%Similarly applying $\delta$ increment to the continuity residual, we have
%\begin{align}\label{def:vms-continuity-jacobian}
%    \delta R^c &= 
%\inner{q}{\grad\cdot(\delta\uvec)}\textbf{\color{blue}(original)}\\
%         &\hspace{10mm}+ \taum\Big(\grad q, \delta[\resUvec]\Big) 
%\textbf{\color{blue}(PSPG equivalent stabilization)}
%\end{align}


%\end{document}

==> sections/3_implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}
\begin{figure}[!t]
	\centering
	\begin{minipage}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
		% Define coordinates for the corners of the cube
		\coordinate (A) at (0,0,0);
		\coordinate (B) at (2,0,0);
		\coordinate (C) at (2,2,0);
		\coordinate (D) at (0,2,0);
		\coordinate (E) at (0,0,2);
		\coordinate (F) at (2,0,2);
		\coordinate (G) at (2,2,2);
		\coordinate (H) at (0,2,2);
		
		% Draw the edges of the cube
		\draw[thick] (A) -- (B) -- (C) -- (D) -- cycle;
		\draw[thick] (A) -- (E) -- (F) -- (B);
		\draw[thick] (E) -- (H) -- (G) -- (F);
		\draw[thick] (H) -- (D);
		\draw[thick] (C) -- (G);
		
		% Draw markers at the corners
		\foreach \point in {A, B, C, D, E, F, G, H} {
			\fill (\point) circle[radius=2pt];
		}
		
		% Draw x and y axis
		\draw[->] (-1,-1,2) -- (0.3,-1,2) node[anchor=west] {$x$};
		\draw[->] (-1,-1,2) -- (-1,0.3,2) node[anchor=south east] {$y$};
		\draw[->] (-1,-1,2) -- (-1,-1,3.7) node[anchor=south east] {$t$};
		
		%	 % Draw ticks on x axis
		%	 \foreach \x in {-2,-1,1,2}
		%	 \draw (\x,2pt) -- (\x,-2pt) node[anchor=north] {\x};
		%	 
		%	 % Draw ticks on y axis
		%	 \foreach \y in {-2,-1,1,2}
		%	 \draw (2pt,\y) -- (-2pt,\y) node[anchor=east] {\y};
		%	 
		%	 % Label origin
		%	 \node[anchor=north east] at (0,0) {0};
		
		\end{tikzpicture}
		\subcaption{$\spDom \subset \mathbb{R}^2,\ {\stDom} \subset \mathbb{R}^3$}
		\label{fig:q1-3d}
	\end{minipage}
	\hspace{3mm}
	\begin{minipage}{0.65\textwidth}
		\centering
		\begin{tikzpicture}
		\def \hx{+2}
		\def \hy{-3}
		\def \hz{-5}
		\def \axscale{0.6}
		
		% Define coordinates for the corners of the cube
		\coordinate (A) at (0,0,0);
		\coordinate (B) at (2,0,0);
		\coordinate (C) at (2,2,0);
		\coordinate (D) at (0,2,0);
		\coordinate (E) at (0,0,2);
		\coordinate (F) at (2,0,2);
		\coordinate (G) at (2,2,2);
		\coordinate (H) at (0,2,2);
		
		% Draw the edges of the cube
		\draw[thick] (A) -- (B) -- (C) -- (D) -- cycle;
		\draw[thick] (A) -- (E) -- (F) -- (B);
		\draw[thick] (E) -- (H) -- (G) -- (F);
		\draw[thick] (H) -- (D);
		\draw[thick] (C) -- (G);
		
		% Draw markers at the corners
		\foreach \point in {A, B, C, D, E, F, G, H} {
			\fill (\point) circle[radius=2pt];
		}
		
		\coordinate (I) at (0+\hx,0+\hy,0+\hz);
		\coordinate (J) at (2+\hx,0+\hy,0+\hz);
		\coordinate (K) at (2+\hx,2+\hy,0+\hz);
		\coordinate (L) at (0+\hx,2+\hy,0+\hz);
		\coordinate (M) at (0+\hx,0+\hy,2+\hz);
		\coordinate (N) at (2+\hx,0+\hy,2+\hz);
		\coordinate (O) at (2+\hx,2+\hy,2+\hz);
		\coordinate (P) at (0+\hx,2+\hy,2+\hz);
		
		% Lraw the edges of the cube
		\draw[thick] (I) -- (J) -- (K) -- (L) -- cycle;
		\draw[thick] (I) -- (M) -- (N) -- (J);
		\draw[thick] (M) -- (P) -- (O) -- (N);
		\draw[thick] (P) -- (L);
		\draw[thick] (K) -- (O);
		
		% Lraw markers at the corners
		\foreach \point in {I, J, K, L, M, N, O, P} {
			\fill (\point) circle[radius=2pt];
		}
		
		\draw[dashed] (A) -- (I);
		\draw[dashed] (B) -- (J);
		\draw[dashed] (C) -- (K);
		\draw[dashed] (D) -- (L);
		\draw[dashed] (E) -- (M);
		\draw[dashed] (F) -- (N);
		\draw[dashed] (G) -- (O);
		\draw[dashed] (H) -- (P);
		
		% Draw x and y axis
		\draw[->] (-1,-1,2) -- (0.3,-1,2) node[anchor=west] {$x$};
		\draw[->] (-1,-1,2) -- (-1,0.3,2) node[anchor=south east] {$y$};
		\draw[->] (-1,-1,2) -- (-1,-1,3.7) node[anchor=south east] {$z$};
		\draw[->, dashed] (-1,-1,2) -- (-1+\axscale*\hx,-1+\axscale*\hy,2+\axscale*\hz) node[anchor=west] {$t$};
		
		\end{tikzpicture}
		\subcaption{$\spDom \subset \mathbb{R}^3,\ {\stDom} \subset \mathbb{R}^4$}
		\label{fig:q1-4d}
	\end{minipage}
	\caption{$Q_1$ reference elements in 3D (left) and 4D (right). $ Q_2 $ elements are constructed similarly by adding an extra DOF at the center of the lines in each direction, and then taking tensor product.}
	\label{fig:q1-spacetime-elements}
\end{figure}
The finite element formulation obtained in \eqref{eq:fem-problem-vms} can be readily coded in any existing FEM codebase that supports continuous Galerkin method. In the following section, we use $ H^1 $ finite element spaces based on globally $ C^0 $  Lagrangian basis functions. Schematic diagrams of $ Q_1 $ reference elements in 3D and 4D are shown in \figref{fig:q1-spacetime-elements}. For spatially 2D problems ($ \spDom \subset \mathbb{R}^2 $), the space-time domain is 3-dimensional (i.e., $ \stDom \subset \mathbb{R}^3 $) where the third dimension serves as time. For spatially 3D problems ($ \spDom \subset \mathbb{R}^3 $, $ \stDom \subset \mathbb{R}^4 $), the fourth dimension stands for time. The $ Q_2 $ element in 3D and 4D are obtained similarly, with additional degrees of freedoms.

The inner products in \eqref{eq:fem-problem-vms} are calculated by Gaussian quadrature rules. The inclusion of time in the FEM approximation results in a $ (d+1) $-dimensional mesh. The Gaussain quadrature points  in higher dimensions are obtained simply by taking Cartesian-product of one-dimensional quadrature points. Since this number grows exponentially with respect to the dimension, the integration time spent on one element also grows exponentially. This potentially makes the process of evaluation of the quantities \eqref{eq:fem-problem-vms-bh} and \eqref{eq:fem-problem-vms-lh} very expensive. Thus, it is imperative that these problems are solved by parallel computing, preferably using domain decomposition strategies. %, essentially by letting different processors perform the Gaussian integration on different parts of the space-time domain. An ideal parallelization scheme will be able to provide a perfect balance between the extra time spent per element and the number of elements that each processor gets work on.

\subsection{Space-time domain decomposition and parallelization}
\begin{figure}[!tb]
	\centering
	\begin{minipage}[b]{0.35\textwidth}
		\includegraphics[trim=50 20 650 300, clip, width=\textwidth] {images/cube-whole.png}
		\label{fig:space-time-whole-mesh}
	\end{minipage}
	\hspace{5em}
	\begin{minipage}[b]{0.28\textwidth}
		\includegraphics[trim=200 20 650 300, clip, width=\textwidth] {images/cube-dd-small-2.png}
	\end{minipage}
	\caption{(\textit{Left}) A cubic space-time mesh in $ (2D+t) $. Spatial coordinates are $ (x,y) $, and $ z $ denotes time. (\textit{Right}) domain decomposition in space-time using 8 sub-domains.}
	\label{fig:space-time-dd}
\end{figure}
In this work, we perform domain decomposition over the full space-time mesh. Such full domain decomposition methods have been previously studied in  \cite{hughes1988space, hulbert1990space, LionsEtAl2001, pontaza2004space, tezduyar2006space, tezduyar2008arterial, scovazzi2007stabilized, song2015nitsche, gander2016analysis, dyja2018parallel} in relation to either finite-difference or discontinuous Galerkin methods. The benefit of developing the stabilized space-time continuous Galerkin method is that the space-time mesh can be decomposed without regard to the sequential time levels. Different sub-domains of the mesh contain different time points, but they are all computed in parallel. We have implemented method \eqref{eq:fem-problem-vms} in our in-house MPI-based parallel finite-element analysis software written in C++. The domain decomposition is performed using \parmetis{} \cite{karypis2003parmetis}, and the linear algebra and nonlinear algorithms are implemented using \petsc{} \cite{balay2001petsc}. An example visualization of the space-time domain decomposition is shown in \figref{fig:space-time-dd}. More details on the parallelization and scalability this method can be found 

%To perform our numerical experiments, we have implemented method \eqref{eq:fem-problem-vms} in our in-house scalable parallel finite-element analysis software written in C++. The software is optimized for distributed memory computing. Distributed memory computing is essential for space-time simulations. This is because the FEM data-structures (e.g., nodal coordinates, connectivity matrix, global matrix etc.) associated with a space-time method can be quite large in size. Domain decomposition is essential to make sure that the each processor only stores the data corresponding to its allocated elements. We have used \parmetis{} \cite{karypis2003parmetis} for domain decomposition of the space-time meshes. More details on the practical aspects of solving the set of nonlinear equations and method of continuation can be found in \ref{sec:implementation-moc}.

% The velocity spaces $ \mvec{V} $ or $ \mvec{V}^h $ have the initial and the boundary conditions baked into them. This effectively means that the final linear system must have the initial conditions and the boundary conditions applied exactly. In either case, the IC and BC information is contained in the RHS $ b_g $. There is no initial or boundary condition available for pressure. The space $ Q $ puts only one constraint on pressure, which is a mean value of zero. In practice, the space $ Q $ can be constructed with any mean value, since the Navier-Stokes momentum equations \eqref{eq:ns-original-momentum} only contains a gradient of $ p $. Thus an effective way of applying this condition is through a Dirichlet condition on a node in the mesh. This is discussed in the context of each example provided in \secref{sec:num-examples-results}. More details on the practical aspects of solving the set of nonlinear equations and method of continuation can be found in \ref{sec:implementation-nonlinear-solve} and \ref{sec:implementation-moc}.




==> sections/4_numerical_examples.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
\section{Numerical results}
\label{sec:num-examples-results}
In this section, we demonstrate the method developed herein on a few benchmark problems. 
\subsection{Convergence studies with manufactured solution}
\label{sec:mms-convergence}
To test the accuracy of the method outlined above, we use the method of manufactured solutions for both $ \nsd = 2,3 $. Once again, the spatiotemporal domain (and thus the computational domain) is $ \stDom = \spDom \times \temporalInterval $. For the convergence studies, we take $ \temporalInterval = [0,1] $. For both $ \nsd = 2,3 $, we choose divergence-free velocities.
\subsubsection{2D example (3D in space-time) [$\spDom \subset \mathbb{R}^2,\ \stDom \subset \mathbb{R}^3$]}
\label{sec:mms-2d}
\input{sections/900_convergence_mms.tex}
% \input{sections/901_comparison_re500.tex}
% \input{sections/902_comparison_re1000.tex}
In two spatial dimensions (i.e., $\spDom \subset \mathbb{R}^2,\ \stDom \subset \mathbb{R}^3$), we take the exact solution $ (u_x, u_y, p) $ to be
\begin{subequations}
    \begin{align}
    	u_x &= \sin(\pi x) \cos(\pi y) \sin(\pi t), \\
    	u_y &= -\cos(\pi x) \sin(\pi y) \sin(\pi t), \\
    	p &= \sin(\pi x) \sin(\pi y) \cos(\pi t).
    \end{align}
\end{subequations}
The velocity vector $\mvec{u} = (u_x, u_y) $ readily satisfies $ \grad\cdot\mvec{u} = 0 $. We obtain the right hand side forcing $ \mvec{f} $ by substituting these exact solutions $ (u_x, u_y, p) $ in  \eqref{eq:ns-original}. With the obtained forcing $ \mvec{f} $, we now solve  \eqref{eq:fem-problem-vms} using both linear ($ Q_1 $) and quadratic ($ Q_2 $) finite elements in 3D. The computational domain is based on $\stDom$, therefore the FEM problem is solved on a 3D mesh. The resulting errors in the $ L^2(\stDom) $-norm are presented for three different Reynolds numbers in  \figref{fig:conv-study-uniref-linear-basis} (for $ Q_1 $ elements) and in  \figref{fig:conv-study-uniref-quadratic-basis} (for $ Q_2 $ elements). On these $ \log-\log $ plots, we notice a slope of 2 for linear $ Q_1 $ elements and a slope of 3 for $ Q_2 $ elements. We also notice that the rate of convergence in this problem is independent of the Reynolds number. This result can be compared with the convergence estimates provided in \thmref{thm:convergence}. It can be seen that the error estimates provided therein under-predict the order of convergence because of the choice of a different norm.

\subsubsection{3D example (4D in space-time) [$\spDom \subset \mathbb{R}^3,\ \stDom \subset \mathbb{R}^4$]}
\label{sec:mms-3d}
In \emph{three} spatial dimensions (i.e., $\spDom \subset \mathbb{R}^3,\ \stDom \subset \mathbb{R}^4$), we take the exact solution $ (u_x, u_y, u_z, p) $ to be
\begin{subequations}
    \begin{align}
    	u_x &= \sin(\pi x) \cos(\pi y) \cos(\pi z) \sin(\pi t), \\
    	u_y &= -\cos(\pi x) \sin(\pi y) \cos(\pi z) \sin(\pi t), \\
        u_z &= \cos(\pi x) \sin(\pi y) \cos(\pi t), \\
    	p &= \sin(\pi x) \sin(\pi y) \sin(\pi z) \cos(\pi t).
    \end{align}
\end{subequations}
Once again, the velocity vector $\mvec{u} = (u_x, u_y, u_z) $ readily satisfies $ \grad\cdot\mvec{u} = 0 $. The forcing $ \fvec $ is obtained in the same way as for $\nsd=2$ (previous subsection). But now we use tesseract-like elements (see \figref{fig:q1-4d}, both $ Q_1 $ and $ Q_2 $) to solve this problem. The $L^2(\stDom)$-norm of the errors in the velocities and the pressure are plotted against the mesh size in \figref{fig:conv-study-uniref-linear-basis-4d}. Once again, $ Q_1 $ elements yield an order of convergence of 2 for all variables. However, $ Q_2 $ elements yield an order of convergence of 3 for the velocities, but 2 for pressure.


%\subsection{Benchmark problems}
\subsection{Lid Driven Cavity Flow}
Next, we test the present method on the well-known ``lid-driven cavity'' problem, for both $\nsd = 2, 3.$

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.23\textwidth}
		\raisebox{-5cm}{\includegraphics[width=\textwidth]{images/ldc-2d-schematic.png}}
		\caption{$\spDom = [0,1]^2$}
		\label{fig:ldc-schematic-2d-spatial}
	\end{subfigure}
	\hspace{5em}
	\begin{subfigure}[b]{0.5\textwidth}
		\begin{tikzpicture}
		\draw (0, 0) node[inner sep=0] {\includegraphics[trim=0 0 80 0, clip, width=\textwidth] {images/ldc-schematic.PNG}};
		\draw (4.7, -3.5) node {$t=T$};		
		\end{tikzpicture}
		\caption{$\stDom = \spDom\times [0,T]$}
		\label{fig:ldc-schematic-2d-space-time}
	\end{subfigure}
	\caption{Two dimensional lid-driven cavity problem. The spatial domain is shown in $\spDom$. All sides are no-slip, except the top surface where $u_x = 1$. The ``space-time'' computational domain is shown in (b), along with all the boundary conditions.}
	\label{fig:ldc-schematic-2d}
\end{figure}

%\input{sections/1001_LDC_setup.tex}

%\input{sections/1007_LDC_benchmark_comparison_re_all.tex}
\input{sections/1007_LDC_benchmark_comparison_re_all_singleplot.tex}
\subsubsection{2D example (3D in space-time) [$\spDom \subset \mathbb{R}^2,\ \stDom \subset \mathbb{R}^3$]}
\label{sec:ldc2d}

\figref{fig:ldc-schematic-2d-space-time} shows a schematic of the ``2D 
version'' of this problem, where $\spDom = [0,1]^2$, and $\stDom = [0,1]^2 \times [0,T]$. The benchmark results for this problem generally refer to the steady-state solution. Thus, the final time $ T $ is chosen such that a steady state is achieved, i.e., $ \partial_t u_i = 0,\ i=1,\ 2 $ for some $ t = t_s $; with $ T $ being strictly larger than  $ t_s $. The ``steady-state'' time value ($ t_s $) increases with increase 
in the Reynolds number, thus $ T $ also grows with $ Re $. In the present work, the time-horizon values 
chosen for the space-time simulations of this problem are $ T =  180, 180, 360, 720$ for $ Re = 1000,\ 3200,\ 5000,\ 7500 $ respectively.

%As the value of the Reynolds number grows, a central vortex develops in the domain, along with boundary layers near all spatial boundaries. Thus a higher mesh refinement is needed near the spatial boundaries. This is shown in  \figref{fig:ldc_mesh_c2}. This spatial-boundary refinement can be done independent of any refinement in the temporal direction. It is important to note that a higher temporal refinement is helpful in resolving the initial transient behavior as well as an accurate solution at the final time. A typical spatio-temporal mesh with all boundary refinement is shown in  \figref{fig:ldc_mesh_c3}. All the following results on this problem are obtained on boundary-refined clustered meshes.

\figref{fig:ldc-re-all-panel-1} shows the results obtained for different Reynolds numbers, $ Re = 1000,\ 3200,\ 5000,\ 7500 $. The left column plots the horizontal velocity $ u_x $ on a vertical line at $ x = 0.5 $ and $ t = T $, in other words, $ u_x(x=0.5, y, t=T) $ vs. $ y $. And similarly the right column plots $ u_y(x, y=0.5, t=T) $ vs. $ x $. The results in \figref{fig:ldc-re-all-panel-1} are compared with reference solutions found in \cite{ghia1982high}.

%\input{sections/1002_LDC_benchmark_comparison_re1000.tex}
%\input{sections/1003_LDC_benchmark_comparison_re3200.tex}
%\input{sections/1004_LDC_benchmark_comparison_re5000.tex}
%\input{sections/1005_LDC_benchmark_comparison_re7500.tex}
%\input{sections/1006_LDC_benchmark_comparison_re10000.tex}

\subsubsection{3D example (4D in space-time), [$\spDom \subset \mathbb{R}^3,\ \stDom \subset \mathbb{R}^4$]}
\label{sec:ldc3d}

A schematic diagram of the driven cavity problem in three dimensions is shown in \figref{fig:ldc-schematic-3d}, where $\spDom = [0,1]^3$ and $\stDom =\spDom \times [0,T]$. The boundary conditions are given by:
\begin{subequations}
\label{eq:ldc3d-bc}
\begin{align}
u_x &= \begin{cases}
1 \ \text{at}\ y=1, \\
0 \ \text{elsewhere}, \\
\end{cases} \\
u_y=u_z &= 0 \ \text{on all surfaces}.
\end{align}
\end{subequations}
We solve \eqref{eq:fem-problem-vms} along with \eqref{eq:ldc3d-bc} for $ \visco = 0.002 $ (or $ Re = 500 $) using a mesh of $ 32^3 \times 100 $ $ Q_1 $ tesseract elements (see \figref{fig:q1-4d}). Temporal slices of the streamlines are shown in \figref{fig:ldc-3d-streamlines}.
\begin{figure}[!b]
	\centering
	\begin{subfigure}[b]{0.3\textwidth}
		\raisebox{-5cm}{\includegraphics[width=\textwidth]{images/ldc-3d-schematc.png}}
		% \caption{$\spDom = [0,1]^3$}
		% \label{fig:ldc-schematic-3d-spatial}
	\end{subfigure}
	\caption{Three dimensional lid-driven cavity problem. The spatial domain is $\spDom = [0,1]^3$. All sides are no-slip, except the $y=1$ surface where $u_x = 1$. The computational domain $\stDom = \spDom \times [0,T]$ is four-dimensional.}
	\label{fig:ldc-schematic-3d}
\end{figure}

%\begin{figure}[!b]
%	\centering
%	\begin{subfigure}[b]{0.9\textwidth}
%		\includegraphics[trim=280 50 175 80,clip, width=\textwidth]{data_files/ldc3d/re500/re500-tspan2p5-vmag.png}
%		% \caption{$\spDom = [0,1]^3$}
%		% \label{fig:ldc-schematic-3d-spatial}
%	\end{subfigure}
%	\caption{Contours of $|\uvec |$ after solving the lid-driven cavity problem in 3D. The computational domain is 4D, therefore, only a $z$-constant slice ($z=0.5)$ is shown here.}
%	\label{fig:ldc-3d}
%\end{figure}

\begin{figure}[!t]
	\centering
	\begin{subfigure}[b]{0.99\textwidth}
		\includegraphics[trim=0 50 0 0,clip, width=\textwidth]{data_files/ldc3d/re500/combined-2.pdf}
		% \caption{$\spDom = [0,1]^3$}
		% \label{fig:ldc-schematic-3d-spatial}
	\end{subfigure}
	\caption{Temporal slices of streamlines (colored by the velocity magnitured $|\uvec |$) after solving the lid-driven cavity problem in 3D. The computational domain is 4D.}
	\label{fig:ldc-3d-streamlines}
\end{figure}


\subsection{Flow past a circular cylinder}
\subsubsection{Problem definition}
%\begin{figure}[!tb]
%	\centering
%	\begin{minipage}[b]{0.6\textwidth}
%		\includegraphics[width=\textwidth]{images/fpc-space.PNG}
%		\caption{Flow past a circular cylinder (2D): problem definition in 
%			space}
%		\label{fig:fpc-schematic-space}
%	\end{minipage}
%\end{figure}
%\begin{figure}[!tb]
%	\centering
%	\begin{minipage}[b]{0.7\textwidth}
%		\includegraphics[width=\textwidth]{images/fpc-schematic-1.png}
%		\caption{Flow past a circular cylinder: problem definition in 
%			space-time}
%		\label{fig:fpc-schematic-space-time}
%	\end{minipage}
%\end{figure}
\begin{figure}[!tb]
	\centering
	\begin{minipage}[b]{0.39\textwidth}
		\includegraphics[width=\textwidth]{images/fpc-space.PNG}
%		\subcaption{\small $ 2 $D spatial domain for flow past a cylinder.}
%		\label{fig:fpc-spatial-domain}
	\end{minipage}
	\begin{minipage}[b]{0.49\textwidth}
		% \includegraphics[width=\textwidth]{images/fpc-schematic-1.png}
		\includegraphics[trim=120 50 75 140, clip, width=\textwidth]{images/fpc-spacetime-schematic-2.pdf}
%		\subcaption{\small $ (2 + 1) $D Spatiotemporal domain}
%		\label{fig:fpc-space-time-domain}
	\end{minipage}
	\caption{Schematic diagram of the flow past a circular cylinder problem: 
	(left) spatial domain, (right) spatiotemporal domain.}
	\label{fig:fpc-schematic-2d}
\end{figure}

\begin{figure}[!tb]
	\centering
	\begin{minipage}[b]{0.6\textwidth}
		% \includegraphics[width=\textwidth]{data_files/FPC_study/fpc_mesh_setup_const-ver2.png}
		\includegraphics[trim=200 20 200 20, clip, width=\textwidth] {images/sample-mesh-2.png}
		\caption{Space-time mesh with hexahedral elements}
		\label{fig:fpc_mesh_const}
	\end{minipage}
	% \hfill
	% \begin{minipage}[b]{0.45\textwidth}
	% 	\includegraphics[width=\textwidth]{data_files/FPC_study/fpc_mesh_setup_prog-ver2.png}
	% 	\caption{Space-time mesh with clustering in time dimension}
	% 	\label{fig:fpc_mesh_prog}
	% \end{minipage}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
	\centering
	\caption{Benchmark configurations}
	\label{tab:expt-config}
	\begin{tabular}{@{}c|ccc|ccc|c|cc|cc@{}}
		\toprule[2pt]
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Reference\\ text\end{tabular}} & \multirow{2}{*}{$D$} & \multirow{2}{*}{$H/D$} & \multirow{2}{*}{$L/D$} & \multirow{2}{*}{$u_c$} & \multirow{2}{*}{$u_{ref}$} & \multirow{2}{*}{$\nu$} & \multirow{2}{*}{$Re = \frac{u_{ref}D}{\visco}$} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Reference\\ values\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Computed\\ values\end{tabular}} \\ \cmidrule(l){9-12} 
		&  &  &  &  &  &  &  & $C_d$ & $St$ & $C_d$ & $St$ \\  \midrule[2pt]
		\multirow{2}{*}{\cite{schafer1996benchmark}} & \multirow{2}{*}{0.1} & \multirow{2}{*}{4.1} & \multirow{2}{*}{22} & 0.3 & 0.2 & $10^{-3}$ & 20 & 5.57 & - & 5.64 & - \\ \cmidrule(l){5-12} 
		&  &  &  & 1.5 & 1.0 & $10^{-3}$ & 100 & 3.22 & 0.295 & 3.12 & 0.29 \\ \midrule[1pt]
		\multirow{2}{*}{\cite{kanaris2011three}} & \multirow{2}{*}{1} & \multirow{2}{*}{5} & \multirow{2}{*}{40} & 1 & 1 & $ \nicefrac{1}{15} $ & 15 & 3.11 & - & 3.24 & - \\ \cmidrule(l){5-12} 
		&  &  &  & 1 & 1 & $ \nicefrac{1}{100} $ & 100 & 1.30 & 0.17 & 1.36 & 0.17 \\ \bottomrule[2pt]
	\end{tabular}
\end{table}

Next, we test our method on the problem of two-dimensional flow past a circular 
cylinder. The setup is taken from \cite{schafer1996benchmark,kanaris2011three,zovatto2001flow}. The schematic of the problem is shown in  
\figref{fig:fpc-schematic-2d}. The spatial domain is $ \spDom = ((I_x\times I_y) \backslash C) $, where $ I_x = [0,L],\ I_y = [0,H] $ and $ C $ denotes a circle of diameter $ {\spDom}_{cyl} $ with center at $ (x_c,y_c) $. The space-time domain $ \stDom = \spDom \times I_t $.
The boundary conditions are specified as:
\begin{subequations}
	\label{eq:fpc-boundary-conditions}
	\begin{align}
	&\text{at } x=0:\enspace u_x(y,t) = \sigma(y),  \quad u_y(y,t) = 0, \\
	&\text{at } x=L:\enspace \normalvec\cdot(p \mmat{I} + \visco \grad \uvec) = 0, \\
	&\text{at } y = 0,\ H:\enspace u_x(y,t) = u_y(y,t) = 0, \\
	&\text{on } C:\enspace u_x(y,t) = u_y(y,t) = 0,
	\end{align}
\end{subequations}
where the inlet flow profile $ \sigma(y) $ is given by
\begin{align}\label{eq:fpc-inlet-vel}
	\sigma(y) = 4 u_c H (y-H) / H^2,
\end{align}
which is a parabolic profile with $ \sigma(0) = \sigma(H)=0 $ and $ \sigma_m := \sigma(\nicefrac{H}{2}) = u_c $. The average inlet velocity is given by $ \bar{\sigma} = \nicefrac{2}{3} u_c $. The force on the cylinder in the direction $ \wvec $ is expressed as
\begin{align}
F_w = \int_{\Gamma_C} \left[ \left( \visco [\grad \uvec + \grad \uvec^T] -p \mathbb{I}\right) \normalvec \right]\cdot \wvec \ dS.
\end{align}
We set $ \wvec = (1,0) $ to extract the drag force, and $ \wvec = (0,1) $ to extract the lift force.

We compare our results against two different setups. These are summarized in \tabref{tab:expt-config}. The first setup is taken from \cite{schafer1996benchmark}, where the viscosity is kept constant, and the Reynolds number is changed by changing the inlet velocity. The second setup is taken from \cite{kanaris2011three}. The Reynolds number for this problem is defined as $ Re = \frac{U_{ref} D}{\nu}$. $ U_{ref} = \bar{\sigma} = \nicefrac{2}{3} u_c $ in the first setup, and $ U_{ref} = \sigma_m = u_c $ in the second setup.
%For this problem, there exists a critical Reynolds number $ Re_{cr} \approx 50 $ below which the flow is laminar and reaches a steady state after a certain time $ T $ \cite{zdravkovich1997flow}. But for higher Reynolds numbers, the wake becomes unstable with periodic oscillations.

We solve \eqref{eq:fem-problem-vms} along with \eqref{eq:fpc-boundary-conditions} using hexahedral $ Q_1 $ elements. \figref{fig:fpc_mesh_const} shows a mesh obtained by discretizing the domain $ \stDom $. For solving the nonlinear system of equations using the Newton-Raphson method, an initial guess is required. Note that the initial guess here refers to a guess for the entire space-time mesh. Coming up with a meaningful guess is non-trivial. In the present case, the initial guess was set to zero for all the nodes in the mesh, except those on the Dirichlet boundaries (this includes the initial-time boundary). Even with this simple initial guess, the Newton-Raphson method is successful in reaching a spatiotemporal solution for this problem.

\subsubsection{Results}
%\begin{figure}[!tb]
%	\centering
%	\includegraphics[trim=0 0 0 0,clip, width=0.75\textwidth]{data_files/FPC_study/fpc-Re20-streamlines.png}
%	\caption{Streamlines for FPC with Re=20}
%	\label{fig:fpc_Re20_streamlines}
%\end{figure}
We present results for $ 20 \leq Re \leq 400 $. Benchmark comparisons are presented in \tabref{tab:expt-config} and in \figref{fig:fpc-2d-validation}. \tabref{tab:expt-config} summarizes the mean coefficient of drag $ C_d $ and the Strouhal number $ St $ for one steady and one unsteady case each taken from \cite{kanaris2011three} and \cite{schafer1996benchmark}. A more extensive comparison (based on the setup of \cite{kanaris2011three}) is presented in \figref{fig:fpc-2d-validation}, including additional references. For $ Re > 50 $, the solution $ (\uvech,\ph) $ reach a time-periodic state after an initial transient phase. To obtain this result in a space-time simulation as discussed in \secref{sec:formulations}, we need to choose the domain as a tensor product of the spatial domain $ \spDom = (I_x\times I_y)\backslash C $ and the time interval $ I_T = [0,T] $ such that $ T > t_c $ or $ [0,t_c] \subset I_T $ (see  \figref{fig:fpc-schematic-2d}).
\begin{figure}[!tb]
	\centering
	\begin{minipage}{0.49\textwidth}
		\centering
		\includegraphics[trim=0 70 0 0,clip, width=0.9\linewidth]{data_files/FPC_study/fpc_vel_x-Re20.png}
		\subcaption{$ u_x $}
		\label{fig:fpc_Re20_velx}
	\end{minipage}
	\begin{minipage}{0.49\textwidth}
		\centering
		\includegraphics[trim=0 70 0 0,clip, width=0.9\linewidth]{data_files/FPC_study/fpc_vel_y-Re20.png}
		\subcaption{$ u_y $}
		\label{fig:fpc_Re20_vely}
	\end{minipage}
	\caption{Velocity contours for flow past a circular cylinder, $ Re = 20 $.}
	\label{fig:fpc_Re20_velocities}
\end{figure}
\begin{figure}[!tb]
	\centering
	\begin{minipage}{0.49\textwidth}
		\centering
		\includegraphics[trim=0 70 0 0,clip, width=0.99\linewidth]{data_files/FPC_study/fpc_vel_x0000-ver2.png}
		\subcaption{$ u_x $}
		\label{fig:fpc_Re100_velx}
	\end{minipage}
	\begin{minipage}{0.49\textwidth}
		\centering
		\includegraphics[trim=0 70 0 0,clip, width=0.99\linewidth]{data_files/FPC_study/fpc_vel_y0000-ver2.png}
		\subcaption{$ u_y $}
		\label{fig:fpc_Re100_vely}
	\end{minipage}
	\caption{Velocity contours for flow past a circular cylinder, $ Re = 100 $.}
	\label{fig:fpc_Re100_velocities}
\end{figure}

\figref{fig:fpc_Re20_velocities} and \figref{fig:fpc_Re100_velocities} show temporal slices of the velocity solutions for $ Re=20 $ and $ Re = 100 $ respectively.
Both show an $ x-t $ slice (at $ y=H/2 $) and several $ x-y $ slices at multiple $ t $-values of the 3D domain. The $ x-t $ slice at $ y=H/2 $ is seen on the left, with the time-axis extending upward. This slice shows the solution $ u_x(x,t)|_{y=H/2} $ evolving in time. Also, the slices in \figref{fig:fpc_Re20_velocities} show the emergence of a steady state, whereas those in \figref{fig:fpc_Re100_velocities} show that the solution exhibits some signs of periodicity around $ t=50 $ and really falls into a periodic pattern roughly around $ t>70 $.

%\input{sections/2001_FPC_Re100_forces.tex}
%\input{sections/2002_FPC_Re100_forces_clustered.tex}
%\input{sections/2003_FPC_Re_study.tex}
%\input{data_files/FPC_study/St_table}
\input{data_files/FPC_study/cd-st-plots.tex}

%\subsection{Solving with large space-time blocks}

%\subsection{Clustered meshes}
%$ <\text{pending}> $
%One of the way to leverage the FEM approximation in the time dimension is to refine the mesh in time 

%\input{sections/1008_LDC_benchmark_comparison_re_all_2.tex}
%\end{document}

==> sections/5_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we present a method for solving flow problems in space-time using continuous Galerkin finite element method. At the discrete level, such a problem can become unstable when the equation is dominated by the convection term. Also, applying equal-order finite elements for both velocity and pressure can render a non-trivial null space for the pressure solution, thus running into non-uniqueness of pressure. Both these problems can be resolved by formulating the FEM problem using a variational multiscale approach. The application of VMS provides stability against both spatial advection as well as temporal advection (i.e., the time derivative term). It also transforms the saddle point operator into a coercive operator, thus restoring the uniqueness of solutions.

As shown in the numerical results in this paper, the proposed method is able to provide convergence rates as expected. The convergence is both in space and in time. The convergence rate is found to be independent of the Reynolds number. We also tested the method on two benchmark problems, namely, the lid driven cavity problem and the flow past a cylinder problem. Both problems displayed satisfactory results that match previously reported results in the literature.

It can be argued that, everything else being equal, a space-time solution is more expensive than a marching solution for the same problem. But this increased complexity of computation also gives us an opportunity to leverage the scaling capabilities of modern codebases designed for supercomputing facilities. Since the entire time-horizon is included in the mesh, a space-time mesh is extremely well-suited for domain-decomposed analyses. Therefore, even though currently a singular marching simulation is cheaper than a single space-time simulation, it can be shown \cite{ishii2019solving} that with a proper design of scalable codes and proper selection of supercomputing resources, the time-cost of solving PDEs in space-time can be significantly reduced in comparison to time-marching approaches.

==> sections/s_analysis.tex <==
\section{Analysis of the variational problem} \label{sec:analysis}
\subsection{Overview} \label{sec:anlys-overview}
In this section, we present an analysis of the boundedness, stability and convergence of the FEM problem \eqref{eq:fem-problem-vms}. For this, we will use the following linearized form of \eqref{eq:fem-problem-vms} where the convection field $ \avec \in \spaceVhd$ is known \textit{a priori} (recall $ \upairh=(\uvech,\ph)\in \spaceVhd\times \spaceQh $):
\begin{align}\label{eq:fem-problem-lin-vms}
\begin{split}
\bformh(\avec; \upairh, \vpairh) &= \lformh(\upairh;\vpairh) \quad \forall \vpairh=(\vvech,\qh) \in \spaceVh \times \spaceQh,
\end{split}
\end{align}
where $ \bformh $ and $ \lformh $ are defined in \eqref{eq:fem-problem-vms-bh-lh}. The analysis in this section closely follows that presented in \cite{zhou1993least}.
%\begin{align}
%\label{eq:fem-problem-vms-lin-bh}
%\begin{split}
%\bformh(\avec; \upairh,\vpairh) &= \bformUnstab(\avec; \upairh,\vpairh) + \innerh{\taum [\opLTAdv[\avec]\uvech+\visco\laplacian\uvech + \grad \ph ]}{[\opLTAdv[\avec]\vvech-\visco\laplacian\vvech +\grad \qh]} + \innerh{\tauc \divergence \uvech}{\divergence \vvech} \\
%&\quad -\innerFTh{\taum [\opLTAdv[\avec]\uvech-\visco\laplacian\uvech + \grad \ph ]}{\vvech},
%\end{split}
%\\
%\label{eq:fem-problem-vms-lin-lh}
%\lformh(\avec; \vpairh) &= \inner{\fvec}{\vvech} + \innerh{\taum \fvec}{[\opLTAdv[\avec]\vvech-\visco\laplacian\vvech +\grad \qh]} - \innerFTh{\taum \fvec}{\vvech}.
%\end{align}

Some preliminaries are summarized in \secref{sec:anlys-prelim}, and the main results are presented in \secref{sec:anlys-results}. A brief overview of the results is as follows:
\begin{enumerate}[\itshape(a)]
	\item We first prove that for a given convection field $ \avec $, the term $ \bformh $ appearing in \eqref{eq:fem-problem-lin-vms} is coercive with respect to the solution $ \uvech $ (\lemref{thm:coercivity}). This also implies that for each given $ \avec $, \eqref{eq:fem-problem-lin-vms} yields a unique solution (\cororef{thm:uniqueness-linearized}).
	\item Next we prove that \eqref{eq:fem-problem-lin-vms} defines a continuous map $ F:\avec\rightarrow \upairh $ (\lemref{thm:map-continuity}). By using Brouwer's fixed point theorem, we then prove that there exists at least one fixed point of \eqref{eq:fem-problem-vms}, such that $ \upairh = F(\upairh) $ (\lemref{thm:existence-nonlinear}).
	\item We then prove that the nonlinear solution, i.e., the fixed point solution of \eqref{eq:fem-problem-vms} is unique (\thmref{thm:uniqueness}).
	\item \label{blah} Finally, we determine the order of convergence of the FEM problem \eqref{eq:fem-problem-vms} in terms of the mesh size $ h $ (\thmref{thm:convergence}).
\end{enumerate}

\subsection{Preliminaries} \label{sec:anlys-prelim}
Before stating the lemmas and theorems, we note a few preliminaries:
\begin{enumerate}[\itshape(I)]
	\item \label{item:discrete-norm} \textit{Discrete norm:} We choose the following discrete norm to prove stability and convergence of the FEM problem \eqref{eq:fem-problem-vms}:
	\begin{align}
	\normVW{\upairh} := \left[ \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec] \uvech + \grad \ph]}^2\right]^{\halfnice}.
	\end{align}
	Note that this norm is dependent on the mesh, the convection field $ \avec $, as well as the choice of the stabilization parameter $ \taum $. The definition of $ \normh{\cdot} $ is given in \eqref{eq:discrete-norms}.
	
	
	\item \label{item:convection-op} \textit{The convection operator:} The operators $ \opLAdv[\avec] $ and $ \opLTAdv[\avec] $ defined in \eqref{eq:opL} and \eqref{eq:opLT} are linear in $ \uvec $. For two advection fields $ \avec^1 $ and $ \avec^2 $, we denote the difference by $ \davec = \avec^1-\avec^2 $. Then we have,
	\begin{align*}
	\opLTAdv[\avec^1]\uvec - \opLTAdv[\avec^2]\uvec &= (\ut + \opLAdv[\avec^1]\uvec) - (\ut + \opLAdv[\avec^2]\uvec) \\
	&= \opLAdv[\avec^1]\uvec - \opLAdv[\avec^2]\uvec \\
	&= (\ddiv{\avec^1}) \uvec + \halfnice (\divergence \avec^1) \uvec - (\ddiv{\avec^2}) \uvec - \halfnice (\divergence \avec^2) \uvec \\
	&= (\ddiv{\delta \avec^{12}}) \uvec + \halfnice (\divergence \delta \avec^{12}) \uvec \\
	&= \opLAdv[\delta \avec^{12}],
	\end{align*}
	i.e.,
	\begin{align}
	\opLTAdv[\delta \avec^{12}] =\opLTAdv[\avec^1]\uvec - \opLTAdv[\avec^2]\uvec = \opLAdv[\avec^1]\uvec - \opLAdv[\avec^2]\uvec = \opLAdv[\delta \avec^{12}].
	\end{align}
	
	
	\item \label{item:adjoint-op} \textit{Adjoint operators:} The adjoint operators of $ \opLAdv[\avec] $ and $ \opLTAdv[\avec] $ are as follows:
	\begin{subequations}
		\begin{align}
		\opLAdvStar[\avec] &= -\opLAdv[\avec], \\
		\opLTAdvStar[\avec] &= -\opLTAdv[\avec].
		\end{align}
	\end{subequations}
    Indeed, for any $ \eta \in C_c^{\infty}(\stDom) $ (i.e., the space of smooth functions with compact support), we have
	\begin{align*}
	\inner{\opLAdv[\adv]\uvec}{\eta} &= \inner{\left[(\ddiv{\avec}) \uvec + \halfnice (\divergence \avec) \uvec\right]}{\eta} = \inner{\left[(\ddiv{\avec}) \uvec + (\divergence \avec) \uvec\right]}{\eta} - \inner{\halfnice (\divergence \avec)\uvec}{\eta} \\
	&= \inner{\divergence (\uvec\avec^T)}{\eta} - \inner{\halfnice (\divergence \avec)\uvec}{\eta} \\
	&= -\inner{\uvec\avec^T}{\grad\eta} - \inner{\uvec}{\halfnice (\divergence \avec)\eta} \quad \text{[integration by parts on the first term]} \\
	&= -\inner{\uvec}{\left[(\ddiv{\avec}) \vvec + \halfnice (\divergence \avec) \vvec\right]} \\
	&=-\inner{\uvec}{\opLAdv[\avec]\eta}.
	\end{align*}
	And similarly,
	\begin{align}
		\inner{\opLTAdv[\adv]\uvec}{\eta} = \inner{\ut}{\eta} + \inner{\opLAdv[\avec]}{\eta} = -\inner{\uvec}{\partial_t \eta} - \inner{\uvec}{\opLAdv[\avec]\eta} = -\inner{\uvec}{\opLTAdv[\avec]\eta}.
	\end{align}
		
	\item \label{item:tau-max} \textit{Maximum value of} $ \taum $: For a given discretization $ \mesh $, we denote the maximum value of $ \taum $ as
	\begin{align}
	\taumMax = \max_{K \in \mesh} \taum^K.
	\end{align}
	
	\item \label{item:inverse-est} \textit{Inverse estimates:} For any function $ \uvech \in \spaceVh  $, the following inverse estimates hold:
	\begin{subequations}
		\begin{align}
		\normElm{\grad\uvech} &\leq \frac{\cinv}{\he}\normElm{\uvech}, \\
		\normElm{\laplacian\uvech} &\leq \frac{\cinv}{\he}\normElm{\grad\uvech}, \\
		{\norm{\uvech}}_{L^{\infty}(e)} &\leq \frac{\cinv}{(\he)^{\nsd / 2}}\normElm{\uvech},
		\end{align}
	\end{subequations}
	for every $ e \in \mesh $, where $ \he $ is the size of element $ e $, and $ \cinv $ is a constant. Details can be found in Section 3.2 of \cite{ciarlet2002finite}.
	
	\item \label{item:trace-ineq} \textit{Trace inequality:} The norm of a function $ \uvec $ on the boundary can be bounded by the norm inside the domain, i.e.,
	\begin{align}
	\norm{\uvec}_{\partial \stDom} \leq \traceConstant \norm{\uvec}_{\stDom} = \traceConstant \norm{\uvec}.
	\end{align}
	A proof can be found in Section 5.5 of \cite{evans2022partial}.
	
	\item \label{item:interp-sobolev} \textit{Interpolation in a Sobolev space:} Let $ k,\ l,\ m \in \mathbb{N} $.And let $\interpolant$ be the interpolation operator from $ \spaceV \cap [H^m(\stDom)]^{\nsd} $ to $\spaceVh$, with order of interpolation $k$. If $k, l, m $ satisfy $0\leq l \leq (k+1) \leq m $, then
	\begin{align} \label{eq:interpolation-sobolev}
	\normH[l]{\vvec-\interp{\vvec}}{\stDom}\leq \approxConstant h^{(k+1-l)}\normH[k+1]{\vvec}{\stDom},
	\end{align}
	where the constant $\approxConstant$ only depends on $k,l,m$ and is independent of $h$ and $v$ (see
	\cite{brenner2007mathematical} and Section 6.7 of \cite{jt1976introduction} for details). The following estimates are direct consequences of \eqref{eq:interpolation-sobolev} (assuming $m=k+1$).
	\begin{subequations}\label{estimate:sobolev-interp}
		\begin{align}
		\normElm{\vvec-\interp{\vvec}} &\leq {\approxConstant}_0 h^{k+1}\normH[k+1]{\vvec}{e}\ \forall e \in \mesh, \label{estimate:sobolev-interp-L2}\\
		\normElm{\grad (\vvec-\interp{\vvec})} &\leq {\approxConstant}_1 h^{k}\normH[k+1]{\vvec}{e}\ \forall e \in \mesh, \label{estimate:sobolev-interp-grad-L2}\\
		\normElm{\partial_t(\vvec-\interp{\vvec})} &\leq {\approxConstant}_1 h^{k}\normH[k+1]{\vvec}{e}\ \forall e \in \mesh, \label{estimate:sobolev-interp-time-der-L2} \\
		\normElm{\laplacian (\vvec-\interp{\vvec})} &\leq {\approxConstant}_2 h^{k-1}\normH[k+1]{\vvec}{e}\ \forall e \in \mesh. \label{estimate:sobolev-interp-laplacian-L2}
		\end{align}
	\end{subequations}
%	For the final time boundary $ \bft $, we similarly have
%	\begin{align}
%	\normL{\vvec-\interp{\vvec}}{\bft} 
%	&\leq C_{a\Gamma}h^{k+\half}\normH[k+1]{\vvec}{\stDom}.
%	\label{estimate:sobolev-interp-boundary-L2}
%	\end{align}
\end{enumerate}



\subsection{Results} \label{sec:anlys-results}
\begin{assumption} \label{thm:assumptions-c1-c2}
	In \eqref{eq:taum-tauc-codina}, $ c_1 > 2,\ c_2 > 0 $.
\end{assumption}
\begin{assumption} \label{thm:assumptions-hmax}
	Given a mesh $ \mesh $, we assume that the maximum mesh size $ h_{max} < \frac{c_2 |\avec|_{\infty}}{\epsilon} $ for some $ \epsilon > 0  $, where $ \epsilon < \frac{2}{\traceConstant} $, and $ \traceConstant $ is defined in \autoref{item:trace-ineq}.
\end{assumption}
\begin{lemma}[\textit{Coercivity}] \label{thm:coercivity}
	If \assumref{thm:assumptions-c1-c2} and \assumref{thm:assumptions-hmax} are satisfied, then the bilinear form $ \bformh $  in \eqref{eq:fem-problem-lin-vms} is coercive, i.e., there exists a positive constant $ \coer $ such that
	\begin{align}
	\bformh(\avec; \upairh, \upairh) \geq \coer \normVW[\avec]{\upairh}^2
	\end{align}
	for all $ \upairh \in \spaceVh\times\spaceQh $.
\end{lemma}
\begin{proof}
	Taking $ \vpairh = \upairh $ in \eqref{eq:fem-problem-lin-vms}, we have
	\begin{multline*}
	\bformh(\avec; \upairh, \upairh) = \halfnice \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\normh{\taum^{\halfnice}\visco \laplacian \uvech}^2 \\
	+ \normh{\tauc^{\halfnice}\divergence\uvech}^2 -\innerFTh{\taum [\opLTAdv[\avec]\uvech + \grad \ph ]}{\uvech} + \innerFTh{\taum\visco\laplacian\uvech}{\uvech}.
	\end{multline*}
	The first three terms are positive. The fourth term can be estimated using an inverse inequality as
	\begin{align*}
	-\normh{\taum^{\halfnice}\visco \laplacian \uvech}^2 \geq -\frac{\visco^2 \cinv^2}{h^2} \normh{\taum^{\halfnice} \visco \grad \uvech}^2.
	\end{align*}
	Using Cauchy's inequality $ -2ab \geq -\oneOver{\epsilon}a^2 - \epsilon b^2 $ ($ \epsilon>0 $)  for any $ a $ and $ b $, the sixth term can be estimated as
	\begin{flalign*}
	-\innerFTh{\taum [\opLTAdv[\avec]\uvech + \grad \ph ]}{\uvech} &\geq - \frac{\epsilon}{2} \normFTh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\taum^{\halfnice} \uvech}^2 \\
	&\geq - \frac{\epsilon \traceConstant}{2} \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\taum^{\halfnice} \uvech}^2.
	\end{flalign*}
	And the seventh term as
	\begin{align*}
	\innerFTh{\taum\visco\laplacian\uvech}{\uvech} &\geq \taumMax\visco \innerFTh{\laplacian\uvech}{\uvech} \\ &\geq -\taumMax\visco \normFTh{\grad \uvech}^2 + 0 \\
	&\geq -\frac{\taumMax\visco \cinv^2}{h^2} \normFTh{\uvech}^2.
	\end{align*}
	Combining,
	\begin{align*}
	\bformh(\avec; \upairh, \upairh)
%	&\geq \half \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\normh{\taum^{\halfnice}\visco \laplacian \uvech}^2 + \normh{\tauc^{\halfnice}\divergence\uvech}^2 \\
%	&\hspace{8em} -\frac{\epsilon}{2}\normFTh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\uvech}^2 -\taumMax\visco \normFTh{\grad \uvech}^2 \\
	&\geq \half \normFT{\uvech}^2 + \visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 -\frac{\visco^2 \cinv^2}{h^2}\normh{\taum^{\halfnice}\visco \grad \uvech}^2 + \normh{\tauc^{\halfnice}\divergence\uvech}^2 \\
	&\hspace{8em} -\frac{\epsilon\traceConstant}{2}\normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}^2 - \oneOver{2\epsilon}\normFTh{\taum^{\halfnice}\uvech}^2 -\frac{\taumMax\visco \cinv^2}{h^2} \normFTh{\uvech}^2 \\
	&= \Xsum_{\elemVol\in\mesh}\left[ \left( 1 - \frac{\taum^e \visco \cinv^2}{h^2}\right) \visco \norm{\grad \uvech}_{\elemVol}^2 + \left(1-\frac{\epsilon\traceConstant}{2}\right) \norm{\taum^{\halfnice}[\opLTAdv[\avec]\uvech + \grad \ph ]}_{\elemVol}^2 + \norm{\tauc^{\halfnice}\divergence\uvech}_{\elemVol}^2 \right] \\
	&\quad +\Xsum_{\elemFT\in\bftmesh} \left[ \left\{ \half -\left(\oneOver{2\epsilon} +\frac{\visco\cinv^2}{h^2}\right) \taumMax \right\} \norm{\uvech}_{\elemFT}^2 \right].
	\end{align*}
	The first term in first sum is positive since (using \eqref{eq:taum-tauc-codina} and \assumref{thm:assumptions-c1-c2})
	\begin{align}
	\oneOver{\taum^e} = \frac{c_1\cinv^2\visco}{h^2} + \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} > \frac{\visco \cinv^2}{h^2} \implies \left( 1 - \frac{\taum^e \visco \cinv^2}{h^2} \right) > 0.
	\end{align}
	The second term is positive by \assumref{thm:assumptions-hmax}. And the coefficient of the last term is
	\begin{align}
	\half \left\{ 1 - \left( \oneOver{\epsilon} + \frac{2\visco \cinv^2}{h^2} \right) \taumMax \right\} = \half \left\{ 1 - \frac{\oneOver{\epsilon} + \frac{2\visco \cinv^2}{h^2}}{\frac{c_2 |\widetilde{\avec}|_{\infty}}{h} + \frac{c_1\cinv^2\visco}{h^2}} \right\} = \half \frac{\left( \oneOver{\epsilon} - \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} \right) + \frac{(c_1-2)\cinv^2\visco}{h^2}  }{\frac{c_2 |\widetilde{\avec}|_{\infty}}{h} + \frac{c_1\cinv^2\visco}{h^2}} >0
	\end{align}
	since $ c_1>2 $ and $ 1/\epsilon > c_2 |\avec|_{\infty} / h^2 $ by \assumref{thm:assumptions-c1-c2} and \assumref{thm:assumptions-hmax}. By choosing $ \coer $ as
	\begin{align*}
	\coer = \min \left\{\left( 1 - \frac{\taumMax \visco \cinv^2}{h^2}\right), \left(1-\frac{\epsilon\traceConstant}{2}\right), \left( \half -\left[\oneOver{2\epsilon} +\frac{\visco\cinv^2}{h^2}\right] \taumMax \right)\right\},
	\end{align*}
	we prove the estimate.
%	Each of the quantities in the parentheses must be positive, i.e.,
%	\begin{align}
%	1 - \frac{\taum^e \visco \cinv^2}{h^2} > 0 &\implies \taum^e < \frac{h^2}{\visco \cinv^2}, \label{eq:cond-1} \\
%	1-\frac{\epsilon\traceConstant}{2} >0 &\implies \epsilon < \frac{2}{\traceConstant}, \label{eq:cond-2} \\
%	\text{and}\ \half -\oneOver{2\epsilon}\taumMax -\frac{\taumMax\visco\cinv^2}{h^2} >0 &\implies \taumMax < \oneOver{{\left(\oneOver{\epsilon} + \frac{\cinv^2\visco}{2h^2}\right)}}. \label{eq:cond-3}
%	\end{align}
%	Using \eqref{eq:taum-tauc-codina} in condition \eqref{eq:cond-1}, we have
%	\begin{align}
%		\left[ \frac{c_1\cinv^2\visco}{h^2} + \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} \right]^{-1} < \frac{h^2}{\visco \cinv^2} \implies \frac{c_1\cinv^2\visco}{h^2} + \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} > \frac{\visco \cinv^2}{h^2},
%	\end{align}
%	which is satisfied since $ c_1 > 1 $.
%	Also, using \eqref{eq:taum-tauc-codina} in \eqref{eq:cond-3}, we have
%	\begin{align*}
%		\oneOver{\epsilon} + \frac{\cinv^2\visco}{2h^2} < \frac{c_1\cinv^2\visco}{h^2} + \frac{c_2 |\widetilde{\avec}|_{\infty}}{h} \implies
%		(2c_1 - 1) \cinv^2 \visco + 2 c_2 |\widetilde{\avec}|_{\infty} h - 2h^2\epsilon > 0,
%	\end{align*}
%	which is satisfied since $ c_1 > 1 $ and since $ h < \frac{c_2 |\widetilde{\avec}|_{\infty}}{\epsilon} $.
%	Now, 
\end{proof}

\begin{corollary} \label{thm:uniqueness-linearized}
	Given $ \avec \in \spaceVh $, \eqref{eq:fem-problem-lin-vms} has a unique solution.
\end{corollary}
\begin{proof}
	Suppose \eqref{eq:fem-problem-lin-vms} does not have a unique solution, and assume that given a particular $ \avec \in \spaceVh $, there are two solutions $ \upairh^1 $ and $ \upairh^2 $. Then we have
	\begin{subequations}
		\begin{align}
		\bformh(\avec; \upairh^1, \vpairh) &= \lformh(\avec;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh \\
		\bformh(\avec; \upairh^2, \vpairh) &= \lformh(\avec;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh.
		\end{align}
	\end{subequations}
	Subtracting, we have
	\begin{align*}
	\bformh(\avec; \upairh^1-\upairh^2, \vpairh) &= 0 \quad \forall \vpairh \in \spaceVh \times \spaceQh.
	\end{align*}
	Choosing $ \vpairh = \upairh^1-\upairh^2 $, we have
	\begin{align*}
	0 = \bformh(\avec; \upairh^1-\upairh^2, \upairh^1-\upairh^2) \geq \coer \normVW[\avec]{\upairh^1-\upairh^2}^2,
	\end{align*}
	which implies that we must have $ \upairh^1=\upairh^2 $. 
\end{proof}
\begin{lemma} \label{thm:map-continuity}
	The linearized stabilized equation \eqref{eq:fem-problem-lin-vms}
	determines a continuous map $ F: \avec \rightarrow \upairh = F(\avec)$.
\end{lemma}
\begin{proof}
	Taking $ \vpairh = \upairh $ in \eqref{eq:fem-problem-lin-vms}, we have
	\begin{align} \label{eq:lemma-map-equality}
	\bformh(\avec; \upairh, \upairh) &= \lformh(\avec;\upairh).
	\end{align}
	From \lemref{thm:coercivity}, we can write $ \coer \normVW[\avec]{\upairh}^2 \leq \bformh(\avec; \upairh, \upairh)  $. And $ \lformh(\avec; \upairh) $ can be estimated as
	\begin{align*}
	\lformh(\avec; \upairh) &= \inner{\fvec}{\uvech} + \innerh{\taum \fvec}{[\opLTAdv[\avec]\uvech-\visco\laplacian\uvech +\grad \ph]} - \innerFTh{\taum \fvec}{\uvech} \\
	&\leq \norm{\fvec}\norm{\uvech} + \normh{\taum^{\halfnice}\fvec} \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech -\visco\laplacian\uvech +\grad \ph]} + \normh{\taum^{\halfnice} \fvec} \normh{\taum^{\halfnice}\uvech} \\
	&\leq \norm{\oneOver{\visco} \fvec}\norm{\visco \grad \uvech} + \normh{\taum^{\halfnice}\fvec} \left(\normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech +\grad \ph]} + \visco \normh{\taum^{\halfnice} \laplacian\uvech} \right) + \normFTh{\taum^{\halfnice} \fvec} \normFTh{\taum^{\halfnice}\uvech} \\
	&\leq \left[\norm{\visco^{-1}\fvec}^2 + 2\normh{\taum^{\halfnice}\fvec}^2 + \normFTh{\taum^{\halfnice}\fvec}^2\right]^{\halfnice} \\
	&\qquad \times \left[\visco\norm{\grad \uvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\avec]\uvech +\grad \ph]}^2 + \visco \normh{\taum^{\halfnice} \laplacian\uvech}^2 + \normFTh{\taum^{\halfnice}\uvech}^2 \right]^{\halfnice}
	\end{align*}
	or,
	\begin{align*}
	\lformh(\avec; \upairh) &\leq C_b \lambda(f) \normVW[\avec]{\uvech}
	\end{align*}	
	where
	\begin{subequations} \label{eq:cb-and-lambdaF}
		\begin{align}
		C_b &= \max \left\{\visco(1+\taumMax), \taumMax|_{\bft} \right\} \\
		\lambda(f) &= \left[\norm{\visco^{-1}\fvec}^2 + 2\normh{\taum^{\halfnice}\fvec}^2 + \normFTh{\taum^{\halfnice}\fvec}^2\right]^{\halfnice}.
		\end{align}
	\end{subequations}
	Then \eqref{eq:lemma-map-equality} gives
	\begin{align*}
	\coer \normVW[\avec]{\upairh}^2 \leq \bformh(\avec; \upairh, \upairh) &= \lformh(\avec;\upairh) \leq C_b \lambda(f) \normVW[\avec]{\upairh} \\
	\implies \normVW[\avec]{\upairh} &\leq R
	\end{align*}
	where
	\begin{align} \label{eq:def:R}
	R = \left(\frac{C_b}{\coer}\right) \lambda(f) = \left(\frac{C_b}{\coer}\right) \left[\norm{\visco^{-1}\fvec}^2 + 2\normh{\taum^{\halfnice}\fvec}^2 + \normFTh{\taum^{\halfnice}\fvec}^2\right]^{\halfnice}.
	\end{align}
	Now if we define the set 
	\begin{align} \label{eq:def:BR}
	B_R = \setbuilder{\upairh \in \spaceVh\times\spaceQh : \normVW[\avec]{\upairh} \leq R},
	\end{align}
	then it is easy to see that given any $ (\avec, \cdot)\in B_R $, $ F $ maps to $ \upairh $ in $ B_R $, i.e., $ F:B_R\rightarrow B_R $. 
 
 Next we prove that $ F $ is continuous.
	Let $ (\avec^i,\cdot) \in B_R \ (i=1,2) $ and that
	\begin{subequations}
		\label{eq:lemma-map-two-funcs}
		\begin{align}
		\bformh(\avec^1; \upairh^1, \vpairh) &= \lformh(\avec^1;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh \\
		\bformh(\avec^2; \upairh^2, \vpairh) &= \lformh(\avec^2;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh
		\end{align}
	\end{subequations}
	Then we also have $ \normVW[\avec^i]{\upairh^i} \leq R $ for $ i = 1,2 $. From \eqref{eq:lemma-map-two-funcs}
	\begin{align*}
	\bformh(\avec^1; \upairh^1, \vpairh) - \bformh(\avec^2; \upairh^2, \vpairh) &= \lformh(\avec^1, \vpairh) - \lformh(\avec^2, \vpairh) \\
	&= \innerh{\taum \fvec}{(\opLTAdv[\avec^1]\vvech - \opLTAdv[\avec^2]\vvech)} \\
	\implies \bformh(\avec^1; \upairh^1, \vpairh) &= \bformh(\avec^2; \upairh^2, \vpairh) + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech}
	\end{align*}
	
	Now,
	\begin{align*}
	\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &= \bformh(\avec^1; \uvech^1, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) \\
	&= \bformh(\avec^2; \uvech^2, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech} \\
	&= -\inner{\uvech^2}{(\opLTAdv[\avec^2]-\opLTAdv[\avec^1])\vvech} \\
	&\quad + \innerh{\taum [\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 + \grad \ph^2 ]}{[\opLTAdv[\avec^2]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
	&\quad- \innerh{\taum [\opLTAdv[\avec^1]\uvech^2-\visco\laplacian\uvech^2 + \grad \ph^2 ]}{[\opLTAdv[\avec^1]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
	&\quad -\innerFTh{\taum (\opLTAdv[\avec^2]\uvech - \opLTAdv[\avec^1] \uvech)}{\vvech} \\
	&\quad + \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{12}]\vvech} \\
	&= -\inner{\uvech^2}{\opLTAdv[\delta \avec^{21}]\vvech} \\
	&\quad + \innerh{\taum \opLTAdv[\delta \avec^{21}]\uvech^2}{[\opLTAdv[\avec^1]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
	&\quad + \innerh{\taum ([\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \ph^2]}{\opLTAdv[\delta \avec^{21}] \vvech} \\
	&\quad -\innerFTh{\taum \opLTAdv[\delta \avec^{21}]\uvech^2}{\vvech} \\
	&\quad - \innerh{\taum \fvec}{\opLTAdv[\delta \avec^{21}]\vvech}
	\end{align*}
	
	\begin{align*}
	\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &= \bformh(\avec^1; \uvech^1, \vvech) - \bformh(\avec^1; \uvech^2, \vvech) \\
	&= -\inner{\uvech^2}{\opLAdv[\delta \avec^{21}]\vvech} \\
	&\quad + \innerh{\taum \opLAdv[\delta \avec^{21}]\uvech^2}{[\opLTAdv[\avec^1]\vvech-\visco\laplacian\vvech +\grad \qh]} \\
	&\quad + \innerh{\taum ([\opLTAdv[\avec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \ph^2]}{\opLAdv[\delta \avec^{21}] \vvech} \\
	&\quad -\innerFTh{\taum \opLAdv[\delta \avec^{21}]\uvech^2}{\vvech} \\
	&\quad - \innerh{\taum \fvec}{\opLAdv[\delta \avec^{21}]\vvech} \\
	&=: S_1 + S_2 + S_3 + S_4 + S_5
	\end{align*}
	$ S_5 $	 can be bounded as
	\begin{align*}
	|S_5| \leq \norm{\taum f}_{L^2}\norm{\delta \avec^{21}}_{L^{\infty}}\norm{\grad \vvech}_{L^2}.
	\end{align*}
	Using the discrete inverse inequality and Poincare's inequality, we have
	\begin{align*}
	\norm{\davec}_{L^{\infty}} &\leq Ch^{-\xi} \norm{\davec}_{L^2} \\
	&\leq Ch^{-\xi} \norm{\grad \davec}_{L^2}
	\end{align*}
	where $ \xi = -1,-\halfnice $ for $ n=2,3 $ respectively. Therefore
	\begin{align*}
	\seminorm{S_5} \leq \cinv h^{-\xi} \norm{\taum f}_{L^2}\norm{\grad \delta \avec^{21}}_{L^2}\norm{\grad \vvech}_{L^2}.
	\end{align*}
	For $ S_1 $ through $ S_4 $, we can similarly obtain
	\begin{align*}
	\seminorm{S_1} &\leq \beta R\norm{\grad \davec}_{L^2}\norm{\grad \vvech}_{L^2} \\
	\seminorm{S_2} &\leq \cinv h^{-\xi}\taumMax \norm{\grad \uvech^2}_{L^2} \norm{\grad \davec}_{L^2} \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} + \visco \normh{\grad \vvech}  \right) \\
	&\leq \cinv h^{-\xi}\taumMax R \norm{\grad \davec}_{L^2} \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} + \visco \normh{\grad \vvech}  \right) \\
	\seminorm{S_3} &\leq \cinv h^{-\xi}\taumMax \left( \normh{\taum^{\halfnice} [\opLTAdv[\avec^2]\uvech^2 + \grad \ph^2]} + \visco \normh{\grad \uvech^2} \right) \norm{\grad \davec}_{L^2} \norm{\grad \vvech}_{L^2} \\
	&\leq \cinv h^{-\xi}\taumMax R \norm{\grad \davec}_{L^2} \norm{\grad \vvech}_{L^2} \\
	\seminorm{S_4} &\leq \cinv h^{-\xi_b} \taumMax R \normFT{\grad \davec} \normFT{\grad \vvech} \\
	&\leq \cinv^2 h^{-\xi_b-1} \taumMax R \norm{\grad \davec} \normFT{\vvech}
	\end{align*}
	where in case of $ S_4 $, we have used $ \normFT{\grad\davec} \leq C\norm{\grad\davec} $ and $ \normFT{\grad \vvech} \leq \frac{\cinv}{h}\normFT{\uvech}$. Thus, combining them, we have
	\begin{align*}
	\bformh(\avec^1; \upairh^1-\upairh^2, \vpairh) &\leq \Xsum_{i=1}^4 \seminorm{S_i} \\
	&\leq \norm{\grad \davec} \Bigg[ C_1(R,h,\taumMax) \normFT{\vvech} + C_2(R,h,\taumMax) \norm{\grad\vvech} \\
	&\qquad\qquad\qquad + C_3(R,h,\taumMax) \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]} \Bigg] \\
	&\leq \norm{\grad \davec} \left[C_1^2 + C_2^2 + C_3^2 \right]^{\halfnice} \left[\normFT{\vvech}^2 + \norm{\grad\vvech}^2 + \normh{\taum^{\halfnice} [\opLTAdv[\avec^1]\vvech + \grad \qh]}^2 \right]^{\halfnice} \\
	&=: \tilde{C} \normVW[\avec^1]{\vpairh} \norm{\grad \davec}
	\end{align*}
	where $ \tilde{C} = \left[C_1^2 + C_2^2 + C_3^2 \right]^{\halfnice} $. Now, if we choose $ \vpairh = \upairh^1 - \upairh^2 $, then
	\begin{align*}
	\bformh(\avec^1; \upairh^1-\upairh^2, \upairh^1-\upairh^2) &\leq \tilde{C}\normVW[\avec^1]{\upairh^1-\upairh^2} \norm{\grad \davec}
	\end{align*}
	By means of coercivity, we also have
	\begin{align*}
	\bformh(\avec^1; \upairh^1-\upairh^2, \upairh^1-\upairh^2) \geq \coer \normVW[\avec^1]{\upairh^1-\upairh^2}^2.
	\end{align*}
	So, we have
	\begin{align*}
	\coer \normVW[\avec^1]{\upairh^1-\upairh^2}^2 &\leq \tilde{C}\normVW[\avec^1]{\upairh^1-\upairh^2} \norm{\grad \davec} \\
	\implies \normVW[\avec^1]{\upairh^1-\upairh^2} &\leq \left(\frac{\tilde{C}}{\coer}\right) \norm{\grad(\avec^1-\avec^2)},
	\end{align*}
	which proves that $ \upairh $ continuously depends on $ \avec $, thus $ F $ is a continuous map.
\end{proof}

\begin{lemma}[\textit{Existence}] \label{thm:existence-nonlinear}
	If $ \fvec \in [L^2(\stDom )]^{\nsd} $, then the nonlinear problem \eqref{eq:fem-problem-vms} has at least one solution $ \upairh = (\uvech, \ph) $.
\end{lemma}
\begin{proof}
	By \lemref{thm:map-continuity}, we know that the linear map $ \upairh = F(\avec) $ corresponding to \eqref{eq:fem-problem-lin-vms} is a continuous map from $ B_R $ to $ B_R $. Therefore by Brouwer's fixed point theorem, $ F $ must have at least one fixed point $ \upairh = F(\uvech) $. Therefore \eqref{eq:fem-problem-vms} has at least one solution.
\end{proof}

%\subsection{Uniqueness of Solution} \label{sec:uniqueness}
\begin{theorem}[\textit{Uniqueness}] \label{thm:uniqueness}
	The nonlinear problem \eqref{eq:fem-problem-vms} has a unique solution $ \upairh = (\uvech, \ph) $ that satisfies \begin{align}
	\normVW[\uvech]{\upairh} \leq R,
	\end{align}
	where $ R = \left(\nicefrac{C_b}{\coer}\right) \lambda(f) $; $ C_b,\ \lambda(f) $ are defined in \eqref{eq:cb-and-lambdaF}, and $ \coer $ is the constant of stability (defined in \lemref{thm:coercivity}).
\end{theorem}
\begin{proof}
	By \lemref{thm:existence-nonlinear},  \eqref{eq:fem-problem-vms} has at least one solution $ \upairh = (\uvech, \ph)$. So, we have
	\begin{align}
		\bformh(\uvech; \upairh, \vpairh) &= \lformh(\uvech;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh.
	\end{align}
	Choosing $ \vpairh = \upairh $ in the above equation, and following a similar process as in the proof of \lemref{thm:map-continuity}, we find that
	\begin{align*}
		\coer \normVW[\uvech]{\upairh}^2 \leq \bformh(\uvech; \upairh, \upairh) &= \lformh(\uvech;\upairh) \leq C_b \lambda(f) \normVW[\uvech]{\upairh} \\
		\implies \normVW[\uvech]{\upairh} &\leq \left(\nicefrac{C_b}{\coer}\right) \lambda(f) = R
	\end{align*}
	To prove that $ \upairh $ is unique, let us assume that $ \upairh^1 = (\uvech^1,\ph^1) $ and $ \upairh^2  = (\uvech^2,\ph^2) $ are two different solutions of \eqref{eq:fem-problem-vms}, i.e.,
		\begin{subequations}
		\label{eq:lemma-uniqueness-two-funcs}
		\begin{align}
			\bformh(\uvech^1; \upairh^1, \vpairh) &= \lformh(\uvech^1;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh \\
			\bformh(\uvech^2; \upairh^2, \vpairh) &= \lformh(\uvech^2;\vpairh) \quad \forall \vpairh \in \spaceVh \times \spaceQh.
		\end{align}
	\end{subequations}
	Suppose $ \eta_h = \upairh^1-\upairh^2 = (\uvech^1-\uvech^2, \ph^1-\ph^2) = (\wvech,\rh)$. Once again, following a similar process as in the proof of \lemref{thm:map-continuity}, we have
	\begin{align*}
		\bformh(\uvec^1; \eta_h, \eta_h) &= \bformh(\uvec^1; \upairh^1-\upairh^2, \eta_h) \\
		 &= \bformh(\uvec^1; \upairh^1, \wvech) - \bformh(\uvec^1; \upairh^2, \wvech) \\
		&= -\inner{\uvech^2}{\opLAdv[\wvech]\wvech} \\
		&\quad + \innerh{\taum \opLAdv[\wvech]\uvech^2}{[\opLTAdv[\uvec^1]\wvech-\visco\laplacian\wvech +\grad \rh]} \\
		&\quad + \innerh{\taum ([\opLTAdv[\uvec^2]\uvech^2-\visco\laplacian\uvech^2 +\grad \rh^2]}{\opLAdv[\wvech] \wvech} \\
		&\quad -\innerFTh{\taum \opLAdv[\wvech]\uvech^2}{\wvech} \\
		&\quad - \innerh{\taum \fvec}{\opLAdv[\wvech]\wvech} \\
		&=: T_1 + T_2 + T_3 + T_4 + T_5
	\end{align*}
	Using \lemref{thm:coercivity}, we have
	\begin{align}
	\coer \normVW[\uvec^1]{\eta_h}^2 \leq \bformh(\uvec^1; \eta_h, \eta_h) = T_1 + T_2 + T_3 + T_4 + T_5 \\
	\label{eq:lemma-uniqueness-e2}
	\implies \coer \left( \normFT{\wvech}^2 + \norm{\grad \wvech}^2 + \normh{\taum^{\halfnice}[\opLTAdv[\uvec^1] \wvech + \grad \rh]}^2\right) - \Xsum_{j=1}^5 T_j \leq 0.
	\end{align}
	Now, we estimate each $ T_j,\ j=1,\ldots,5 $ as follows.
	\begin{align*}
		\seminorm{T_1} &\leq \beta R \norm{\grad \wvech}^2, \\
		\seminorm{T_2} &\leq \cinv h^{-\xi} \taumMax R \left(\norm{\grad \wvech} \normh{\taum^{\halfnice}[\opLTAdv[\uvech^1]\wvech + \grad \rh]} + \visco\norm{\grad \wvech}^2\right) \\
		&\leq \cinv h^{-\xi} \taumMax R \left[\left(\visco + \half\right) \norm{\grad \wvech}^2 + \half \normh{\taum^{\halfnice}[\opLTAdv[\uvech^1]\wvech + \grad \rh]}^2 \right], \\
		\seminorm{T_3} &\leq \cinv h^{-\xi} \taumMax R \norm{\grad \wvech}^2, \\
		\seminorm{T_4} &\leq \cinv h^{-\xi_b} \taumMax R \normFT{\grad \wvech}^2 \\ 
		&\leq \cinv^2 h^{-\xi_b-1} \taumMax R \normFT{\wvech}^2, \\
		\seminorm{T_5} &\leq \cinv h^{-\xi} \taumMax \norm{\fvec} \norm{\grad\wvech}^2.
	\end{align*}
	Substituting each of these five estimates into \eqref{eq:lemma-uniqueness-e2}, and collating the similar terms, we have
	\begin{align} \label{eq:lemma-uniqueness-e3}
		\lambda_1 \normFT{\wvech}^2
		+\lambda_2 \normh{\taum^{\halfnice}\left[\opLTAdv[\uvech^1] \wvech + \grad \rh \right]}^2 + \lambda_3 \norm{\grad \wvech}^2 \leq 0,
	\end{align}
	where
	\begin{align*}
		\lambda_1(h) &= \coer - \cinv^2 h^{-\xi_b-1} \taumMax R, \\
		\lambda_2(h) &= \coer - \half \cinv^2 h^{-2\xi}  {\taumMax}^2 R^2, \\
		\lambda_3(h) &= \coer - \left[\beta R + \cinv h^{-\xi}\taumMax \left\{R \left( \nicefrac{3}{2} + \visco \right) + \norm{\fvec} \right\} + \half \cinv^2 h^{-2\xi} {\taumMax}^2 R^2 \right].
	\end{align*}
    There exists a $ \hzero $ such that for each $ h \leq \hzero $, we have $\lambda_i(h) \geq 0,\ i=1,2,3$. Then each of the norms appearing on the left hand side of \eqref{eq:lemma-uniqueness-e3} must amount to 0. Thus we must have $ \wvech = \mathbf{0} $, and also $ \rh = 0 $. Therefore, we have that  $ \upairh^1 = \upairh^2 $, proving the uniqueness of the solution.
\end{proof}

\begin{theorem}[\textit{Convergence}] \label{thm:convergence}
	Assume that the exact solution of \eqref{eq:fem-problem-vms} is $ \phi = (\uvec, p) \in (H^{k+1}(\stDom )\cap \spaceV) \times (H^{k+1}(\stDom )\cap\spaceQ),\ k \in \mathbb{N} $. Then for the discrete solution $ \upairh $, we have the following estimate:
	\begin{align}
	\normVW[\uvec]{\upairh - \upair} \leq C h^{k},
	\end{align}
	where $ C $ depends on $ \norm{\uvec}_{H^{k+1}} $ and $ \norm{p}_{H^{k+1}} $, and $ k $ is the order of the basis functions.
\end{theorem}
\begin{proof}
	Suppose $ \interpolant^u: \spaceV \cap H^{k+1}(\stDom) \rightarrow \spaceVh  $ is the projection of $ \uvec $ from $\spaceV$ to $\spaceVh$; and similarly $ \interpolant^p: \spaceQ \cap H^{k+1}(\stDom ) \rightarrow \spaceQh $. We assume that both $ \interpolant^u $ and $ \interpolant^p $ have the degree of interpolation $ k \in \mathbb{N} $.
	
	Let $ \wvech = \uvech - \interpolant\uvech $ and $ \rh = \ph - \interpolant\ph $, and $ \hat{\eta} = (\wvech, \rh)$. Consequently $ \hat{\eta} = \upairh - \interpolant\upairh $. Using \eqref{eq:fem-problem-lin-vms},
	\begin{align*}
		\bformh(\uvec; \hat{\eta}, \hat{\eta}) &= \bformh(\uvec; \upairh - \interp{\upair}, \hat{\eta}) \\
		&= \bformh(\uvec; \upairh, \hat{\eta}) - \bformh(\uvec; \interp{\upair}, \hat{\eta}) \\
		&= \bformh(\uvec; \upair, \hat{\eta}) - \bformh(\uvec; \interp{\upair}, \hat{\eta}) \\
		&= \bformh(\uvec; \upair-\interp{\upair}, \hat{\eta}) \\
		&= -\inner{\duh}{\opLTAdv[\uvec] \wvech} + \visco \inner{\grad (\duh)}{\grad \wvech} - \inner{\dph}{\divergence\wvec} + \inner{\divergence (\duh)}{\rh} \\
		&\quad + \innerFT{\duh}{\wvech} + \innerh{\taum [\opLTAdv[\uvec] (\duh) -\visco \laplacian (\duh) + \grad (\duh)] }{[\opLTAdv[\uvec]-\visco\laplacian\wvech + \grad\rh]} \\
		&\quad \innerh{\tauc \divergence(\duh)}{\divergence \wvech} - \innerFTh{\taum [\opLTAdv[\uvec](\duh)-\visco\laplacian(\duh)+\grad (\dph)]}{\wvech} \\
		&= \Xsum_{i=1}^{8} S_i
	\end{align*}
	Denote $ \alpha := k+1 $, $ \eeu := \normH[k+1]{\uvec}{e} $ and $ \eep := \normH[k+1]{p}{e} $. Using the estimates in \eqref{estimate:sobolev-interp} we have
	\begin{subequations}
		\begin{align}
		\normElm{\duh} &\leq C\he^{\alpha}\eeu, \\
		\normElm{\grad \duh} &\leq C \he^{\alpha-1}\eeu, \\
		\normElm{\partial_t \duh} &\leq C \he^{\alpha-1}\eeu, \\
		\normElm{\laplacian \duh} &\leq C\he^{\alpha-2}\eeu, \\
		\normElm{\dph} &\leq C\he^{\alpha}\eep, \\
		\normElm{\grad \dph} &\leq C\he^{\alpha-1} \eep.
	\end{align}
	\end{subequations}
	Then,
	\begin{align*}
	S_1 = -\inner{\duh}{\opLTAdv[\uvec] \wvech} =\elmsum -\inner{\duh}{\opLTAdv[\uvec] \wvech}_e &= \elmsum \beta \normElm{\grad \duh}\normElm{\grad \uvec}\normElm{\grad \wvech} \\
	&\leq \elmsum \beta R C \he^{\alpha-1} \eeu \normElm{\grad\wvech}
	\end{align*}
	\begin{align*}
	S_2 = \visco \inner{\grad (\duh)}{\grad \wvech} = \elmsum \visco \inner{\grad (\duh)}{\grad \wvech}_e &\leq \elmsum \visco \normElm{\grad \duh}\normElm{\grad \wvech} \\
	&\leq \elmsum \visco C\he^{\alpha-1}\eeu \normElm{\grad \wvech}
	\end{align*}
	\begin{align*}
	S_3 =  - \inner{\dph}{\divergence\wvec} = \elmsum - \inner{\dph}{\divergence\wvec}_e \leq \elmsum \normElm{\dph}\normElm{\divergence\wvech} &\leq \elmsum \sqrt{\nsd}\normElm{\dph}\normElm{\grad \wvech} \\
	&\leq \elmsum \sqrt{\nsd}C\he^{\alpha}\eep\normElm{\grad \wvech}
	\end{align*}
	\begin{align*}
	S_4 &=  \inner{\divergence (\duh)}{\rh} = \inner{\divergence (\eie{\uvec})}{\rh} = \inner{\divergence \uvec - \divergence \interp{\uvec}}{\rh} = 0,
	\end{align*}
	since $ \divergence\uvec =0 $ and $ \divergence\interp{\uvec} = 0$.
	\begin{align*}
	S_5 &= \innerFT{\duh}{\wvech} = \elmsumFT {\inner{\duh}{\wvech}}_e \leq \elmsumFT \normElm{\duh} \normElm{\wvech} \leq \elmsumFT C\he^{\alpha}\eeu \norm{\wvech}_e 
	\end{align*}
	\begin{align*}
	S_6 &= \innerh{\taum [\opLTAdv[\uvec] (\duh) -\visco \laplacian (\duh) + \grad (\duh)] }{[\opLTAdv[\uvec]-\visco\laplacian\wvech + \grad\rh]} \\
	&= \elmsum \inner{\taum [\opLTAdv[\uvec] (\duh) -\visco \laplacian (\duh) + \grad (\duh)] }{[\opLTAdv[\uvec]-\visco\laplacian\wvech + \grad\rh]}_e \\
	&\leq \elmsum \taum^e \left(CR\he^{\alpha-1}\eeu + \visco C \he^{\alpha-2}\eeu + C\he^{\alpha}\eep \right) \left[\normElm{\opLTAdv[\uvec]\wvech + \grad\rh} + \frac{\visco \cinv}{\he} \normElm{\grad \wvech}\right]
	\end{align*}
	\begin{align*}
	S_7 = \innerh{\tauc \divergence(\duh)}{\divergence \wvech} &= \elmsum \inner{\tauc \divergence(\duh)}{\divergence \wvech}_e \leq \elmsum \tauc^e\normElm{\divergence\duh}\normElm{\divergence\wvech} \\
	&\leq \elmsum \tauc^e\sqrt{\nsd}\normElm{\grad\duh} \sqrt{\nsd}\normElm{\grad\wvech} \leq \elmsum \tauc^e \nsd C\he^{\alpha-1}\eeu \normElm{\grad \wvech} 
	\end{align*}
	\begin{align*}
	S_8 &= \innerFTh{\taum [\opLTAdv[\uvec](\duh)-\visco\laplacian(\duh)+\grad (\dph)]}{\wvech} \\
	&= \elmsumFT \inner{\taum [\opLTAdv[\uvec](\duh)-\visco\laplacian(\duh)+\grad (\dph)]}{\wvech}_e \\
	&\leq \elmsumFT \taum^e \left[ C\he^{\alpha-1}\eeuFT  + \visco C\he^{\alpha-2}\eeuFT + C\he^{\alpha}\eepFT \right]\normElm{\wvech}
	\end{align*}
	Combining all terms, we have
	\begin{align*}
	\Xsum_{i=1}^{8} S_i &= \elmsumFT \lambda_1^e \normElm{\wvech} + \elmsum \lambda_2^e \normElm{\grad \wvech} + \elmsum \lambda_3^e \normElm{\opLTAdv[\uvec]\wvech + \grad\rh} \\
	&\leq \left[ \elmsumFT (\lambda_1^e)^2 + \elmsum (\lambda_2^e)^2 + \elmsum (\lambda_3^e)^2 \right]^{\halfnice} \times \left[ \elmsumFT \normElm{\wvech}^2 + \elmsum \normElm{\grad \wvech}^2 + \elmsum \normElm{\opLTAdv[\uvec]\wvech + \grad\rh}^2 \right]^{\halfnice} \\
	&= \lambda \normVW[\uvec]{(\wvech,\rh)} = \lambda \normVW[\uvech]{\eta},
	\end{align*}
	where
	\begin{align*}
	\lambda_1^e &= \he^{\alpha-2}\left[C\he^2\eeuFT + \taum^e \left(C\he\eeuFT + \visco C \eeuFT + C\he^2\eepFT \right)\right], \\
	\lambda_2^e &= \he^{\alpha-2} \big[\beta R C\he^2 \eeu + \visco C\he\eeu + C\sqrt{\nsd}\he^2\eep + C\taucMax\nsd \he \eeu \\ & \qquad\qquad\qquad\qquad\qquad\qquad + \taum^e\left( CR\eeu + \visco C\visco\he^{-1}\eeu + C\he\visco\cinv \eep \right) \big], \\
	\lambda_3^e &= \he^{\alpha-2}\taum^e \left[CR\he\eeu + \visco C\eeu + C\he^2\eep \right], \\
	\text{and}\ \lambda &= \left[ \elmsumFT (\lambda_1^e)^2 + \elmsum (\lambda_2^e)^2 + \elmsum (\lambda_3^e)^2 \right]^{\halfnice} .
	\end{align*}
	We have $ \taum^e \sim \he^2 $, therefore we have
	\begin{align*}
		\lambda_1 &= C_1 h^{\alpha}, \\
		\lambda_2 &= C_2 h^{\alpha-1}, \\
		\lambda_3 &= C_3 h^{\alpha},
	\end{align*}
	where $ h=\max_{e \in \mesh} \he $.
	Using coercivity of the bilinear form, we have
	\begin{align*}
	\coer\normVW[\uvec]{\hat{\eta}}^2 \leq \bformh(\uvec; \hat{\eta}, \hat{\eta}) \leq \lambda \normVW[\uvec]{\hat{\eta}},
	\end{align*}
	therefore
	\begin{align}
	\normVW[\uvec]{\hat{\eta}} \leq \coer^{-1}\lambda = Ch^{\alpha-1}.
	\end{align}
	By triangle inequality,
	\begin{align*}
		\normVW[\uvec]{\upairh - \upair} &\leq \normVW[\uvec]{\upairh - \interpolant\upair} + \normVW[\uvec]{\interpolant \upair - \upair} \\
		&\leq C h^{\alpha-1} + C h^{\alpha-1}\\
		&= C h^{k}.
	\end{align*}
\end{proof}

\subsection{The case of nonzero initial and boundary conditions} \label{sec:nonzero-icbc}
In \eqref{eq:ns-original-dirichlet} and the preceding analysis, we considered zero boundary conditions. Suppose instead, we have the following set of equations:
\begin{subequations}\label{eq:ns-original-D}
	\begin{align}
		\opLTAdv[\uvecTilde]\uvecTilde -\visco\laplacian \uvecTilde+\grad p - 
		\fvecTilde &= \zerovec, \text{ }\xvecst\in\stDom, \label{eq:ns-original-momentum-D}
		\\
		\grad\cdot\uvecTilde &= 0, \text{ }\xvecst\in\stDom, \label{eq:ns-original-continuity-D}
		\\
		\uvecTilde &= \gvec, \text{ }\xvecst\in\bsp, \label{eq:ns-original-dirichlet-D}
		%	\\
		%	\mathscr{B}_{NR} \uvec &= h, \text{ }\xvecst\in\Gamma_{S2}\subseteq\bsp, \label{eq:ns-original-neumann}
		\\
		\uvecTilde &= \uvec_0, \text{ }\xvecst\in\bit, \label{eq:ns-original-ic-D},
	\end{align}
\end{subequations}
where \eqref{eq:ns-original-D} differs from \eqref{eq:ns-original} only on the boundary conditions (i.e. \eqref{eq:ns-original-dirichlet} and \eqref{eq:ns-original-dirichlet-D}). In this case, we proceed as follows.
Consider the following function spaces
\begin{subequations}
	\begin{align}
	\spaceVd_g &= \left\{ \mvec{v} \in \mvec{H}^1(\stDom):\ \mvec{v} = \mvec{g} \text{ on }\bsp, \text{ } \mvec{v} = \uvec_0 \text{ on } \bit \right\}, \\
	\spaceHdiv &= \setbuilder{\vvec \in \mvec{H}^1(\stDom):\ \divergence\vvec = 0}.
	\end{align}
\end{subequations}
Suppose $ (\tilde{\uvec}, p) $ is a solution of \eqref{eq:ns-original-D}. Now, let $ \uproxy \in \spaceVd_g \cap \spaceHdiv $, such that $ \text{Tr}(\uproxy) = \gvec $. Then the difference $ \uvec := \tilde{\uvec} - \uproxy \in \spaceVd $. Substituting $ \tilde{\uvec} = \uvec + \uproxy $ in \eqref{eq:ns-original}, and using the $ \opLTAdv $ notation (see \eqref{eq:def-la-ma}), we have
\begin{subequations}\label{eq:ns-transformed}
	\begin{align}
	\opLTAdv[\uvec+\uproxy]\uvec -\visco\laplacian\uvec + \grad p - \left[\fvecTilde - (\opLTAdv[\uvec+\uproxy]\uproxy - \visco\laplacian\uproxy)\right] &= \zerovec, \ \xvecst\in\stDom, \label{eq:ns-transformed-momentum}
	\\
	\grad\cdot\uvec &= 0, \ \xvecst\in\stDom, \label{eq:ns-transformed-continuity}
	\\
	\uvec &= 0, \ \xvecst\in\bsp \cup \bit. \label{eq:ns-transformed-dirichlet}
	\end{align}
\end{subequations}
where $ \uproxy $ is assumed to be sufficiently smooth. For a known advection field $ \avec \in \spaceVd $, the momentum equations can be written as
\begin{align}
	\opLTAdv[\avec+\uproxy]\uvec -\visco\laplacian\uvec + \grad p - \fvec &= \zerovec, \ \xvecst\in\stDom,
\end{align}
where $ \fvec := \left[\tilde{\fvec} - (\opLTAdv[\avec+\uproxy]\uproxy - \visco\laplacian\uproxy)\right] $. Since $ \uproxy $ is a chosen function, \eqref{eq:ns-transformed} can be solved for $ \uvec $ using a Galerkin formulation, and then added to $ \uproxy $ to obtain the solution $ \tilde{\uvec} $ of \eqref{eq:ns-original}. With this reformulation, we can proceed in the same way as \secref{sec:anlys-results} and obtain similar error estimates. 

%%For all the analytical results in the sequel, we will assume that an appropriate function $ \uproxy $ is available, and that \eqref{eq:ns-original} has been transformed into the form of \eqref{eq:ns-transformed}.
